Reconstructing Test Labels from Noisy Loss Functions

Machine learning classifiers rely on loss functions for performance evaluation, often on a private (hidden) dataset. In a recent line of research, label inference was introduced as the problem of reconstructing the ground truth labels of this private dataset from just the (possibly perturbed) cross-entropy loss function values evaluated at chosen prediction vectors (without any other access to the hidden dataset). In this paper, we formally study the necessary and sufficient conditions under which label inference is possible from \emph{any} (noisy) loss function value. Using tools from analytical number theory, we show that a broad class of commonly used loss functions, including general Bregman divergence-based losses and multiclass cross-entropy with common activation functions like sigmoid and softmax, it is possible to design label inference attacks that succeed even for arbitrary noise levels and using only a single query from the adversary. We formally study the computational complexity of label inference and show that while in general, designing adversarial prediction vectors for these attacks is co-NP-hard, once we have these vectors, the attacks can also be carried out through a lightweight augmentation to any neural network model, making them look benign and hard to detect. The observations in this paper provide a deeper understanding of the vulnerabilities inherent in modern machine learning and could be used for designing future trustworthy ML.

==> AISTATS'22/bregman.tex <==


 

% \begin{proof}
% See Appendix.
% \end{proof}

% Thus, a separating vector for the Bregman loss is obtained by setting $g(\theta_i) = \tau \ln p_i$, where $p_i$ is the $i^{th}$ prime number, as follows:
% \begin{align*}
%     &\frac{1}{N}\paran{\theta_i (a-b)+\phi(1)- \phi(0)-a} = \tau \ln p_i \\
%     \implies & \theta_i = \frac{N\tau \ln p_i + \phi(0) + a - \phi(1)}{a-b}.
% \end{align*}

% \subsection{Examples of Bregman Losses: Norm-Like Divergence Loss}
% The norm-like divergence based loss is defined with respect to $F(x,y) = x^\alpha + y^\alpha$, for some given $\alpha \geq 2$. Note that for $\alpha = 2$, this is the same as the Squared-Euclidean divergence based loss. From the definition of $F$, we obtain $\nabla F(x,y) = [\alpha x^{\alpha-1}, \alpha y^{\alpha-1}]$, and the constants required for the prediction vector computation as follows:
% \begin{align*}
%     \phi(0) &= F(0,1) = 1 = \phi(1)\\
%     a &= \langle \nabla F([1,0]), [1,-1] \rangle = \alpha, \text{and}\\
%     b &= \langle \nabla F([0,1]), [1,-1] \rangle = -\alpha.
% \end{align*}
% From this, we obtain that setting the prediction vector as follows suffices:
% $$\theta_i = \paran{N\tau \ln p_i +\alpha}/(2\alpha).$$
% Robust label inference can now be performed using Algorithm~\ref{alg:linearly_separable} (steps 2 through 5).

==> AISTATS'22/codomain_intro.tex <==
We begin our discussion by formally defining the notion of codomain separability and its connections to label inference in the noised as well as unnoised setting. Our objects of interest are functions whose domain is the Cartesian product of the space of all labelings (defined by the  $\ZZZ_K^N = \ZZZ_K \times \dots \times \ZZZ_K \ \text{($N$ times)} = \{0,\dots,K-1\}^N$) and an arbitrary set $\Theta \subseteq \mathbb{R}^N$. Here, $K \geq 2$ represents the number of label classes.
% , for e.g., in the binary case $K =2$. 
This formulation captures the common scenario in machine learning, where we evaluate a loss function using the true labeling in $\ZZZ_K^N$ for $N$ datapoints based on a (prediction) vector in $\mathbb{R}^N$ generated by an ML model. $\Theta$ is the space of prediction vectors, and for $\theta =[\theta_1,\dots,\theta_N] \in \Theta$, the value of $\theta_i$ encodes the label prediction for the $i$th datapoint. We work with different loss functions that place different restrictions on $\Theta$. All missing details from this section are presented in Appendix~\ref{app:prelim}.
% For example, in the case of binary cross-entropy loss (log-loss), we have a prediction probability vector $\theta \in [0,1]^N$ and a labeling $\sigma \in \{0,1\}^N$; the loss on $(\sigma,\theta)$ is given by:
% \begin{align}
%     \label{eq:log_loss_defn}
%     \logloss\paran{\sigma,\theta} = \frac{-1}{N}\ln \paran{\prod_{i=1}^N \theta_i^{\sigma_i}(1-\theta_i)^{1-\sigma_i}}.
% \end{align}
% In this case, $\theta_i$ is the probability assigned to the event $\sigma_i = 1$ by the ML model.
% As another example, consider another common loss function ....
% \shiva{Add another example that we consider.}
% As another example, consider another common loss function, the Kullback-Leibler loss (or KL-loss in short), which is defined as follows for $\theta \in [0,1]^N$ and $\sigma \in \{0,1\}^N$ (see~\citep{van2014renyi} for a primer on R\'enyi divergences):
% \begin{align}
%     \label{eq:kl_loss_defn}
%     \textsc{KL-Loss}(\sigma,\theta) = \sum_{i=1}^N \paran{\sigma_i \ln \frac{\sigma_i}{\theta_i} + (1-\sigma_i) \ln \frac{(1-\sigma_i)}{(1-\theta_i)}}.
% \end{align}
% More generally, the R\'enyi-Loss of order $\alpha \in (0,\infty)$ can be defined for $\theta \in [0,1]^N$ and $\sigma \in \{0,1\}^N$ as follows (for $\alpha = 1$ this is the same as the KL-loss above):
% \begin{align}
%     \label{eq:R\'enyi_loss_defn}
%     \textsc{R\'enyi-Loss}_\alpha(\sigma,\theta) = \frac{1}{\alpha-1}  \sum_{i=1}^N \ln   \paran{\sigma_i^\alpha \theta_i^{1-\alpha} + (1-\sigma_i)^\alpha (1-\theta_i)^{1-\alpha}}.
% \end{align}
% For example, in the case of multiclass cross-entropy loss (with $K$ classes), we have $\Theta \in [0,1]^{N \times K}$.  
% Note that different loss functions place different restrictions on $\Theta$ (i.e., $\Theta \in [0,1]^{N\times K}$, $\Theta \in \{0,1\}^N$, etc.). For the binary label case that we consider in this paper, we can convert $\theta \in [0,\infty)^N$ to $\theta' \in [0,1]^N$ by using the transformation $\theta_i' = \theta_i/(1+\theta_i)$. This is equivalent to saying that for the $i$th datapoint, the probability that it belongs to class $1$, as predicted by $\theta'$ is $\theta_i'$, and that for class $0$ is $1 - \theta_i' = 1/(1+\theta_i)$.

\noindent\textbf{Codomain Separability.} Informally, we call a function codomain separable if there exists some vector $\theta \in \Theta$ such that the function output is distinct on each $\ZZZ_K^N$ (keeping $\theta$ fixed). Thus, when $\theta$ is known, this one-one correspondence between the function's output and the labelings in $\ZZZ_K^N$ can be exploited to exactly recover all the labels from just observing the output.
% \footnote{Codomain separability differs from other notions of separability defined in the literature for functional analysis.}
% For example, multiplicatively separable functions $f(x,y)$ can be expressed as a product of two functions $f(x,y) = g(x)h(y)$, and additively separable functions satisfy $f(x,y) = g(x) 
% + h(y)$. Another important distinction we make is with hyperplane separability over sets of points in $\mathbb{R}^N$, which is a common notion in non-negative matrix factorization and image segmentation literature~\citep{arora2016computing,donoho2004does}.
% \shiva{Using \emph{\zero-codomain separability} to separate it from $\tau$-codomain separability?}
\begin{definition} [$\tau$-codomain separability]
\label{def:codomain_separability}
Let $f: \ZZZ_K^N \times \Theta \to \mathbb{R}$ be a function. For $\theta \in \Theta$, define $\Lambda_{\theta}(f) := \min_{\sigma_1,\sigma_2 \in \ZZZ_K^N} \abs{f(\sigma_1,\theta) - f(\sigma_2,\theta)}$ to be the minimum difference in the function output keeping $\theta$ fixed. For a fixed $\tau > 0$, we say that $f$ admits \emph{$\tau$-codomain separability} using $\theta$ if $\Lambda_{\theta}(f) \geq \tau$. In particular, we say that $f$ admits \emph{\zero-codomain separability} using $\theta$ if there exists any $\tau > 0$ such that $\Lambda_{\theta}(f) \geq \tau$. 
\end{definition}
% Note that, for a fixed $\theta$, if a function is $\tau$-codomain separable, then it is also $\tau'$-codomain separable for $0 < \tau' < \tau$.
Compared to $\tau$-codomain separability for $\tau >0$, the \zero-codomain separability is weaker as it only requires $\Lambda_{\theta}(f) > 0$. This condition is used for label inference in the unnoised case. As an example for $\tau$-codomain separability, consider the function 
% $f:\{0,1\}^N \times \mathbb{R}^N \to \mathbb{R}$, defined as 
$f(\sigma,\theta) = \langle \sigma, \theta \rangle$ for $\sigma \in \{0,1\}^N$. To demonstrate codomain separability, it suffices to set $\theta = [1,2,4,\dots,2^{N-1}]$
% . Using this, the output $f(\sigma,\theta)$ is the integer whose binary representation (in reverse) is given by the \emph{bits} defined in $\sigma$. Moreover, since the difference between any two integers that can be represented this way is one, it also holds that $\Lambda_\theta(f) = 1$, 
which makes $f$ admit $1$-codomain separability. Multiplying each entry in $\theta$ by $\tau$ will make $f$ admit $\tau$-codomain separability for any $\tau > 0$. In upcoming sections, we discuss our constructions that make many popular loss functions separable. In Appendix~\ref{sec:negative_results}, we present some function classes that are provably not $\tau$-codomain separable.  

% As another example, consider the binary cross-entropy loss from~\eqref{eq:log_loss_defn}. The result \cite[Theorem~5]{aggarwal2020logloss} demonstrates a construction that for any $\tau > 0$ makes this loss $\tau$-codomain separable.



% \begin{theorem} \label{thm:conp}
% \textsc{Codomain-Sep} is co-NP-hard.
% \end{theorem}


% (see Appendix~\ref{app:hardness_results}, where we provide a Karp reduction from the Tautology problem).
 
% Our general goal will be to construct $\theta$'s that allows for separability with larger values of $\tau$ as that translates into label reconstruction attacks that can handle more noise.    
% Depending, on $f$, Note that $f$ may not be codomain separable using some other $\theta\in\Theta$. 
% Furthermore, for $\theta_1, \theta_2 \in \Theta$, each of which makes $f$ codomain separable, the corresponding $\tau$ can be different.

\noindent\textbf{Robust Label Inference.} The goal with robust label inference is to recover the true labeling (in $\ZZZ_K^N$) upon observing only the loss function output, even if noised. Observe that the results trivially hold for the unnoised case if we can handle arbitrary noise levels. 
% A particular focus will be on the binary label case.
%, when the latter is perturbed using some noise.
\begin{definition}[$\tau$-Robust Label Inference]
\label{def:robust_label_inference}
Let $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$ be a function, and $\sigma^\star \in \ZZZ_K^N$ be the (unknown) true labeling. For a given $\tau > 0$, we say that $f$ admits $\tau$-robust label inference if there exists $\theta \in \Theta$ and an algorithm (Turing machine) $\mathcal{A}$ that can recover $\sigma^\star$ given any $\ell \in \mathbb{R}$ where $\abs{f(\sigma^\star,\theta) - \ell} < \tau$, \emph{i.e.,} for all $\sigma^\star \in \ZZZ_K^N$, we have $\mathcal{A}\paran{\theta, N, \ell} = \sigma^\star$.
\end{definition}
% Observe that the above definition can also work for the unnoised case by setting $\tau$ arbitrarily small.
We reiterate an important point to note here that $\tau$-robust label inference requires perfect reconstruction of $\sigma^\star$, which is a {\em stronger} notion than that required by notions like {\em blatant non-privacy}~\citep{dinur2003revealing}, where the goal is to only reconstruct a good fraction of $\sigma^\star$. Also, while the above definition is based on a single query, we later relax this requirement to study robust label inference under a multi-query model.  


The following proposition formally establishes the connection between the above definitions of codomain separability and robust label inference. 
% The proposition is stated for the noised setting (\emph{i.e.} with $\tau > 0$), but also extends to the unnoised setting. 
% For label inferences in the unnoised setting, it suffices that $f$ admits \zero-codomain separability.

\begin{proposition}\label{prop:bound_on_tau_for_label_inference}
For any $\tau>0$, the function $f$ admits $\tau$-robust label inference using $\theta \in \Theta$ iff $\Lambda_{\theta}(f) \geq 2\tau$. 
\end{proposition}

Suppose the adversary picks $\theta \in \Theta$ based on Definition~\ref{def:codomain_separability} and gets back the noisy loss function value $\ell$ from the curator (server). Proposition~\ref{prop:bound_on_tau_for_label_inference} then allows for a natural label inference algorithm (which we call~\LabelInf) which iterates over all possible labelings to recover the one which is closest to the observed loss score:
\begin{align} \label{eq:labelinf}
    \mathbf{\LabelInf:}\;\; \sigma^* \gets \arg\min_{\sigma\in \ZZZ_K^N} \abs{f(\sigma,\theta) -\ell} 
\end{align}
% The algorithm $\mathcal{A}$ (the adversary) has the freedom on choosing $\theta \in \Theta$. The adversary sends a prediction vector $\theta$ to a machine (server) that holds the (private) dataset $\sigma \in \{0,1\}^N$ and gets back the noisy loss function. 
% In the setting where the scores are noised, we assume that the adversary knows an upper bound on the resulting error. Often the former can be inferred from the knowledge of the precision on the machine that returns the loss score to the adversary.
% \abhi{Add details on a general Algorithm for Robust-Label Inference in the $\mathsf{APA}$ model.}
% \renewcommand{\thealgocf}{}
% \SetAlgoCaptionSeparator{}
%       \begin{algorithm}[t]
%         \SetAlgoLined
%         \SetKwInput{KwData}{Input}
%         \SetKwInput{KwResult}{Output}
%         \SetKwInOut{Model}{Model Setting}
%         \KwData{Number of datapoints $N$, bound on error (noise) $\tau > 0$}
%         \KwResult{Recovered labels $\hat{\sigma}$}
%         % \Model{A server (oracle) with private dataset with true labels $\sigma^\star$}
%         \smallskip
%         Design a vector $\theta\in \Theta$ with respect to which $f$ admits $2\tau$-codomain separability (Definition~\ref{def:codomain_separability}).\\
%         Query the server using $\theta$ as the prediction vector and observe output $\ell$ with $\abs{f(\sigma^\star,\theta) - \ell } < \tau$.\\
%          \textbf{Return} $\hat{\sigma} \gets \arg\min_{\sigma\in \ZZZ_K^N} \abs{f(\sigma,\theta) -\ell}$.
%         \caption{\LabelInf: Robust Label Inference for function $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$}
%         \label{alg:general_label_inference}
%         \end{algorithm}
% \begin{remark} \label{rem:first}
A special case of \LabelInf is the unnoised setting, wherein $\ell = f(\sigma^\star,\theta)$. In that case, it suffices to design a vector  $\theta \in \Theta$ with respect to which $f$ admits \zero-codomain separability and $\tau$ plays no role.
% (i.e., can be set to an arbitrarily small positive constant).
% \end{remark}

While intuitive, an important feature about the approach outlined in \LabelInf~\eqref{eq:labelinf} is that it makes just one call to the server to retrieve the (loss) function $f$ evaluated at a single $\theta$, but still reconstructs the entire private vector. However, the exponential time exhaustive search over the space of all labelings makes it impractical. We optimize for this runtime to sub-exponential time (for single query) and polytime time (using multiple-queries) in Section~\ref{sec:linearly_separable}. 
% Even the exponential search is a local computation for the adversary.
% repeat the experiment 1,000 times and the maximum vector length at which 100\% accuracy is achieved is 3 and 1 at noise magnitude 0.0001 and 0.01, which are smaller than 10 and 8 by \LabelInf. When the noise magnitude increases to 0.1 and 1, the randomly generated vector cannot correctly infer label vector even at length 1 with 100\% accuracy.\\}. 
% The following theorem follows from the above discussion.
% \begin{theorem} \label{thm:inf}
% Let $f :\ZZZ_K^N \times \Theta \to \mathbb{R}$ be a loss function. Then, \LabelInf performs $\tau$-robust label inference on $f$, in that it recovers $\sigma^\star$ (i.e., $\hat{\sigma} = \sigma^\star$) from $
% \ell$ where $\abs{f(\sigma^\star,\theta) - \ell } < \tau$.
% \end{theorem}
\vspace{-0.9ex}

\noindent\textbf{Role of Arithmetic Precision.} Our label inference attacks use number theoretic constructions with large integers and products of primes, which can render these attacks impractical to run (within a single query) on limited floating-point precision machines. We begin by observing that Definition~\ref{def:codomain_separability} does not take into account fixed arithmetic precision, which has an effect on separability by placing a bound on the resolution. For example, even if $f(\sigma_1,\theta) \neq f(\sigma_2,\theta)$, this difference may not be observable with only $\phi$ bits of precision,. We extend the notion of codomain separability in the finite precision model in Appendix~\ref{app:apa_fpa}, and present multi-query label inference attacks to recover all labels within fixed precision in Sections~\ref{sec:linearly_separable} and~\ref{sec:experiments}. For simplicity, we focus on inference attacks under arbitrary precision arithmetic in the main body of this paper.

% \LabelInf is also described in the arbitrary precision model. The prediction vectors that we use in our attacks, e.g., say in the multiclass cross-entropy loss in Theorem~\ref{thm:multi_class_proof} contains entries that are doubly-exponential in $N$ (number of  datapoints) and $K$ (number of classes). This would prohibit the correct computation of loss scores beyond some values of $N$ and $K$ in the $\mathsf{FPA}(\phi)$ model. However, this issue could be overcome by the ability to perform multiple queries that we utilize in our experimental evaluation in Section~\ref{sec:experiments}. 



==> AISTATS'22/conclusion.tex <==
In this paper, we demonstrated how a large class of common ML loss functions can be exploited to recover the unknown test labels. Our attacks, based on tools from analytical number theory, succeed with provable guarantees, even when provided with noisy loss function values. Our investigation also highlights the role of number of queries and arithmetic precision. We also demonstrate how our attack could be carried out using a simple augmentation to any neural network model, making it look benign. 
% The observations in this paper provide a deeper understanding of the vulnerabilities inherent in modern machine learning and could be used for designing future trustworthy ML.

%understanding of the vulnerabilities inherent to machine learning, 

% formalized a notion of codomain separability of arbitrary loss functions. Through an equivalence established between this notion and the ability to perform label inference attacks, we characterize necessary and sufficient conditions for label inference from a large class of commonly used loss functions in ML, under arbitrary noise levels. 
% % For defending against such attacks, one could consider differentially private mechanisms for releasing loss scores~\cite{dwork2014algorithmic}, which will ascertain desired levels of plausible deniability on the labels recovered by an adversary. 

% An interesting open question is to study the implications of codomain separability on discrete function optimization (e.g., maximization of functions defined on the space of all labelings $\ZZZ_K^N$). Intuitively, a large separation in the function's output space can be exploited to design algorithms that converge inside a small neighborhood around the global optimum, which may then be recoverable using local search.

==> AISTATS'22/empirical_analysis.tex <==
We now present an empirical evaluation of our label inference attacks. We analyze the following datasets: 
\input{single_query_plot}
\input{plots}
\vspace{-1em}
\begin{CompactItemize}
    \item {\bf{Titanic}}~\citep{titanic}: a binary classification dataset (2201 rows) on the survival status of passengers.
    \item {\bf{IMDB}}~\citep{imdb}: a binary classification dataset (25000 rows) on the movie reviews.
    \item {\bf{Satellite}}~\citep{satellite}: a six-class classification dataset (6430 rows) on the satellite images of soil.
    \item {\bf{MNIST}}~\citep{mnist}: a ten-class classification dataset (70000 rows) on handwritten digits.
    \item {\bf{CIFAR}}~\citep{cifar10}: a ten-class classification dataset (60000 rows) on color images.
    % , fetched from  \url{https://www.openml.org/d/40704}
\end{CompactItemize}
As our attacks construct prediction vectors that are independent of the dataset contents, we ignore the dataset features in our experiments, but all the labels of the dataset are considered for the attack\footnote{All experiments are run on a 64-bit machine with 2.6GHz 6-Core processor, using the standard IEEE-754 double precision format. For reproducibility, the code is included as part of the supplementary material.}. We consider four common loss functions arising from Sections~\ref{sec:linearly_separable} and \ref{sec:logloss}, two of which are multiclass losses (multiclass cross-entropy (\Klogloss~\eqref{eq:multi_class_log_loss}) and softmax cross-entropy~\eqref{eq:softmax}), and the other two are binary losses (binary Itakura-Saito (\textsc{ISLoss}~\eqref{eq:IS}) and sigmoid cross-entropy~\eqref{eq:sigmoid_definition}). 
% For our label inference attacks, we implement both the single query exponential search, \LabelInf~\eqref{eq:labelinf}, and the multi-query polynomial time search outlined in Section~\ref{sec:linearly_separable}.
As a baseline, for the binary labeled dataset (Titanic) with the (plain) cross-entropy loss, we implemented the label inference attack of~\citep{aggarwal2021icml}.
% (see Theorem~\ref{thm:from_icml}, Appendix~\ref{app:experiments} for a restatement of their main result). 
We also present additional experimental results in Appendix~\ref{app:experiments}.

We start with the distinction between our experiments and the approach outlined in \LabelInf, which is presented in the arbitrary precision model.
% \footnote{To baseline \LabelInf with a naive exponential search over the space of all labelings, we simulated label inference on the Titanic dataset (see Section~\ref{sec:experiments}) for the cross-entropy loss, by replacing the prediction vector $\theta$ from Step 1 in \LabelInf by a uniformly random vector in $[0,1]^N$. We observed that over 1000 independent runs, the randomly generated vector failed to correctly infer the true label for even a single datapoint at even mild noise levels ($\tau=0.1$ and higher).}. 
For \Klogloss, simulating \LabelInf on a finite precision machine must be able to differentiate $\min_{i,k}\theta_{i,k}$ from 0 (or else the label inference will be ambiguous). A rough analysis (from Theorem~\ref{thm:multi_class_proof}) gives that 
% $\min_{i,k}\theta_{i,k}\approx \vartheta_{N,1}/\vartheta_{N,K} = 3^{2^{(N-1)K+1}N\tau}/3^{2^{(N-1)K+K}N\tau}=\Omega(3^{-2^{NK}N\tau})$, which requires a precision of 
$\phi=\Omega(2^{NK}N\tau)$ bits are required to make this distinction. This bound hides constant factors, but gives an idea of how arithmetic precision  plays a role in our experiments. 

%\noindent\textbf{Results on (Softmax) Multiclass Cross-Entropy Losses.} 
Figure~\ref{fig:singlequery} shows the number of datapoints $N$ recovered by \LabelInf as we increase the noise for \textsc{ISLoss}, \Klogloss, and  softmax cross-entropy loss. We sample 1000 random sets of labels each of length $N$ from the dataset here. At error magnitude $\tau = 1$, the noise is comparable to the actual loss function values computed. We measure accuracy as the percentage of labels correctly inferred out of $N$.
% (since the largest N for at least 50\% accuracy is 8 for sigmoid and softmax cross-entropy), 
Figure~\ref{fig:singlequery}(a) shows that the number of datapoints ($N$) for which 100\% label inference accuracy is achieved with \textsc{ISLoss} as we vary noise magnitude. As expected at lower noise magnitude the attacks can extract more labels correctly and this quantity decreases as the noise magnitude ($\tau$) increases. Note that as mentioned, our attacks are independent of the dataset feature set, therefore the recovery performance is same on both Titanic and IMDB, as they are both binary labeled.
Figure~\ref{fig:singlequery}(b) shows the number of datapoints ($N$) for which 100\% label inference accuracy is achieved with \Klogloss. Here, the results differ (except for MNIST and CIFAR) because the datasets have different number of classes $K$.
At the same noise magnitude, the accuracy also drops as the number of classes ($K$) increases from 2 (in Titanic) to 10 (in MNIST and CIFAR), which is also expected. These happen because of the dependence on number of datapoints and number of classes in our prediction vector construction (Theorem~\ref{thm:multi_class_proof}), which given fixed machine precision runs into representation issues. 
We note that the construction from~\citep{aggarwal2021icml} on the Titanic dataset (the only case where it is applicable), works slightly better (especially at lower $\tau$ values) than ours due to a small difference in the exponent: it holds that $\min_{i \in [N]}(-\ln \theta_{i}) = \Omega(2^N N\tau)$ in their paper, but $\Omega(2^{2N}N\tau)$ when using Theorem~\ref{thm:multi_class_proof}.
% However, our construction is very general and extends to multiclass cross-entropy loss and beyond, which the construction in~\citep{aggarwal2021icml} does not handle.. 

% Using the prediction vectors from Section~\ref{sec:logloss}, on these 1000 samples of length 8 from Titanic, the mean loss value is 3.64 for cross-entropy, 0.51 for sigmoid cross-entropy, and 0.81 for softmax cross-entropy.

% We further observe that for the Titanic dataset, the construction from~\citep{aggarwal2021icml} works slightly better (especially at lower $\tau$ values) than our construction provided by Theorem~\ref{thm:multi_class_proof}. This is due to a small difference in the exponent: we have $\min_{i \in [N]}\theta_{i} = \Omega(3^{-2^N N\tau})$ in~\citep{aggarwal2021icml} (see Appendix~\ref{app:experiments}), but $\Omega(3^{-2^{2N}N\tau})$ when using Theorem~\ref{thm:multi_class_proof} with $K=2$ (as mentioned above).
% On the other hand our construction is very general and extends to multiclass cross-entropy loss and beyond, which the construction in~\citep{aggarwal2021icml} does not handle.  

Figures~\ref{fig:singlequery}(c)-(d) show the number of datapoints on which \LabelInf achieves at least 50\% accuracy for \Klogloss and softmax cross-entropy losses respectively. We notice this number is smaller for softmax cross-entropy loss, which is also not surprising. Through a similar argument as that above for the number of bits required for cross-entropy loss, one can show that computing the softmax cross-entropy loss will require an additional $\Omega(NK + \ln(N\tau))$ bits (see the discussion in Appendix~\ref{app:experiments} for details). This additional requirement further constraints the number of labels that can be recovered with softmax cross-entropy loss.

We also examine a multi-query label inference algorithm in Figure \ref{fig:multiquery}. For these plots, we simulated \LabelInf on $M < N$ datapoints at a time (instead of all), to obtain a total of $\lceil N/M\rceil$ queries. The idea is to use Figure~\ref{fig:singlequery} to determine the maximum number of labels that can be correctly inferred in a single query for a given noise level, and then perform label inference on only those many datapoints at a time.  As expected, we observed that the accuracy increases with the number of queries: for \textsc{ISLoss} on Titanic, we achieved 100\% accuracy using $M \geq 220$ with $\tau=0.0001$, and $M \geq 1100$ with $\tau = 1$. The accuracy is again lower for the softmax case again due to reasons mentioned above. Additional experimental results on \Klogloss and sigmoid cross-entropy losses are included in Appendix~\ref{app:experiments}.


==> AISTATS'22/introduction.tex <==
Consider a situation where a machine learning (ML) modeler is interacting with a data curator who owns a private dataset for a classification task. The curator agrees to evaluate on this private dataset the prediction vector (or an ML model) that the modeler submits, and replies back with loss function values. Such a situation is commonly encountered in machine learning competition settings like Kaggle~\citep{kaggle}, KDDCup~\citep{kdd_cup}, and ILSVRC Challenges~\citep{ilsvrc}. In some competitions, the features of the private (hold-out) dataset are revealed but not its labels, and the modeler submits the prediction vector on those features. In some other competitions, no information about the private dataset is revealed (i.e., neither the features nor the labels). The modeler submits a model that is then evaluated on the private dataset. 
% In these settings, it is common for the curator to return the loss scores to the modeler (such as for the purposes of fine-turning the models or ranking etc.). 
A similar situation also appears when dealing with sensitive datasets, where either labels, or, both features and labels could be considered sensitive, and a modeler and curator interact through loss scores.

In this paper, we investigate if it is possible for a (malicious) modeler to recover \emph{all} the private labels using these interactions with the data curator (server). More broadly, we investigate the problem of robust label inference, where the goal is to infer the labels of a hidden dataset from only the (noisy) loss function queries evaluated on the dataset. Of particular interest will be the case where the modeler gets {\em just one} loss query output, which could be distorted by noise. Surprisingly, we show that even with just this single query (and no access to the private feature set or any side knowledge), for many common loss functions including general Bregman divergence-based losses and multiclass cross-entropy with common activation functions like sigmoid and softmax, our inference attack succeeds in exactly recovering {\em  all} the labels. This is a stronger privacy violation than that postulated by {\em blatant non-privacy}~\citep{dinur2003revealing}, where the goal is to only reconstruct a good fraction of the true labels. 

Our observations in this paper have important ramifications, for example, when used by an adversary to execute a privacy breach by learning labels associated with a sensitive dataset, or by an unscrupulous participant to an ML competition for learning the unknown test labels. Our results call to attention these vulnerabilities which might be currently under silent exploitation. Armed with this information, individuals and organizations, which vend these seemingly innocuous aggregate metrics from their models can grasp the potential scope of the resulting information leakage.

\noindent\textbf{Overview of Our Results and Techniques.} Our attacks rely on a mathematical notion of {\em codomain separability} of loss functions, which posits that the output of the loss function is \emph{sufficiently} distinct on every possible labeling of the input datapoints (see Definition~\ref{def:codomain_separability}). We assume that the curator that returns the loss scores can add noise to these scores up to some (known) error bound $\tau$. This noise can also be introduced as error when the scores are communicated over noisy channels or computed on low-precision machines\footnote{Our assumptions about the noise generation process ensure that our attacks succeed irrespective of the noise process used by the data curator. Knowledge about the noise distribution can be helpful though. For random noise, by first generating a bound on the noise using a tail bound, our techniques can be applied.}. As one would expect, separating the loss function outputs by more than $2\tau$ is a necessary and sufficient condition for this label recovery to be accurate (see Proposition~\ref{prop:bound_on_tau_for_label_inference}). While intuitive, this result gives a natural candidate for label inference, from just one loss query, using an exhaustive (exponential) local search (see~\LabelInf~\eqref{eq:labelinf}). 

% Using,  The runtime can be made also present a scheme search runtime can be made su
% We discuss some caveats associated with using this approach on machines with finite floating point precision. We also  runtime using analytical properties of squarefree integers (see Section~\ref{sec:label_inference_linear}). 

Throughout this paper, we assume that the adversary knows the loss function, number of datapoints $N$ and an upper bound $\tau$ on the resulting error (noise). We also assume that the loss is computed on all the datapoints. The main technical challenge here is to design prediction vectors for which a loss function demonstrates the required codomain separability to handle arbitrary noise levels. Our key idea here is to use sets with distinct subset sums. Two simple examples of such sets of size $n$ are $\{1,2,4,\dots,2^{n-1}\}$ and $\{\ln p_1, \dots, \ln p_n\}$, where $p_1,\dots,p_n$ are distinct primes. Sets like these are useful when characterizing the sufficient conditions under which the required codomain separability can be achieved. For example, in the binary classification setting with $N$ datapoints, the following problem comes up often in our analysis: $\text{Construct $\theta = [\theta_1,\dots,\theta_N]$ such that}$ 
\begin{align*}
\ \min_{\sigma_1,\sigma_2 \in \{0,1\}^N}\abs{\sum_{i:\sigma_1(i)=1}g(\theta_i) - \sum_{j:\sigma_2(j)=1}g(\theta_j)} \geq b,    
\end{align*}
for some function $g$ and bound $b$. To satisfy this inequality, it suffices to set $\theta$ such that the set $g(\theta) := \{g(\theta_i),\dots,g(\theta_N)\}$ has all distinct subset sums. This is because the summation operators essentially filter out subsets of elements from the vector $\theta$, and because $\sigma_1 \neq \sigma_2$ in the minima operator, these subsets must differ in at least one element. Now, to ensure that the minimum difference of the subset sums in $g(\theta)$ is at least $b$, one can solve for $g(\theta_i) = 2^ib$ or $g(\theta_i) = b\ln p_i$ (or using some other set with distinct subset sums) depending on actual form of $g$ and the application.










We use these ideas and tools from analytical number theory to provide constructions of adversarial prediction vectors for broad classes of ML loss functions based on Bregman divergences (Section~\ref{sec:linearly_separable}) and multiclass cross-entropy (Section~\ref{sec:logloss}), for both the unnoised and the noised setting. The analytical properties of squarefree integers also helps us to reduce the computation time needed by the adversary.
% In the unnoised setting, the adversary gets the true loss function score, whereas in the noised setting, the adversary only gets the loss function score within an absolute error bound. 
In addition to the single query model where the adversary has to work with only one (noisy) loss function value, we also analyze extensions where the adversary has access to multiple (noisy) loss function values from different prediction vectors. This extension comes in handy as with sufficient queries the local computation time required at the adversary becomes polynomial. Additionally, to handle situations an actual ML model is required (and not just the prediction vector), we provide a construction of a feed-forward neural network, which can be used to carry out these label inference attacks while making them look benign (see Section~\ref{sec:neural_network}). We also point out some caveats associated with our approaches on machines with finite floating point precision.

% Together, these constructions call to attention these vulnerabilities which might be currently under silent exploitation. Armed with this information, individuals and organizations, which vend these seemingly innocuous aggregate metrics from their classification models, can grasp the potential scope of the resulting information leakage. 

% Together, these constructions characterize the vulnerability of loss functions in leaking private information about the ground truth labels, which we empirically verify in Section~\ref{sec:experiments}. 


% \noindent\textbf{Central Idea.} 
% % admit this property and generalize our constructions to special classes of functions . 
% % We show that this problem is co-NP-Hard in general through a Karp reduction from the Tautology problem (see Appendix~\ref{app:hardness_results}).
% % However, when achieved, this property ensures that the true labeling can be unambiguously recovered from the loss scores. We also discuss cases where this separability (and hence, label inference) is not achievable (see Appendix~\ref{sec:negative_results} for such classes of loss functions). 
% %  Under the mild assumption that this bound is known, we show how the true labeling can now be recovered from the loss scores.  We simulate (and formally analyze) both single-query and multi-query algorithms for label inference. 
% At the onset, the fact that we can recover the true labels just from these quite different and highly non-linear loss functions might sound surprising. To make these attacks succeed,
% our main algorithmic approach 



\noindent\textbf{Defenses.} Our focus in this paper is on characterizing the vulnerability of loss functions in leaking private information. Viewed from this perspective, our results establishes lower bounds on the amount of noise needed (as a function of precision, number of queries, etc) on releasing these loss functions for any {\em reasonable notion} of label privacy. A rigorous defense mechanism against our proposed attack would be to release the loss scores under on differential privacy~\citep{dwork2006calibrating} with carefully calibrated noise that overcomes this lower bound. This will ascertain desired levels of plausible deniability on the labels recovered by an adversary.

We also highlight that in general, determining whether a loss function is codomain separable is co-NP-hard (Theorem~\ref{thm:conp}). We establish this through a (polynomial time) Karp reduction from the {\em Almost Tautology} problem from Boolean satisfiability theory (see Appendix~\ref{app:hardness_results}). Based on standard consensus on the complexity of this class of problems, it is unlikely that there is a general polynomial time algorithm for robust label inference from loss functions~\citep{arora2009computational}.

% For defending against such attacks, one could consider differentially private mechanisms for releasing loss scores~\cite{dwork2014algorithmic}, which will ascertain desired levels of plausible deniability on the labels recovered by an adversary. 


\noindent\textbf{Related Work.} Label inference attacks were first introduced in~\citep{whitehill2018climbing} for binary log-loss using a heuristic solution to a min-max optimization problem. This attack does not recover all the labels and works only in the unnoised setting. The noised setting for binary log-loss was recently studied by~\citep{aggarwal2021icml}. While their approach was not formalized using codomain separability, their construction also used the idea of making the loss function outputs distinct for each labeling of the dataset using distinct subset sums. However, their algorithm runs in exponential time and works only in the unnoised setting for the multiclass case. Furthermore, they also restrict only to cross-entropy loss. Our paper not only subsumes these results, but also significantly extends them by showing that most commonly used loss functions in ML applications are vulnerable to leaking private information about the ground truth labels. Moreover, we provide single query sub-exponential time and multi-query polynomial time attacks that can be carried out through benign looking ML models and settle the computational complexity of robust label inference from arbitrary loss functions.\footnote{
% An alternate view of our results can be seen through the lens of information theory. In the standard channel coding problem, the goal is to construct a coding scheme (in our case, the prediction vector) that takes a message (true labels), passes it though a noisy channel (loss function), to produce an output which is then used to infer the message (label inference mechanism). A standard coding theory goal is to have a high minimum distance between the codewords (separability). Our idea for using sets with distinct subset sums in our construction is motivated by 
Our approach is also reminiscent of similar concepts used in information theory, e.g., coding schemes based on Sidon sequences~\citep{o2004complete} and Golomb rulers~\citep{robinson1967class}, where the goal is to have a high minimum distance between the codewords.}.

% In addition to covering the case of multiclass cross-entropy with noise, we examine cross-entropy with various activation functions and Bregman divergence-based losses that are common in ML applications.

% For attacks on leaderboards, such as in Kaggle competitions,~\citep{blum2015ladder} demonstrate an adversarial boosting attack, where the adversary observes loss scores on randomly generated prediction vectors to generate a labeling which, with probability $2/3$, gives a low loss score. Our focus on the other hand is on exact label recovery, especially in the noised setting.

% For attacks on leaderboards, such as in Kaggle competitions,~\citep{blum2015ladder} demonstrates an adversarial boosting attack, in which the adversary observes loss scores on randomly generated prediction vectors to generate a labeling which, with probability $2/3$, gives a low loss score. Our focus, on the other hand is on a different problem on exact label recovery, especially in the noised setting. 

 

% \noindent\textbf{Paper Organization.} \abhi{Add here.} \shiva{not sure this is needed}


% Our results call to attention these vulnerabilities which might be currently under silent exploitation. Armed with this information, individuals and organizations, which vend these seemingly innocuous aggregate metrics from their classification models, can grasp the potential scope of the resulting information leakage.

% \subsection{Overview of Our Results}
% \input{overview}

==> AISTATS'22/linearly_separable.tex <==
\vspace{-0.5em}
Our main focus in this paper is on an important class of (binary) loss functions, which we refer to as \emph{linearly-decomposable}. These functions can be expressed as a sum of two terms: one dependent on the true labeling $\sigma$, and the other only on the prediction vector $\theta$. As we will see, this decomposition allows for an efficient construction of prediction vectors for robust label inference from such functions. We present only our main ideas here and defer all missing details to Appendix~\ref{app:linearly_separable}.

\begin{definition}
\label{def:linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function. We say that a binary loss function $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ is linearly-decomposable if there exists some invertible function $g:[0,1] \to \mathbb{R}$ and some function $h:[0,1]^N \to \mathbb{R}$, such that:
\vspace{-0.5em}
\begin{align}
    \label{def:sqfree_linearly_separable}
    f(\sigma,\theta) &= h(\theta) + \sum_{i=1}^N \sigma_i g(\theta_i) = h(\theta) + \sum_{i:\sigma_i=1} g(\theta_i).
\end{align}
\end{definition}
\vspace{-0.5em}
This class of functions includes many commonly used loss functions in the ML literature. For example, all Bregman divergence-based binary loss functions satisfy the linear-decomposability property.
\begin{lemma}
\label{lem:bregman_is_linear}
Let $F:[0,1] \times [0,1] \to \mathbb{R}$ be a strongly convex function and $D_F(p,q) = F(p) - F(q) - \langle \nabla F(q),p - q\rangle$ be the Bregman divergence associated with $F$. Then, the corresponding loss function, defined as $f_F(\sigma,\theta) = \frac{1}{N}\sum_{i=1}^N D_F\paran{[\sigma_i,1-\sigma_i],[\theta_i,1-\theta_i]}$, is linearly-decomposable. 
\end{lemma}
Unlike the distance metrics for probability distributions, Bregman divergences does not require its inputs to be necessarily distributions~\citep{bregman1967relaxation}. To use these divergences as loss functions, we directly compare the outputs of the ML model with the point distribution from the ground truth labels, as we do in the definition of $f_F(\sigma,\theta)$ (similar to~\citep{liu2016clustering}). 

We also focus on a special class of linearly-decomposable functions for which the linear split is based purely on the labels: one term corresponding to datapoints with true label $0$, and the other for datapoints with true label $1$. More formally, if $g:[0,1] \to \mathbb{R}$ is some deterministic function, then we say that a binary loss function $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ is $g$-linearly-decomposable if it can be expressed as follows:
\begin{align}
\label{eq:linear_separable}
f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i:\sigma_i=1} g(\theta_i) + \sum_{i:\sigma_i=0} g(1-\theta_i)}.    
\end{align}
In many cases, as we will see, functions in this sub-class are easier to analyze for codomain separability.
% It follows directly from the equation above that all $g$-linearly decomposable functions are also linearly decomposable per Definition~\ref{def:linear_separable}. 
Observe that the KL-divergence loss (which reduces to binary cross-entropy or log-loss) is of this form, using $g(\theta_i) = -\ln \theta_i$. Some other
common examples of $g$-linearly-decomposable loss functions include the (i) Itakura-Saito divergence based loss, which uses $g(\theta_i) = 1/\theta_i + \ln \theta_i - 2$; (ii) Squared Euclidean loss, which can be expressed using $g(\theta_i) = (1-\theta_i)^2$; and, (iii) norm-like loss, which uses $g(\theta_i) = 1 + (\alpha-1)\theta_i^\alpha - \alpha \theta_i^{\alpha-1} + (\alpha-1)(1-\theta_i)^\alpha$ for some $\alpha \ge 2$. We provide detailed constructions for robust label inference from these particular loss functions in Appendix~\ref{app:linearly_separable}.

\vspace{-0.5em}
\subsection{Establishing Codomain Separability}
\vspace{-0.5em}
As argued in Section~\ref{sec:prelim}, the first step for label inference is to design prediction vectors using which the loss functions are sufficiently codomain-separable. We provide two different constructions of such prediction vectors for linearly-decomposable functions. Each construction uses a different set with distinct subset sums to ensure that the loss scores are in 1-1 correspondence with the set of all possible labelings. The first construction uses powers of 2, which follows naturally from the requirement of the $2\tau$ separation needed for $\tau$-robust label inference (as in Proposition~\ref{prop:bound_on_tau_for_label_inference}). We analyze multiple loss functions using this construction. Our second construction uses a set consisting of (log) primes, which enables us to perform robust label inference in sub-exponential time using results from number theory. We discuss these constructions in detail below.
% \shiva{say something about the pros of the two constructions}






\noindent\textbf{Construction 1:} As mentioned above, our first construction is based on the fact that the set $S_m = \{1,2,4,\dots,2^m\}$ has distinct subset sums. To see this, observe that each subset sum in $S_m$ is an integer whose binary representation (in reverse) is given by the \emph{bits} defined by the indices of elements contained in that subset. Moreover, since the difference between any two integers that can be represented this way is one, it also holds that the minimum subset sum difference is 1. Scaling each element of $S_m$ also scales the minimum difference as needed. The theorem below states our main result from this construction.
\begin{theorem}
\label{thm:linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is $g$-linearly-decomposable. Then, for any $\tau > 0$, the function $f$ is $2\tau$-codomain separable if there exists $\theta \in (0,1)^N$ so that $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$. If $\tau=0$, then setting $g(\theta_i) - g(1-\theta_i) > 0$ for all $i \in [N]$ suffices for \zero-codomain separability.
\end{theorem}

Based on this theorem, the prediction vectors can be constructed as follows: (1) Compute $x^*(y)$ as the solution to $g(x)-g(1-x) = y$; (2) If $x^*(y)$ exists, then set $\theta_i = x^*(2^iN\tau)$ for all $i \in [N]$. This vector $\theta$ can now be used for $\tau$-robust label inference from $f$ using~\LabelInf (see Section~\ref{sec:experiments} for our empirical analysis using this construction). The following corollaries follow for specific loss functions such as Itakura-Saito divergence loss, squared Euclidean, and norm-like divergence losses (see detailed proofs in Appendix~\ref{app:linearly_separable}). For simplicity, we discuss only the unnoised case in Corollary~\ref{cor:eucl}, for which it suffices to demonstrate \zero-codomain separability.

% \shiva{explain why such a $\theta$ might not exist for all loss functions, and why the \zero-codomain separability always exists?}

\begin{corollary} \label{cor:IS}
The Itakura-Saito divergence loss is $2\tau$-codomain separable with $\theta_i = (1+3^{2^{i}N\tau})^{-1}$.
\vspace*{-0.25em}
\end{corollary}

% However, such a $\theta$ might not exist for all loss functions, e.g., it does not exist for squared Euclidean and norm-like divergence losses, and we will deal those loss functions later. It does exist though for the Itakura-Saito divergence loss (defined in~\eqref{eq:IS}, Appendix~\ref{app:bregman}).
% mentioned earlier can satisfy the required condition in Theorem~\ref{thm:linear_separable} on $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$.


% \noindent\textbf{Linearly-Decomposable Functions Not Covered by Theorem~\ref{thm:linear_separable}.} We now deal with linearly-decomposable functions for whom there exists no $\theta$ that could satisfy the condition required in Theorem~\ref{thm:linear_separable} (examples include, squared Euclidean and norm-like divergence loss). Here, we establish the weaker \zero-codomain separability, which as discussed earlier suffices for label inference in the unnoised case. 

\begin{corollary} \label{cor:eucl}
The squared Euclidean loss  is \zero-codomain separable using $\theta_i = (1/2)\paran{1-\ln(p_i)/N}$, where $p_i$ is the $i$th prime number for $i \in [N]$. The norm-like divergence loss for $\alpha \geq 2$ is \zero-codomain separable using $\theta$ that satisfies $(1-\theta_i)^{\alpha-1}-\theta_i^{\alpha-1} = (\ln p_i)/(N\alpha)$.
\end{corollary}

% \begin{theorem}
% \label{thm:zero_codomain_linear_separable}
% Let $g:[0,1] \to \mathbb{R}$ be some deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Let $\theta \in (0,1)^N$ be some vector and $S_\theta = \{g(\theta_i) - g(1-\theta_i)\}_{i=1}^N$. Then, the function $f$ is \zero-codomain separable with respect to $\theta$ if $\mu(S_\theta)>0$, i.e., all subset sums in the set $S_\theta$ are distinct.
% \end{theorem}
% Finally, the idea behind the multi-query attack mentioned in Theorem~\ref{thm:multi_query_general} also extends to loss functions covered by Theorem~\ref{thm:zero_codomain_linear_separable}, thus, providing a multi-query polynomial time inference here as well. 

% \subsection{Optimizing Robust Label Inference using Square Free Prime Factorization}
\noindent\textbf{Construction 2:} Our main motivation for this second construction is to infer all labels within sub-exponential time. Starting from Definition~\ref{def:sqfree_linearly_separable}, we can
% express the minimum codomain separation in $f$ (given a prediction vector $\theta$) in a way that obviates the connection to distinct subset sums: 
% $$\Lambda_\theta(f) = \min_{\sigma_1 \ne \sigma_2} | \sum_{i:\sigma_1(i)=1} g(\theta_i) - \sum_{i:\sigma_2(i)=1} g(\theta_i)|.$$
% We can now analyze for robust label inference (given some bound $\tau > 0$ on the error) by selecting the elements of the set $g(\theta) := \{g(\theta_1),\dots,g(\theta_N)\}$ in a way that it has distinct subset sums and that the minimum difference of these subset sums is at least $2\tau$ (using Proposition~\ref{prop:bound_on_tau_for_label_inference}). While there are many ways in which $g(\theta)$ can be constructed (for example, using powers of 2, as was done in Theorem~\ref{thm:linear_separable}),
ensure $\Lambda_\theta(f) \geq 2\tau$ (as is needed for $\tau$-robust label inference from Proposition~\ref{prop:bound_on_tau_for_label_inference}) by setting $g(\theta_i) = 3P\tau  \ln p_i$ (if possible to do so within the domain of $g$), where $p_i$ is the $i^{th}$ prime number and $P=\prod_{i=1}^N p_i$. This particular choice of $g(\theta_i)$ ensures that each subset sum in the set $g(\theta)$ corresponds to the logarithm of a unique integer (using its prime factorization), and leads to the desired codomain separation as follows.
\begin{theorem}
\label{thm:linearly_decomposable_using_primes}
Let $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable (Definition~\ref{def:sqfree_linearly_separable}). Let $p_i$ is the $i^{th}$ prime number and $P=\prod_{i=1}^N p_i$, is the product of the first $N$ primes. Then, for any $\tau > 0$, setting $g(\theta_i)=3P\tau  \ln p_i$ for loss functions in Equation~\ref{def:sqfree_linearly_separable} ensures that $\Lambda_\theta(f) \geq 2\tau$. If $\tau=0$, setting $g(\theta_i)=\ln p_i$ suffices for \zero-codomain separability.
\end{theorem}
We will now see how this choice of prime-based vector entries enable efficient label inference for any given $\tau$.
\vspace{-0.5em}
\subsection{Establishing Robust Label Inference}
\label{sec:label_inference_linear}
\vspace{-0.5em}
We discuss three approaches to recover the ground truth labels from the (perturbed) loss score obtained on prediction vectors we just designed. We distinguish each approach based on its runtime complexity and number of queries made to the server.

\noindent\textbf{Exponential Time Single-Query Inference.} The first approach is discussed in \LabelInf~\eqref{eq:labelinf}, which iterates over all $2^N$ possible labelings to find the one that is closest to the observed loss score. Both constructions 1 and 2 ensure that this algorithm always returns the true labeling within a single query to the server.

\noindent\textbf{Sub-Exponential Time Single-Query Inference.} To avoid the exhaustive search as above, we first substitute the prediction vector from Construction 2 in the expression for the loss function to obtain $f(\sigma,\theta) = h(\theta) + 3P\tau \ln \paran{\prod_{i:\sigma_i = 1}p_i}$.
Now, we know that due to codomain separation, the labeling that minimizes the distance between the observed loss $\ell$ and the true loss $f(\sigma,\theta)$ above is the true labeling $\sigma^*$:
\begin{align*}
    \sigma^* &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\ell - \paran{h(\theta) + 3P\tau \ln \paran{\prod_{i:\sigma_i = 1}p_i}}} \\
    % &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\parfrac{\ell - h(\theta)}{3P\tau} - \ln \paran{\prod_{i:\sigma_i = 1}p_i}}\\
    % &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\ln \parfrac{\exp\parfrac{\ell - h(\theta)}{3P\tau}}{\prod_{i:\sigma_i = 1}p_i}}\\
    &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\exp\parfrac{\ell - h(\theta)}{3P\tau} - \paran{\prod_{i:\sigma_i = 1}p_i}}.
\end{align*}

To obtain $\sigma^*$ from the equation above without using an exhaustive search over $\{0,1\}^N$, we observe that the expression inside the argmin essentially seeks a \emph{square-free} integer closest to some known real quantity. An integer is said to be squarefree if it has no repeated prime factors. This can be checked using the Booker-Hiary-Keating algorithm from~\citep{Booker_2015} in sub-exponential time. Once such an integer is obtained, its prime factors are in 1-1 correspondence with the indices in $\sigma^*$ that have label $1$. 
\vspace{-0.5em}
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
\begin{algorithm}[ht]
\caption{\textsc{CloSqFree}$(x,m)$}\label{alg:closest_square_Free}
If $x \leq 2$ or $m=2$, then \textbf{return} 2.

Let $p_i$ be the $i^{th}$ prime number. If $p_1\cdots p_m \leq x$, then \textbf{return} $p_1\cdots p_m$.

\For{$k=0,1,2,\dots,\lfloor x \rfloor-1$}{
If $\lfloor x \rfloor - k \in \textsc{SqFree}(m)$, then \textbf{return} $\lfloor x \rfloor - k$.

If $\lceil x \rceil + k \in \textsc{SqFree}(m)$, then \textbf{return} $\lceil x \rceil + k$.
}
\end{algorithm}
%\footnote{Strictly speaking, the Booker-Hiary-Keating algorithm relies on the validity of the Generalized Reimann Hypothesis for Dirichlet L-functions to avoid integer factorization.}
% \vspace{-0.5em}
The problem of label inference on linearly-decomposable loss functions is, thus, reduced to the calculation of the nearest square-free integer to a given real number. More concretely, the expression for recovering the true labeling can be written as follows:
$$\sigma^* = \left\{i: p_i\text{ divides }\textsc{CloSqFree}\paran{e^{\frac{\ell - h(\theta)}{3P\tau}},N}\right\},$$
where $\textsc{CloSqFree}(x,m) = \arg\min_{y \in \textsc{SqFree}(m)} |x-y|$ denotes the closest squarefree integer to $x$. The notation $\textsc{SqFree}(m)$ denotes the set of all square free integers whose largest prime factor is at most the $m^{th}$ prime number $p_m$. We outline an optimized version of $\textsc{CloSqFree}$ in Algorithm~\ref{alg:closest_square_Free}, which runs in $O(N\exp\paran{(\ln N)^{O(1)}})$ time. 

% Recall that a positive integer $M$ is square-free if it doesn't have any repeated prime factors. Extending this definition, we say that $M$ is $n$-square-free if $M$ is square free and the largest prime factor of $M$ is at most $n^{th}$ prime number $p_n$. For example, $105 = 3 \times 5 \times 7$ is 4-square-free, since the largest prime factor of 105 is the 4$^{th}$ prime number (7), but it is not 3-square-free. We denote by $\textsc{SqFree}(m) = \{x:\text{$x$ is $m$-square-free}\}$ to be the set of all $m$-square-free positive integers. We denote the closest m-square-free number to $x$ as follows: 
% $$\textsc{CloSqFree}(x,m) = \arg\min_{y \in \textsc{SqFree}(m)} |x-y|.$$ 




% \begin{algorithm}[t!]
% \caption{Sub-Exponential Time Robust Label Inference for Linearly-Decomposable Loss Functions}
% \label{alg:linearly_separable}
% \vspace{0.5em}
% \KwInput{$N$: number of datapoints, $\tau$: error bound}
% \KwOutput{Labeling $\hat{\sigma} \in \{0,1\}^N$}
% \vspace{0.5em}
% Set $\theta_i \gets g^{-1}(3P\tau \ln p_i)$ (assuming the inverse exists), where $p_i = i^{th}$ prime and $P=p_1p_2\cdots p_N$.

% Obtain the loss score $\ell$ using the vector $\theta$.

% Let $A \gets \textsc{CloSqFree}\paran{\exp\paran{\frac{\ell - h(\theta)}{3P\tau}},N}$.

% For $i\in [N]$, set $\hat{\sigma}_i \gets 1$ if $p_i$ divides $A$, else $\hat{\sigma}_i \gets 0$.

% \textbf{Return} $\hat{\sigma}$ as the labeling.

% \end{algorithm}
% \shiva{Cite the Algo in the paper}

\noindent\textbf{Multi-Query Polynomial Time Attacks.} 
Loss functions that are $g$-linearly-decomposable also allow for an efficient multi-query label inference algorithm. In particular, we could have a trade-off between the ability to perform  multiple queries with faster computation times for solving the optimization problem in \LabelInf~\eqref{eq:labelinf}. 
% As noted in Section~\ref{sec:prelim}, whereas the optimization problem in \LabelInf can be naively solved using an exponential search over $\sigma$. 
To see this, observe that setting $\theta_i = 1/2$ gives $g(\theta_i) - g(1-\theta_i) = 0$. Thus, if we want to infer the first $M < N$ labels in a single query, we can set $\theta = [\theta_1,\dots,\theta_M,1/2,\dots,1/2]$, where 
% to obtain: 
% % so that the following holds:
% % \begin{align*}
% %     f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i\leq M: \sigma(i)=1} (g(\theta_i)-g(1-\theta_i)) + \sum_{i=1}^M g(1-\theta_i) + \frac{(N-M)g(1/2)}{M}}.
% % \end{align*}
% % From this, we immediately obtain that:
% \begin{multline*}
%         \Lambda_\theta(f) = \frac{1}{N} \min_{\sigma_1,\sigma_2} |\sum_{i\leq M:\sigma_1(i)=1}\paran{g(\theta_i)-g(1-\theta_i)}    \\ 
%     - \sum_{j\leq M:\sigma_2(j)=1}\paran{g(\theta_j)-g(1-\theta_j)}|.
% \end{multline*}
$\theta_1,\dots,\theta_M$ are produced according to either Constructions 1 or 2. Using this $\theta$ will ensure that if $f(\sigma_1,\theta) = f(\sigma_2,\theta)$, then $\sigma_1[:M] = \sigma_2[:M]$.
% Similar to Theorem~\ref{thm:linear_separable}, choosing $\theta_i$ that ensures $g(\theta_i)-g(1-\theta_i) > 2^iN\tau$ will ensure $\Lambda_\theta(f) > 2\tau$. Moreover, using this $\theta$ will ensure that if $f(\sigma_1,\theta) = f(\sigma_2,\theta)$, then $\sigma_1[:M] = \sigma_2[:M]$ must hold.
After recovering the first $M$ labels, we can recover the next $M$ labels using $\theta = [1/2,\dots,1/2,\theta_{M+1},\dots,\theta_{2M},1/2,\dots]$, and so on. 
% \shiva{Removed Thereom 4}

% \input{neurips2021/single_query_plot}
% \begin{theorem}
% \label{thm:multi_query_general} 
% Let $g:[0,1] \to \mathbb{R}$ be some finite deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable using $g$. Then, for $\tau > 0$ and integer $M \geq 1$, a sufficient condition for $f$ to admit $\tau$-robust label inference with $\lceil N/M \rceil$ queries is for the inequality $g(x) - g(1-x) > 2^iN\tau$ to have a solution for all $i \in [N]$. Similarly, if 
% % there exist $x_1,\dots,x_M \in (0,1)$ such that $g(x_i) - g(1-x_i) > 2^iN\tau$ for all $i \in [M]$.
% \end{theorem}
Observe that an $\lceil N/M \rceil$-query algorithm for robust label inference will require $O(N2^M/M)$ local computations by the adversary (using \LabelInf~\eqref{eq:labelinf} in each query). Thus, while the single query case required $O(2^N)$ computations, any multi-query algorithm using $M=O(\log N)$ requires only $O(\text{poly}(N))$ time.

==> AISTATS'22/linearly_seperable_copy.tex <==
We begin our analysis with the discussion of an important class of (binary) loss functions, which we refer to as \emph{linearly-decomposable}. Loss functions in this class can be expressed as a sum of two terms: one corresponding to the datapoints that have label $1$ and the other for the datapoints with label $0$. As we will see, this decomposition allows an efficient construction of prediction vectors for robust label inference from such functions. We refer the reader to Appendix~\ref{app:linearly_separable} for missing proofs and technical details from this section.

\begin{definition}
\label{def:linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function. We say that a binary loss function $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ is linearly-decomposable in $\{0,1\}^N$ using $g$ if it can be expressed as follows:
\begin{align}
\label{eq:linear_separable}
f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i:\sigma_i=1} g(\theta_i) + \sum_{i:\sigma_i=0} g(1-\theta_i)}.    
\end{align}
\end{definition}

Observe that the KL-divergence loss (which reduces to binary cross-entropy loss) is of this form, using $g(\theta_i) = -\ln \theta_i$, which allows our results to subsume those presented by~\citep{aggarwal2021icml}. Some other
common examples of linearly-decomposable loss functions include the (i) Itakura-Saito divergence based loss, which can be expressed using $g(\theta_i) = 1/\theta_i + \ln \theta_i - 2$; (ii) squared Euclidean loss, which can be expressed using $g(\theta_i) = (1-\theta_i)^2$; and, (iii) norm-like divergence loss, which can be expressed using $g(\theta_i) = 1 + (\alpha-1)\theta_i^\alpha - \alpha \theta_i^{\alpha-1} + (\alpha-1)(1-\theta_i)^\alpha$ for some $\alpha \ge 2$. These loss functions are some popular instances of the general class of
Bregman divergence-based loss functions. The following lemma shows a general result that all Bregman divergence-based loss functions will satisfy this linearly-decomposability property.
\begin{lemma}
\label{lem:bregman_is_linear}
Let $F:[0,1] \times [0,1] \to \mathbb{R}$ be a strongly convex function and $D_F(p,q) = F(p) - F(q) - \langle \nabla F(q),p - q\rangle$ be the Bregman divergence associated with $F$. Let $f_F(\sigma,\theta)$ be the corresponding loss function, defined as follows:
$$f_F(\sigma,\theta) = \frac{1}{N}\sum_{i=1}^N D_F\paran{[\sigma_i,1-\sigma_i],[\theta_i,1-\theta_i]}.$$
Then, $f_F(\sigma,\theta)$ is linearly-decomposable. 
\end{lemma}
Note that unlike the distance metrics for probability distributions, Bregman divergence does not require its inputs to be necessarily distributions~\citep{bregman1967relaxation}. Thus, to use these divergences as loss functions (as is common, e.g.,~\citep{liu2016clustering}) one can directly compare the outputs of the ML model with the point distribution from the ground truth labels as we do in the definition of $f_F(\sigma,\theta)$. 



% ~\citep{bregman1967relaxation}We defer the details on our general result for $\tau$-codomain separability on Bregman divergence, including that for the Mahalanobis divergence loss (which is not linearly-decomposable) to Appendices~\ref{app:bregman} and~\ref{app:breg_general}. We also prove that the class of linearly-decomposable functions also contains all Bregman divergence based losses (see Appendix~\ref{sec:bregman_decomposable}).



\subsection{Establishing Codomain Separability}

\begin{theorem}
\label{thm:linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Then, for any $\tau > 0$, the function $f$ is $2\tau$-codomain separable if there exists $\theta \in (0,1)^N$ so that $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$.
\end{theorem}

Observe that Theorem~\ref{thm:linear_separable} immediately allows constructing a vector that will make a given linearly-decomposable function $f$ admit $\tau$-codomain separability for a given $\tau > 0$: (1) Compute $x^*(y)$ as the solution to $g(x)-g(1-x) = y$; (2) If $x^*(y)$ exists, then set $\theta_i = x^*(2^iN\tau)$ for all $i \in [N]$. This vector $\theta$ can now be used for $\tau$-robust label inference from $f$ using Algorithm~\LabelInf. However, such a $\theta$ might not exist for all loss functions, e.g., it does not exist for squared Euclidean and norm-like divergence losses, and we will deal those loss functions later. It does exist though for the Itakura-Saito divergence loss (defined in~\eqref{eq:IS}, Appendix~\ref{app:bregman}).
% mentioned earlier can satisfy the required condition in Theorem~\ref{thm:linear_separable} on $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$.
\begin{corollary} \label{cor:IS}
The Itakura-Saito divergence loss is $2\tau$-codomain separable with $\theta_i = (1+3^{2^{i}N\tau})^{-1}$.
\end{corollary}

\noindent\textbf{Linearly-Decomposable Functions Not Covered by Theorem~\ref{thm:linear_separable}.} We now deal with linearly-decomposable functions for whom there exists no $\theta$ that could satisfy the condition required in Theorem~\ref{thm:linear_separable} (examples include, squared Euclidean and norm-like divergence loss). Here, we establish the weaker \zero-codomain separability, which as discussed earlier suffices for label inference in the unnoised case. 

% \noindent\textbf{A Note on the \zero-Codomain Separability of Linearly-Decomposable Functions.} Observe that in Theorem~\ref{thm:linear_separable}, the condition on the function $g$ has a linear dependence on $\tau$, which will not suffice for label inference in the un-noised setting (where $\tau=0$). We state the result for this special case in the Theorem below\footnote{Note that while it is true that any vector with respect to which a function is $\tau$-codomain separable (for $\tau>0$) also allows \zero-codomain separability, we mention Theorem~\ref{thm:zero_codomain_linear_separable} to cover cases where $\tau$-codomain separability is hard to demonstrate (see the discussion about Norm-Like loss following the statemnt of Theorem~\ref{thm:zero_codomain_linear_separable}).} and show how it can be used to achieve \zero-codomain separability for the Square-Euclidean loss and the Norm-Like loss. 

\begin{theorem}
\label{thm:zero_codomain_linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Let $\theta \in (0,1)^N$ be some vector and $S_\theta = \{g(\theta_i) - g(1-\theta_i)\}_{i=1}^N$. Then, the function $f$ is \zero-codomain separable with respect to $\theta$ if $\mu(S_\theta)>0$, i.e., all subset sums in the set $S_\theta$ are distinct.
\end{theorem}
\begin{corollary} \label{cor:eucl}
The squared Euclidean loss  is  \zero-codomain separable using $\theta_i = (1/2)\paran{1-\ln(p_i)/N}$, where $p_i$ is the $i$th prime number for $i \in [N]$. The norm-like divergence loss for $\alpha \geq 2$ is \zero-codomain separable using $\theta$ that satisfies $(1-\theta_i)^{\alpha-1}-\theta_i^{\alpha-1} = (\ln p_i)/(N\alpha)$.
\end{corollary}
Finally, the idea behind the multi-query attack mentioned in Theorem~\ref{thm:multi_query_general} also extends to loss functions covered by Theorem~\ref{thm:zero_codomain_linear_separable}, thus, providing a multi-query polynomial time inference here as well. 

\subsection{Optimizing Robust Label Inference using Square Free Prime Factorization}

Our approach for $\tau$-robust label inference in this section will be to first demonstrate $2\tau$-codomain separability (as before), and then reduce the reconstruction of the true labels from noised loss score (using the separating prediction vector) to computing the closest square free integer of some real value. This algorithm runs in sub-exponential time, which is much faster than Algorithm~\LabelInf that uses exhaustive search. The main steps of our construction are provided in Algorithm~\ref{alg:linearly_separable} and outlined as follows.

Observe that any loss function of the form $f(\theta,\sigma) = \sum_{i=1}^N \paran{\sigma_i g(\theta_i) + (1-\sigma_i)h(\theta_i)}$ can be rewritten as $f(\theta,\sigma) = \Sigma_{i=1}^N \sigma_i g'(\theta_i) + \sum_{i=1}^N h(\theta_i)$, where $g'(\theta_i) = g(\theta_i)-h(\theta_i)$. For this section, we will generalize Definition~\ref{def:linear_separable} slightly to say that a loss function $f: \{0,1\}^N \times [0,1]^N \to \mathbb{R}$ is said to be linearly-decomposable if there exists some invertible function $g:[0,1] \to \mathbb{R}$ and some function $h:[0,1]^N \to \mathbb{R}$, such that we can write:
\begin{align}
    \label{def:sqfree_linearly_separable}
    f(\sigma,\theta) &= h(\theta) + \sum_{i=1}^N \sigma_i g(\theta_i) = h(\theta) + \sum_{i:\sigma_i=1} g(\theta_i).
\end{align}
This reformulation not only extends to a larger set of loss functions than those covered by Definition~\ref{def:linear_separable}, but also allows us to express the minimum codomain separation in $f$ (given a prediction vector $\theta$) in a way that obviates the connection to distinct subset sums:
\begin{align}
\label{eq:sqfree_min_separation}
    \Lambda_\theta(f) = \min_{\sigma_1 \ne \sigma_2}\abs{\sum_{i:\sigma_1(i)=1} g(\theta_i) - \sum_{i:\sigma_2(i)=1} g(\theta_i)}.
\end{align}
We can now analyze for robust label inference (given some bound $\tau > 0$ on the error) by selecting the elements of the set $g(\theta) := \{g(\theta_1),\dots,g(\theta_N)\}$ in a way that it has distinct subset sums and that the minimum difference of these subset sums is at least $2\tau$ (using Proposition~\ref{prop:bound_on_tau_for_label_inference}). While there are many ways in which $g(\theta)$ can be constructed (for example, using powers of 2, as was done in Theorem~\ref{thm:linear_separable}), we choose to set $g(\theta_i) = 3P\tau  \ln p_i$ (if possible to do so within the domain of $g$), where $p_i$ is the $i^{th}$ prime number and $P=\prod_{i=1}^N p_i$, is the product of the first $N$ primes. This particular choice of $g(\theta_i)$ ensures that each subset sum in the set $g(\theta)$ corresponds to the logarithm of a unique integer (using its prime factorization). 
\begin{lemma}
\label{lem:linearly_decomposable_using_primes}
Let $p_i$ is the $i^{th}$ prime number and $P=\prod_{i=1}^N p_i$, is the product of the first $N$ primes. Then, for any $\tau > 0$, setting $g(\theta_i)=3P\tau  \ln p_i$ for loss functions in Equation~\ref{def:sqfree_linearly_separable} ensures that $\Lambda_\theta(f) \geq 2\tau$. 
\end{lemma}
\begin{proof}
We prove this by substituting $g(\theta_i) = 6P\tau \ln p_i$ in Equation~\ref{eq:sqfree_min_separation} as follows:
\begin{align*}
    \Lambda_\theta(f) &= \min_{\sigma_1 \ne \sigma_2}\abs{\sum_{i:\sigma_1(i)=1} g(\theta_i) - \sum_{j:\sigma_2(j)=1} g(\theta_j)}\\
    &= (3P\tau)\ \min_{\sigma_1 \ne \sigma_2}\abs{\sum_{i:\sigma_1(i)=1} \ln p_i - \sum_{j:\sigma_2(j)=1} \ln p_j}\\
    &= (3P\tau)\ \min_{\substack{S_1,S_2 \subseteq [N]\\S_1 \cap S_2 = \emptyset}} \abs{\ln \parfrac{\prod_{i \in S_1}p_i}{\prod_{s \in S_2}p_j}} \geq 2\tau.
\end{align*}
Too see why the last inequality holds, let $S_1^*$ and $S_2^*$ denote the sets of primes that achieve the minimum value above. Then, without loss of generality, it must hold that $\prod_{j \in S_2^*}p_j \leq P$ and $\prod_{j \in S_2^*}p_j \leq 1 + \prod_{i \in S_1^*}p_i$. Thus, using the fact that $1.5x\ln \parfrac{1+x}{x} > 1$ for all $x \geq 1$, we obtain that $1.5P$ times the log expression above is at least $1$. Further scaling by $2\tau$ gives $\Lambda_\theta(f) \geq 2\tau$.
\end{proof}

Now that we have the desired codomain separation needed for $\tau$-robust label inference\footnote{For the unnoised case ($\tau$=0), a similar argument to that in Lemma~\ref{lem:linearly_decomposable_using_primes} can be used to show that $g(\theta_i)=\ln p_i$ suffices.}, we demonstrate how our choice of $g(\theta_i)$ in this section allows for label inference in sub-exponential time. To see this, we simplify the expression for the loss function as follows:
\begin{align*}
    f(\sigma,\theta) = h(\theta) + 3P\tau \ln \paran{\prod_{i:\sigma_i = 1}p_i}.
\end{align*}
We know that due to codomain separation, the labeling that minimizes the distance between the observed loss $\ell$ and the true loss $f(\sigma,\theta)$ above is exactly the ground truth labeling $\sigma^*$:
\begin{align*}
    \sigma^* &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\ell - \paran{h(\theta) + 3P\tau \ln \paran{\prod_{i:\sigma_i = 1}p_i}}} \\
    &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\parfrac{\ell - h(\theta)}{3P\tau} - \ln \paran{\prod_{i:\sigma_i = 1}p_i}}\\
    &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\ln \parfrac{\exp\parfrac{\ell - h(\theta)}{3P\tau}}{\prod_{i:\sigma_i = 1}p_i}}\\
    &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\exp\parfrac{\ell - h(\theta)}{3P\tau} - \paran{\prod_{i:\sigma_i = 1}p_i}}.
\end{align*}

To obtain $\sigma^*$ from the equation above without using an exhaustive search over $\{0,1\}^N$, we observe that the expression inside the argmin essentially seeks a \emph{square-free} integer closest to some known real quantity. Once such an integer is obtained, its prime factors are in 1-1 correspondence with the indices in $\sigma^*$ that have label $1$. The problem of label inference on linearly-decomposable loss functions is, thus, reduced to the calculation of the nearest square-free integer to a given real number, which we discuss as follows. We use the Booker-Hiary-Keating algorithm from~\citep{Booker_2015} for checking square-freeness of integers in sub-exponential time\footnote{Strictly speaking, the Booker-Hiary-Keating algorithm for checking square-freeness of integers relies on the validity of the Generalized Reimann Hypothesis for Dirichlet L-functions to relax the dependence on integer factorization~\citep{Booker_2015}.}.

Recall that a positive integer $M$ is square-free if it doesn't have any repeated prime factors. Extending this definition, we say that $M$ is $n$-square-free if $M$ is square free and the largest prime factor of $M$ is at most $n^{th}$ prime number $p_n$. For example, $105 = 3 \times 5 \times 7$ is 4-square-free, since the largest prime factor of 105 is the 4$^{th}$ prime number (7), but it is not 3-square-free. We denote by $\textsc{SqFree}(m) = \{x:\text{$x$ is $m$-square-free}\}$ to be the set of all $m$-square-free positive integers. We denote the closest m-square-free number to $x$ as follows: 
$$\textsc{CloSqFree}(x,m) = \arg\min_{y \in \textsc{SqFree}(m)} |x-y|.$$ 

\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}

\begin{algorithm}[t]
\caption{\textsc{CloSqFree}$(x,m)$}\label{alg:closest_square_Free}
\vspace{0.5em}
If $x \leq 2$ or $m=2$, then \textbf{return} 2.

Let $p_i$ be the $i^{th}$ prime number. If $x < p_i$ for some $i > 1$, then \textbf{return} \textsc{CloSqFree}$(x,i-1)$.

If $p_1\cdots p_m \leq x$, then \textbf{return} $\lfloor x \rfloor$.

\For{$k=0,1,2,\dots,\lfloor x \rfloor-1$}{
If $\lfloor x \rfloor - k \in \textsc{SqFree}(m)$, then \textbf{return} $\lfloor x \rfloor - k$.

If $\lceil x \rceil + k \in \textsc{SqFree}(m)$, then \textbf{return} $\lceil x \rceil + k$.
}
\end{algorithm}

\begin{algorithm}[t]
\caption{Sub-Exponential Time Robust Label Inference for Linearly-Decomposable Loss Functions}
\label{alg:linearly_separable}
\vspace{0.5em}
\KwInput{$N$: number of datapoints, $\tau$: error bound}
\KwOutput{Labeling $\hat{\sigma} \in \{0,1\}^N$}
\vspace{0.5em}
Set $\theta_i \gets g^{-1}(3P\tau \ln p_i)$ (assuming the inverse exists), where $p_i = i^{th}$ prime and $P=p_1p_2\cdots p_N$.

Obtain the loss score $\ell$ using the vector $\theta$.

Let $A \gets \textsc{CloSqFree}\paran{\exp\paran{\frac{\ell - h(\theta)}{3P\tau}},N}$.

For $i\in [N]$, set $\hat{\sigma}_i \gets 1$ if $p_i$ divides $A$, else $\hat{\sigma}_i \gets 0$.

\textbf{Return} $\hat{\sigma}$ as the labeling.

\end{algorithm}

\subsection{Multi-Query Polynomial Time Attacks} 
The linear-decomposability of $f$ allows for an efficient multi-query label inference algorithm for $f$. In particular, we could have a trade-off between the ability to perform  multiple queries with faster computation times for solving the optimization problem solved in Step 3 of Algorithm~\LabelInf. 
% As noted in Section~\ref{sec:prelim}, whereas the optimization problem in Algorithm~\LabelInf can be naively solved using an exponential search over $\sigma$. 
To see this, observe that setting $\theta_i = 1/2$ gives $g(\theta_i) - g(1-\theta_i) = 0$. Thus, if we want to infer the first $M < N$ labels in a single query, we can set $\theta = [\theta_1,\dots,\theta_M,1/2,\dots,1/2]$ to obtain: 
% so that the following holds:
% \begin{align*}
%     f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i\leq M: \sigma(i)=1} (g(\theta_i)-g(1-\theta_i)) + \sum_{i=1}^M g(1-\theta_i) + \frac{(N-M)g(1/2)}{M}}.
% \end{align*}
% From this, we immediately obtain that:
\begin{multline*}
        \Lambda_\theta(f) = \frac{1}{N} \min_{\sigma_1,\sigma_2} |\sum_{i\leq M:\sigma_1(i)=1}\paran{g(\theta_i)-g(1-\theta_i)}    \\ 
    - \sum_{j\leq M:\sigma_2(j)=1}\paran{g(\theta_j)-g(1-\theta_j)}|.
\end{multline*}

Similar to Theorem~\ref{thm:linear_separable}, choosing $\theta_i$ that ensures $g(\theta_i)-g(1-\theta_i) > 2^iN\tau$ will ensure $\Lambda_\theta(f) > 2\tau$. Moreover, using this $\theta$ will ensure that if $f(\sigma_1,\theta) = f(\sigma_2,\theta)$, then $\sigma_1[:M] = \sigma_2[:M]$ must hold.  Note that after recovering the first $M$ labels, we can recover the next $M$ labels using $\theta = [1/2,\dots,1/2,\theta_{M+1},\dots,\theta_{2M},1/2,\dots,1/2]$, and so on. The result below immediately follows.

% \input{neurips2021/single_query_plot}

\begin{theorem}
\label{thm:multi_query_general} 
Let $g:[0,1] \to \mathbb{R}$ be some finite deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable using $g$. Then, for $\tau > 0$ and integer $M \geq 1$, a sufficient condition for $f$ to admit $\tau$-robust label inference with $\lceil N/M \rceil$ queries is for the inequality $g(x) - g(1-x) > 2^iN\tau$ to have a solution for all $i \in [N]$.
% there exist $x_1,\dots,x_M \in (0,1)$ such that $g(x_i) - g(1-x_i) > 2^iN\tau$ for all $i \in [M]$.
\end{theorem}
Observe that an $\lceil N/M \rceil$-query algorithm for robust label inference will require $O(N2^M/M)$ local computations by the adversary (using Algorithm~\LabelInf in each query). Thus, while the single query case ($M = N$) required $O(2^N)$ computations, any multi-query algorithm using $M=O(\log N)$ requires only $O(\text{poly}(N))$ local computations, which allow a polynomial-time robust label inference.

% \subsection{Bregman Divergence Loss Functions are Linearly Decomposable}
% \label{sec:bregman_is_linearly_decomposable}
% \input{bregman}

==> AISTATS'22/log_loss_analysis.tex <==
We now show that the ideas of codomain separability also extend to the particular case of
multiclass cross-entropy loss and its variants. 
% The results in this section answers an open question from~\citep{aggarwal2020logloss} about label inference attacks from noisy multiclass cross-entropy loss evaluations. 
% We start with establishing $\tau$-codomain separability for multiclass cross-entropy loss and its variants, for any $\tau > 0$. This implies that for these loss functions, Algorithm~\LabelInf succeeds in recovering all the labels when the loss scores are noised by less than $\tau$ in magnitude.
We provide an overview of our results and defer all missing details to Appendix~\ref{app:logloss}. 
% This extends the results in~\citep{aggarwal2021icml}, where $\tau$-robust label inference in the binary case ($K=2$) was discussed. 
% Missing details from this section are collected in Appendix~\ref{app:logloss}.
% it is possible to design a prediction vector such that the multiclass cross-entropy loss scores differ by more than $2\tau$ on any two distinct labelings. Therefore, one could Algorithm~\LabelInf to perform 
% We begin by explaining the intuition behind our construction and then provide a formal proof of correctness. We also discuss how to generalize this approach to commonly used variants of the cross-entropy loss. We will end this section with a discussion around the computational hardness of label reconstruction for such losses, and show that this problem is in EXPTIME.

\noindent\textbf{Multiclass Cross-Entropy Loss.} We first recall the definition of multiclass cross-entropy.
We assume $K \geq 2$ classes, and let $N$ and $\ZZZ_{K}$ denote the number of datapoints and the set of label classes, respectively. The $K$-ary cross-entropy loss on $\theta$ with respect to a labeling $\sigma \in \ZZZ_{K}^N$ is defined as follows:
	\begin{align}
	\label{eq:multi_class_log_loss}
		\Klogloss\paran{\sigma, \theta} := \frac{-1}{N}\sum_{i=1}^N \sum_{k=0}^{K-1} \ \Big([\sigma_i = k] \cdot \ln \theta_{i,k} \Big),
	\end{align}
 where $[\sigma_i = k] = 1$ if $\sigma_i = k$ and $0$, otherwise.
Here, $\theta \in \Theta = [0,1]^{N \times K}$ is a matrix of prediction probabilities, where the $i$th row is the vector of prediction probabilities $\theta_{i,0},\dots,\theta_{i,K-1}$ (with $\sum_{k \in \ZZZ_K} \theta_{i,k} = 1$) for the $i$th datapoint on classes $0,\dots,K-1$ respectively. 

With this definition, we can now describe our construction of a matrix $\theta \in [0,1]^{N \times K}$ that makes $\Klogloss$ function $2\tau $-codomain separable for any $\tau >0$ (i.e., $\Lambda_{\theta}(\Klogloss) \geq 2 \tau $). At a high level, we obtain the required codomain separability for $\Klogloss$ by splitting the loss into label dependent and independent terms, and designing the entries in the matrix $\theta$ in such a way that the expression reduces to a distinct integer in some set. This calibration allows us to control the minimum difference in the output of the cross-entropy loss on different labelings, which we can scale to the desired amount ($\geq 2\tau$) easily. The following theorem summarizes our construction.  
% (see the Appendix for a detailed proof). 
% \shiva{can we add $\tau = 0$ to this theorem ....}
\begin{theorem}\label{thm:multi_class_proof}
Let $\tau > 0$. Define matrices $\vartheta, \theta \in \mathbb{R}^{N \times K}$ such that $\vartheta_{n,k} = 3^{\paran{2^{(n-1)K+k}N\tau}}$ and $\theta_{n,k} = \vartheta_{n,k} / \sum_{k=1}^K \vartheta_{n,k}$. Then, it holds that $\Klogloss$ is $2 \tau $-codomain separable using $\theta$. If $\tau = 0$, then using $\vartheta_{n,k} = 3^{\paran{2^{(n-1)K+k}}}$ ensures \zero-codomain separability.
\end{theorem}
Using Theorem~\ref{thm:multi_class_proof} and Proposition~\ref{prop:bound_on_tau_for_label_inference} implies that for these cross-entropy loss functions, the approach outlined in~\LabelInf~\eqref{eq:labelinf} succeeds in recovering all the labels when the loss scores are noised by less than $\tau$ in magnitude. We bring to the reader's attention the doubly-exponential nature of the entries used to construct the prediction vector in Theorem~\ref{thm:multi_class_proof}. This blowup is unfortunately unavoidable for constructing $\tau$-codomain separability, even for the binary case (see \citep[Theorem~7]{aggarwal2021icml}).


\noindent\textbf{Extensions of Cross-Entropy Loss.} Often in practice, when using the cross-entropy loss to assess the performance of ML models (like CNNs), it is common to apply an activation function (such as softmax or sigmoid) before the cross-entropy loss calculation. For example, a common idea in multiclass classification is to apply the softmax function (to convert any sequence of real outputs into a probability distribution) as:
\begin{align} \label{eq:softmax}
 \frac{-1}{N}\sum_{i=1}^N \sum_{k=0}^{K-1} \ \Big([\sigma_i = k] \cdot \ln \textsc{softmax}(\theta_{i,k}) \Big),
\end{align}
where $ \textsc{softmax}(\theta_{i,k}) = \exp(\theta_{i,k})/\sum_{j=1}^K \exp(\theta_{i,j})$.
% For example, a common idea in multiclass classification is to apply the softmax function (to convert any sequence of real outputs into a probability distribution),
% % $\textsc{Softmax}:\mathbb{R}^K \to [0,1]^K$, that modifies any vector $\mathbf{v} = (v_1,\dots,v_K) \in \mathbb{R}^K$ using the transformation $v_i \mapsto \exp(v_i)/\sum_{j=1}^K \exp(v_j)$. 
% % This leads to the softmax cross-entropy loss, $\textsc{Softmax-K-LLoss}:\ZZZ_K^N \times \mathbb{R}^{N \times K} \to \mathbb{R}$, 
% defined as follows for $\sigma \in \ZZZ_K^N$, $\theta \in [0,1]^{N \times K}$:
% \begin{align*}
%  \frac{-1}{N}\sum_{i=1}^N \sum_{k=0}^{K-1} \ \Big([\sigma_i = k] \cdot \ln \textsc{softmax}(\theta_{i,k}) \Big), \mbox{ where } 
%  \textsc{softmax}(\theta_{i,k}) = \exp(\theta_{i,k})/\sum_{j=1}^K \exp(\theta_{i,j}).
% \end{align*}
To extend Theorem~\ref{thm:multi_class_proof} to this setting, we do the following: (1) Let $\theta \in [0,1]^{N \times K}$ be the matrix from Theorem~\ref{thm:multi_class_proof}. 
% Recall that by definition, $\theta$ is such that for each $i \in [N]$, the vector $\theta_i \in [0,1]^K$ is a probability distribution; 
(2) For each $i \in [N]$, solve the following (fully specified) system of equations for $\theta'_{i,k}$'s: for all $k \in \ZZZ_K , i \in [N]$: $\exp\paran{\theta'_{i,k}}/\sum_{j=1}^K \exp\paran{\theta'_{i,j}} = \theta_{i,k}$.
% \begin{align}
% \exp\paran{\theta'_{i,k}}/\sum_{j=1}^K \exp\paran{\theta'_{i,j}} = \theta_{i,k}.    
% \end{align}
% This is a system of linear equations in the variables $\exp\paran{\theta'_{i,j}}$, for each $i \in [N]$, hence, can be solved in polynomial time using standard techniques.
Once $\theta'$ is obtained, since $\textsc{softmax}(\theta'_{i,k}) = \theta_{i,k}$, from Theorem~\ref{thm:multi_class_proof}, we get that softmax cross-entropy loss is $2\tau $-codomain separable using $\theta'$. A similar argument also works for Sigmoid cross entropy loss (Appendix~\ref{app:logloss}).

% the approach outlined in \LabelInf~\eqref{eq:labelinf} can now be used for $\tau$-label inference.



% The former compresses arbitrary reals into the range $(0,1)$, while the latter can convert any sequence of real outputs into a probability distribution.
% The outputs from the model do not necessarily represent probability distributions. In such cases, transformations are applied to these outputs before they can be fed into the cross-entropy loss computation. 


==> AISTATS'22/neural_network.tex <==
The results in previous sections highlight how prediction vectors ($\theta$'s) could be generated that succeed with $\tau$-robust label inference. 
% Typically, these prediction vectors are output of a ML model, and in many scenarios (e.g., ML contests held by Kaggle and other platforms) the submission to the server is not the prediction vector but rather the ML model itself. 
This raises an interesting question of whether the prediction vectors utilized in these label inference attacks can actually be an output of a non-trivial benign looking ML model? We answer this question in the affirmative in this section.

\noindent\textbf{Setup.} Assume a classification problem on $K$ classes.
We will design a multi-layer feed-forward neural network $\textsc{MutNet}$ using following specifications.
% for which we have a . We will assumethe following specifications for $\textsc{MutNet}$: 
(1) The input to $\textsc{MutNet}$ is a vector $\mathbf{v} \in \mathbb{R}^{d_1}$ with true label $\sigma_\mathbf{v} \in \ZZZ_K$.   (2) The output of $\textsc{MutNet}$ is a vector in $ (0,1)^{d_2}$ that represents an encoding of the prediction. 
% (3) $\textsc{MutNet}$ has a  series of linear transformations $M_1,\dots,M_3$ and bias vectors $\mathbf{b}_1,\dots,\mathbf{b}_m$ such that:
% \begin{align}
% \label{eq:forward_prop}
%     \mathbf{u}_1   = \mathbf{v}, \quad \forall k\in [m]\ \ \mathbf{u}_{k+1} = h\paran{\mathbf{u}_{k}^\top M_k + \mathbf{b}_k},
% \end{align}
% where $h$ is an activation function (e.g., the sigmoid function, or the ReLU function). 
% The output of this network is, therefore, $\mathbf{z} := \mathbf{u}_{m+1}$. 
% which represents the ground truth corresponding to $\mathbf{v}$ (using some binary representation of the objects in $\mathcal{D}$)
Let $f: \ZZZ_K \times (0,1)^{d_2} \to \mathbb{R}$ be a  loss function.  % Consequently, when this loss is observed (after possible noising) by the adversary on its input, it uses \LabelInf to infer the ground truth labeling for that input. 
% We assume an oracle access to loss function $f:\{0,1\}^{d_2} \times (0,1)^{d_2} \to \mathbb{R}$, evaluated at $(\sigma_v,\mathbf{u}_{m+1})$. As before, it suffices to get a noisy evaluation of this loss function. 
% on Since $\sigma_v$ is unknown, we assume an oracle access to a loss function computed on $\mathbf{z}$ and $\sigma$. 
% Our task is to design the matrices $M_1,\dots,M_m$ such that the network $\textsc{MutNet} = (M_1,\dots,M_m)$ allows recovering, for any input $\mathbf{v}$, the ground truth $\sigma_\mathbf{v}$  through only one query to the oracle. We show that this is possible for any codomain separable loss function that the oracle computes. 
% Our network is composed of two parts. 
The goal of the network is to ensure that on any input $\mathbf{v}$ the network generates an output $\mathbf{u}_{m+1}$ such that $f$ admits $2\tau$-codomain separability using $\mathbf{u}_{m+1}$. Consequently, for any input $\mathbf{v}$, given a noisy value of $f(\sigma_{\mathbf{v}},\mathbf{u}_{m+1})$, an adversary can use \LabelInf to infer~$\sigma_{\mathbf{v}}$.

% \shiva{explain why a trivial network that only outputs $\mathbf{u}_{m+1}$ does not suffice? why take this trouble?}\abhi{True. I was thinking from the point of making the neural network arbitrarily large so its benign. But I see your point. I am open to just mentioning the ReLU construction here, which suffices to prove our point I think.}

% The main steps in our construction are as follows:
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\textwidth]{neurips2021/neural_schematic.png}
%     \caption{Caption}
%     \label{fig:neural_schematic}
% \end{figure}

\noindent\textbf{Our Mutator Network.} We construct a 2-layer network $\textsc{MutNet}_{\mathbf{x}}:\mathbb{R}^{d_1} \to (0,1)^{d_2}$ that can convert any real vector $\mathbf{v} \in \mathbb{R}^{d_1}$ into any desired fixed vector $\mathbf{x} \in (0,1)^{d_2}$. The transformations we use in this network are the \textsc{ReLU} and \textsc{Sigmoid} activation functions: one layer of the former and one layer of the latter. Let $M_1\in \mathbb{R}^{d_1 \times d_1}$ and $M_2 \in \mathbb{R}^{d_1 \times d_2}$ be matrices such that all entries in $M_1$ are negative (the entries in $M_2$ can be arbitrary). Let $\mathbf{x}'$ be a vector such that $x'_i = \ln x_i/(1 - x_i)$. Then, for an input vector $\mathbf{u}_1 = \mathbf{v}$, the transformations in $\textsc{MutNet}_{\mathbf{x}}$ are as follows:
$% \label{eq:mutator}
% \centering
   \mathbf{u}_2 = \textsc{ReLU}\paran{\mathbf{v}^\top M_1},\ \mathbf{u}_3 = \textsc{Sigmoid}\paran{\mathbf{u}_2^\top M_2 + \mathbf{x}'}
$, where $\textsc{ReLU}$ and $\textsc{Sigmoid}$ are applied element-wise on their input vectors. Effectively, this construction inhibits the propagation of $\mathbf{v}$ by outputting the same vector $\mathbf{u}_3 = \mathbf{x}$ always.
By setting $\mathbf{x}$ to the desired (prediction vector) $\theta$ for $2\tau$-codomain separability on $f$, we get that $\abs{f(\sigma_\mathbf{v},\textsc{MutNet}_\theta(\mathbf{v})) - \ell} \leq \tau$ (Theorem~\ref{thm:nn}).
% The following lemma  establishes the correctness of this transformation:
% \begin{lemma}
% Let $\mathbf{x} \in (0,1)^{d_2}$ be fixed. Then, for any $\mathbf{v} \in \mathbb{R}^{d_1}$, the output of $\textsc{MutNet}_{\mathbf{x}}$ equals $\mathbf{x}$.
% \end{lemma}
% \noindent\textbf{Part 2: Rest of the Network.} 
% % Observe that it suffices to ensure that the output of our construction $\mathbf{z}$ is such that it makes the loss function computed by the oracle is codomain separable. 
% The second part of the network takes $\mathbf{u}_4$ and generates a $\mathbf{u}_{m+1}$ that makes $f(\sigma_\mathbf{v},\mathbf{u}_{m+1})$ $2\tau$-codomain separable, where $\tau$ is error bound on the loss function evaluation. To achieve this, we work backwards from a desired target $\mathbf{u}_{m+1}$ and derive conditions on the network and the value of $\mathbf{u}_4$ that makes it possible. Firstly, we set  $h$ in~\eqref{eq:forward_prop} as the \textsc{Sigmoid} activation, and exploit its one-one correspondence to invert~\eqref{eq:forward_prop}. In other words, if the output of the $k^{th}$-layer ($k \geq 4$) is $\mathbf{u}_{k+1} \in (0,1)^{d_2}$, then the output from one layer before $\mathbf{u}_{k} \in (0,1)^{d_2}$ can be obtained by solving the following system of equations: 
% \begin{align}
% \label{eq:back_prop_attack}
%     \mathbf{u}_{k} M_{k} = \textsc{Sigmoid}^{-1}(\mathbf{u}_{k+1}) - \mathbf{b}_k,
% \end{align}
% where $\textsc{Sigmoid}^{-1}:x \mapsto \ln \paran{x/(1-x)}$ is performed element-wise on its input and is well defined. By constructing $\mathbf{b}_k \in \mathbb{R}^{d_2}$ such that $\textsc{Sigmoid}^{-1}(\mathbf{u}_{k+1}) - \mathbf{b}_k \in (0,1)^{d_2}$ and setting $M_{k} \in \mathbb{R}^{d_2 \times d_2}$ such that $\|M_{k}\|_2 \leq 1/\sqrt{d_2}$, we ensure that $\mathbf{u}_{k} \in (0,1)^{d_2}$ is a unique solution to~\eqref{eq:back_prop_attack}.
% \shiva{explain the $\|M_{k}\|_2 \leq 1/\sqrt{d_2}$ condition?} \abhi{To ensure that $\mathbf{u}_{k} \in (0,1)^{d_2}$. If $M_k$ has a large norm, then the solution to (7) can have $\mathbf{u}_{k}$ which may not be within $(0,1)^{d_2}$.}
% % solving for $\mathbf{u}_4$, gives the 
% % The value of $\mathbf{u}_4$ generated from here is used to design t the $\textsc{MutNet}_{\mathbf{x}}$
% \noindent\textbf{Putting it all together.} 
% We given the end-to-end construction in Algorithm~\imitNet. The mutator network is designed to always output the desired value of $\mathbf{u}_4$ (on all inputs), that when propagated through the second part of the network generated the desired $\mathbf{u}_{m+1}$. The result follows.  
% We can now give an end-to-end construction for a neural network that will produce a vector $\theta\in (0,1)^{d_2}$ such that the loss computed the oracle is $2\tau$-separable using $\theta$. 
% Consequently, when this loss is observed (after possible noising) by the adversary on its input, it uses \LabelInf to infer the ground truth labeling for that input. 
% We outline these steps 

% \begin{theorem}
% \label{thm:imit_net_correctness}
% % Let $\tau \geq 0$ be a bound on the noise and $f:\{0,1\}^{d_2} \times (0,1)^{d_2} \to \mathbb{R}$. 
% % Let $ be any loss function for which there exists a vector with respect to which $f$ is $2\tau_{\text{max}}$-codomain separable. 
% % Then, for any integer $m \geq 4$, 
% Algorithm~\imitNet returns an $m$-layer neural network whose output is a prediction vector with respect to which $f$ is $2\tau_{\text{max}}$-codomain separable. 
% % that allows $\tau$-robust label inference. 
% % Here, $f$-oracle refers to an oracle that computes the loss using the function $f$ on the prediction vector and the true labeling.

% % In other words, if $\textsc{MutNet} \gets \imitNet (\tau_{\text{max}})$, then for any vector $\mathbf{v} \in \mathbb{R}^{d_1}$, the function $f$ is $2\tau_{\text{max}}$-codomain separable with respect to $\textsc{MutNet}(\mathbf{v})$.
% \end{theorem}
% Combining this with Theorem~\ref{thm:inf} gives the following result.
% \begin{theorem} \label{thm:nn}
% Let $\tau > 0$ and let $\theta \in (0,1)^{d_2}$ be such that $f:\ZZZ_K \times (0,1)^{d_2} \to \mathbb{R}$ is $2\tau$-codomain separable using $\theta$. Then, for any input $\mathbf{v} \in (0,1)^{d_2}$, given $\ell$ such that $\abs{f(\sigma_\mathbf{v},\textsc{MutNet}_\theta(\mathbf{v})) - \ell} \leq \tau$, the approach outlined in~\LabelInf~\eqref{eq:labelinf} recovers $\sigma_\mathbf{v}$.
% \end{theorem}
\begin{remark}
We note that  any neural network model can be modified to carry out our attack, as an adversary can replace the top layer of any neural network model with the above construction. This highlights the versatility of our attack.
\end{remark}



% \begin{algorithm}[t]
%         \SetAlgoLined
%         \SetKwInput{KwData}{Input}
%         \SetKwInput{KwResult}{Output}
%         \SetKwInOut{Model}{Model Setting}
%         \KwData{Bound on error (noise) $\tau > 0$}
%         \KwResult{Neural network $\textsc{Net}_f:\mathbb{R}^{d_1} \to (0,1)^{d_2}$ (with $d_1 \geq d_2$)}
%         \Model{Oracle access to the loss function $f$ on the server with true labelings.}
        
%         \smallskip
        
%         Let $\theta \in (0,1)^{d_2}$ be a vector such that $f$ is $2\tau$-codomain separable with respect to $\theta$.\\
        
%         % Set $\mathbf{z}_{m+1} \gets \theta$.\\
        
%         % \For{$i = m,m-1,\dots,4$}{
%         %     Let $\mathbf{w}_i \gets \textsc{Sigmoid}^{-1}(\mathbf{u}_{i+1})$ (element-wise).\\
%         %     Let $\mathbf{b}_i \in \mathbb{R}^{d_2}$ be such that $\mathbf{w}_i - \mathbf{b}_i \in (0,1)^{d_2}$.\\
%         %     Let $M_{i} \gets \mathbb{R}^{d_2 \times d_2}$ be a full rank matrix with norm $\|M_{i}\|_2 \leq 1/\sqrt{d_2}$.\\
            
%         %     Let $\mathbf{u}_{i}$ be the solution to the system of equations $\mathbf{u}_i M_i = \mathbf{w}_i - \mathbf{b}_i$.\\
%         %     Let $\mathcal{T}_i$ denote the transformation $\mathbf{z} \mapsto \textsc{Sigmoid}\paran{\mathbf{z}^\top M_i + \mathbf{b}_i}$ (element-wise).
%         % }
        
%         Set $M_1,M_2\in (-\infty,0)^{d_1 \times d_1}$ and $M_3 \in \mathbb{R}^{d_1 \times d_2}$ arbitrarily.\\
        
%         For $j \in \{1,2\}$, define the transformation $\mathcal{T}_j$ as the map $\mathbf{z} \mapsto \textsc{ReLU}\paran{\mathbf{z}^\top M_j}$ (element-wise).\\
        
%         Define the transformation $\mathcal{T}_3$ as the map $\mathbf{z} \mapsto \textsc{Sigmoid}\paran{\mathbf{z}^\top M_3 + \theta}$ (element-wise).\\
        
%         Let $\textsc{Net}_f(\mathbf{z})$ denote the map $\mathbf{z} \mapsto \mathcal{T}_3 \circ \mathcal{T}_2 \circ \mathcal{T}_1 (\mathbf{z})$.\\
        
%         \textbf{Return} $\textsc{Net}_f$.
%         \caption{\imitNet: Network to generate prediction vectors for robust label inference}
%         \label{alg:imitation_network}
%         \end{algorithm}


==> AISTATS'22/neurips2021/codomain_intro.tex <==
We begin our discussion by formally defining the notion of codomain separability and its connections to the problem of label inference in the noised and unnoised settings (missing details in Appendix~\ref{app:prelim}). 
% We defer all missing details from this section to the Appendix~\ref{app:prelim}.  

Our objects of interest are functions whose domain is the Cartesian product of the space of all labelings (defined by the  $\ZZZ_K^N = \ZZZ_K \times \dots \times \ZZZ_K \ \text{($N$ times)} = \{0,\dots,K-1\}^N$) and an arbitrary set $\Theta \subseteq \mathbb{R}^N$. Here, $K \geq 2$ represents the number of label classes.
% , for e.g., in the binary case $K =2$. 
This formulation captures the common scenario in machine learning, where we evaluate a loss function using the true labeling in $\ZZZ_K^N$ for $N$ datapoints based on a (prediction) vector in $\mathbb{R}^N$ generated by an ML model. $\Theta$ is the space of prediction vectors, and for $\theta =[\theta_1,\dots,\theta_N] \in \Theta$, the value of $\theta_i$ encodes the label prediction for the $i$th datapoint. For example, in the case of binary cross-entropy loss (log-loss), we have a prediction probability vector $\theta \in [0,1]^N$ and a labeling $\sigma \in \{0,1\}^N$; the loss on $(\sigma,\theta)$ is given by:
\begin{align}
    \label{eq:log_loss_defn}
    \logloss\paran{\sigma,\theta} = \frac{-1}{N}\ln \paran{\prod_{i=1}^N \theta_i^{\sigma_i}(1-\theta_i)^{1-\sigma_i}}.
\end{align}
In this case, $\theta_i$ is the probability assigned to the event $\sigma_i = 1$ by the ML model.
% As another example, consider another common loss function ....
% \shiva{Add another example that we consider.}
% As another example, consider another common loss function, the Kullback-Leibler loss (or KL-loss in short), which is defined as follows for $\theta \in [0,1]^N$ and $\sigma \in \{0,1\}^N$ (see~\citep{van2014renyi} for a primer on R\'enyi divergences):
% \begin{align}
%     \label{eq:kl_loss_defn}
%     \textsc{KL-Loss}(\sigma,\theta) = \sum_{i=1}^N \paran{\sigma_i \ln \frac{\sigma_i}{\theta_i} + (1-\sigma_i) \ln \frac{(1-\sigma_i)}{(1-\theta_i)}}.
% \end{align}
% More generally, the R\'enyi-Loss of order $\alpha \in (0,\infty)$ can be defined for $\theta \in [0,1]^N$ and $\sigma \in \{0,1\}^N$ as follows (for $\alpha = 1$ this is the same as the KL-loss above):
% \begin{align}
%     \label{eq:R\'enyi_loss_defn}
%     \textsc{R\'enyi-Loss}_\alpha(\sigma,\theta) = \frac{1}{\alpha-1}  \sum_{i=1}^N \ln   \paran{\sigma_i^\alpha \theta_i^{1-\alpha} + (1-\sigma_i)^\alpha (1-\theta_i)^{1-\alpha}}.
% \end{align}
We work with different loss functions that place different restrictions on $\Theta$. For example, in the case of multiclass cross-entropy loss (with $K$ classes), we have $\Theta \in [0,1]^{N \times K}$.  
% Note that different loss functions place different restrictions on $\Theta$ (i.e., $\Theta \in [0,1]^{N\times K}$, $\Theta \in \{0,1\}^N$, etc.). For the binary label case that we consider in this paper, we can convert $\theta \in [0,\infty)^N$ to $\theta' \in [0,1]^N$ by using the transformation $\theta_i' = \theta_i/(1+\theta_i)$. This is equivalent to saying that for the $i$th datapoint, the probability that it belongs to class $1$, as predicted by $\theta'$ is $\theta_i'$, and that for class $0$ is $1 - \theta_i' = 1/(1+\theta_i)$.

\noindent\textbf{Codomain Separability.} Informally, we call a function codomain separable if there exists some vector $\theta \in \Theta$ such that the function output on each $\ZZZ_K^N$  is distinct (keeping $\theta$ fixed). Thus, when $\theta$ is known, this one-one correspondence between the function's output and the labelings in $\ZZZ_K^N$ can be exploited to exactly recover all the labels from just observing the output.
% \footnote{Codomain separability differs from other notions of separability defined in the literature for functional analysis.}
% For example, multiplicatively separable functions $f(x,y)$ can be expressed as a product of two functions $f(x,y) = g(x)h(y)$, and additively separable functions satisfy $f(x,y) = g(x) 
% + h(y)$. Another important distinction we make is with hyperplane separability over sets of points in $\mathbb{R}^N$, which is a common notion in non-negative matrix factorization and image segmentation literature~\citep{arora2016computing,donoho2004does}.
% \shiva{Using \emph{\zero-codomain separability} to separate it from $\tau$-codomain separability?}
\begin{definition} [$\tau$-codomain separability]
\label{def:codomain_separability}
Let $f: \ZZZ_K^N \times \Theta \to \mathbb{R}$ be a function. For $\theta \in \Theta$, define $\Lambda_{\theta}(f) := \min_{\sigma_1,\sigma_2 \in \ZZZ_K^N} \abs{f(\sigma_1,\theta) - f(\sigma_2,\theta)}$ to be the minimum difference in the function output keeping $\theta$ fixed. For a fixed $\tau > 0$, we say that $f$ admits \emph{$\tau$-codomain separability} using $\theta$ if $\Lambda_{\theta}(f) \geq \tau$. In particular, we say that $f$ admits \emph{\zero-codomain separability} using $\theta$ if there exists any $\tau > 0$ such that $\Lambda_{\theta}(f) \geq \tau$. 
\end{definition}
Note that, for a fixed $\theta$, if a function is $\tau$-codomain separable, then it is also $\tau'$-codomain separable for $0 < \tau' < \tau$. Compared to $\tau$-codomain separability for $\tau >0$, the \zero-codomain separability is weaker as it only requires $\Lambda_{\theta}(f) > 0$. This condition is used for label inference in the unnoised case. 

As an example for $\tau$-codomain separability, consider the function 
% $f:\{0,1\}^N \times \mathbb{R}^N \to \mathbb{R}$, defined as 
$f(\sigma,\theta) = \langle \sigma, \theta \rangle$ for $\sigma \in \{0,1\}^N$. To demonstrate $\tau$-codomain separability, it suffices to set $\theta = [1,2,4,\dots,2^{N-1}]$. Using this, the output $f(\sigma,\theta)$ is the integer whose binary representation (in reverse) is given by the \emph{bits} defined in $\sigma$. Moreover, since the difference between any two integers that can be represented this way is one, it also holds that $\Lambda_\theta(f) = 1$, which makes $f$ admit $1$-codomain separability using $\theta$. Multiplying each entry in $\theta$ by $\tau$ will, thus, make $f$ admit $\tau$-codomain separability for any $\tau > 0$.

% As another example, consider the binary cross-entropy loss from~\eqref{eq:log_loss_defn}. The result \citep[Theorem~5]{aggarwal2020logloss} demonstrates a construction that for any $\tau > 0$ makes this loss $\tau$-codomain separable.

We highlight that in general, determining whether a loss function is codomain separable is co-NP-hard 
% (see Appendix~\ref{app:hardness_results}, where we provide a Karp reduction from the Tautology problem).
However, in the upcoming sections, we discuss our constructions that make many popular loss functions separable. In Appendix~\ref{sec:negative_results}, we present some function classes that are provably not $\tau$-codomain separable.   
% Our general goal will be to construct $\theta$'s that allows for separability with larger values of $\tau$ as that translates into label reconstruction attacks that can handle more noise.    
% Depending, on $f$, Note that $f$ may not be codomain separable using some other $\theta\in\Theta$. 
% Furthermore, for $\theta_1, \theta_2 \in \Theta$, each of which makes $f$ codomain separable, the corresponding $\tau$ can be different.

\noindent\textbf{Robust Label Inference.} Next, we formally define the problem of (robust) label inference from functions defined over the domain $\ZZZ_K^N \times \Theta$. Informally, the goal here is to recover some true labeling (in $\ZZZ_K^N$) upon observing only the function output, even if noised. We consider recovery from noised (perturbed) function outputs in this paper, and the results trivially holds for the unnoised case. 
% A particular focus will be on the binary label case.
%, when the latter is perturbed using some noise.
\begin{definition}[$\tau$-Robust Label Inference]
\label{def:robust_label_inference}
Let $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$ be a function. Let $\sigma^\star \in \ZZZ_K^N$ be an unknown true labeling. For a given $\tau > 0$, we say that $f$ admits $\tau$-robust label inference if there exists $\theta \in \Theta$ and an algorithm (Turing machine) $\mathcal{A}$ that can recover $\sigma^\star$ given any $\ell \in \mathbb{R}$ where $\abs{f(\sigma^\star,\theta) - \ell} < \tau$, \emph{i.e.,} for all $\sigma^\star \in \ZZZ_K^N$, we have $\mathcal{A}\paran{\theta, N, \ell} = \sigma^\star$.
% When $\ell = f(\sigma^\star,\theta)$ (the unnoised case), we say that $f$ admits label inference if there exists $\theta \in \Theta$ and an algorithm (Turing Machine) $\mathcal{A}$ that can recover $\sigma^\star$ given  $f(\sigma,\theta)$.
\end{definition}
Observe that the above definition can also work for the unnoised case by setting $\tau$ arbitrarily small. An important point to note here is that $\tau$-robust label inference requires perfect reconstruction of $\sigma^\star$, which is a {\em stronger} notion than that required by notions like {\em blatant non-privacy}~\citep{dinur2003revealing}, where the goal is to only reconstruct a good fraction of $\sigma^\star$. Also, while the above definition is based on a single query, we will later relax this requirement to study $\tau$-robust label inference under a multi-query model.  


The following simple proposition formally establishes the connection between the above definitions of separability and robust label inference. The proposition is stated for the noised setting. 
% For label inferences in the unnoised setting, it suffices that $f$ admits \zero-codomain separability.

\begin{proposition}\label{prop:bound_on_tau_for_label_inference}
A function $f$ admits $\tau$-robust label inference using $\theta \in \Theta$ if and only if $\Lambda_{\theta}(f) \geq 2\tau$. 
\end{proposition}


In a typical ML setting, assume that we have a server (machine) that holds a private labeled dataset with labels in $\sigma^\star \in \ZZZ_K^N$. Let $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$ denote a (classification) loss function. In Algorithm~\LabelInf, we present a general label inference technique based on Proposition~\ref{prop:bound_on_tau_for_label_inference}. The adversary picks $\theta \in \Theta$ based on Definition~\ref{def:codomain_separability}, to query the server, and gets back the noisy loss function value. It then iterates over the labelings to recover the closest one to the loss value. Throughout this paper, we assume that the adversary knows the loss function, number of datapoints $N$ and an upper bound $\tau$ on the resulting error. We also assume that the loss is computed on all labels in $\sigma^\star$. 




% The algorithm $\mathcal{A}$ (the adversary) has the freedom on choosing $\theta \in \Theta$. The adversary sends a prediction vector $\theta$ to a machine (server) that holds the (private) dataset $\sigma \in \{0,1\}^N$ and gets back the noisy loss function. 
% In the setting where the scores are noised, we assume that the adversary knows an upper bound on the resulting error. Often the former can be inferred from the knowledge of the precision on the machine that returns the loss score to the adversary.

 





% \abhi{Add details on a general Algorithm for Robust-Label Inference in the $\mathsf{APA}$ model.}
\renewcommand{\thealgocf}{}
\SetAlgoCaptionSeparator{}
       \begin{algorithm}[t]
        \SetAlgoLined
        \SetKwInput{KwData}{Input}
        \SetKwInput{KwResult}{Output}
        \SetKwInOut{Model}{Model Setting}
        \KwData{Number of datapoints $N$, bound on error (noise) $\tau > 0$}
        \KwResult{Recovered labels $\hat{\sigma}$}
        \Model{A server (oracle) with private dataset with true labels $\sigma^\star$}
        
        \smallskip
        Design a vector $\theta\in \Theta$ with respect to which $f$ admits $2\tau$-codomain separability (Definition~\ref{def:codomain_separability}).\\
        Query the server using $\theta$ as the prediction vector and observe output $\ell$ with $\abs{f(\sigma^\star,\theta) - \ell } < \tau$.\\
         \textbf{Return} $\hat{\sigma} \gets \arg\min_{\sigma\in \ZZZ_K^N} \abs{f(\sigma,\theta) -\ell}$.
        \caption{\LabelInf: Robust Label Inference for function $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$}
        \label{alg:general_label_inference}
        \end{algorithm}

\begin{remark} \label{rem:first}
A special case of Algorithm~\LabelInf is the unnoised setting, wherein $\ell = f(\sigma^\star,\theta)$. In that case, in Algorithm~\LabelInf, it suffices to design a vector  $\theta \in \Theta$ with respect to which $f$ admits \zero-codomain separability and $\tau$ plays no role (i.e., can be set to an arbitrarily small positive constant).
\end{remark}

An important feature about Algorithm~\LabelInf is that it makes just one call to the server to retrieve the (loss) function $f$ evaluated at a single $\theta$, but still reconstructs the entire private vector (see theorem below).\!\footnote{To baseline Algorithm~\LabelInf with a naive exponential search over the space of all labelings, we simulated label inference on the Titanic dataset (see Section~\ref{sec:experiments}) for the cross-entropy loss, by replacing the prediction vector $\theta$ from Step 1 in Algorithm~\LabelInf by a uniformly random vector in $[0,1]^N$. We observed that over 1000 independent runs, the randomly generated vector failed to correctly infer the true label for even a single datapoint at even mild noise levels ($\tau=0.1$ and higher).\\} We also note that the optimization problem $\arg\min_{\sigma\in \ZZZ_K^N} \abs{f(\sigma,\theta) -\ell}$ can be solved naively by an exponential search over all $\sigma$ in general, and  faster for certain functions under multiple-queries as we discuss in Section~\ref{sec:linearly_separable}. Even the exponential search is a local computation for the adversary.
% repeat the experiment 1,000 times and the maximum vector length at which 100\% accuracy is achieved is 3 and 1 at noise magnitude 0.0001 and 0.01, which are smaller than 10 and 8 by Algorithm~\LabelInf. When the noise magnitude increases to 0.1 and 1, the randomly generated vector cannot correctly infer label vector even at length 1 with 100\% accuracy.\\}. 
% The following theorem follows from the above discussion.
\begin{theorem} \label{thm:inf}
Let $f :\ZZZ_K^N \times \Theta \to \mathbb{R}$.
Algorithm~\LabelInf performs $\tau$-robust label inference on $f$, in that it recovers $\sigma^\star$ (i.e., $\hat{\sigma} = \sigma^\star$) from $
\ell$ where $\abs{f(\sigma^\star,\theta) - \ell } < \tau$.
\end{theorem}
\vspace*{-0.9ex}

\subsection{Separability in Arbitrary Precision vs.\ Finite Floating-Point Precision} 
\label{sec:apa_fpa}
One important consideration in our label inference attacks is the precision of arithmetic that is required at the adversary. In this context, there are two natural models of arithmetic computation: a) arbitrary precision and b) finite floating-point precision. Arbitrary precision arithmetic model allows precise arithmetic results even with very large numbers. In the floating-point precision model, the arithmetic is constrained by limited precision. An example of the floating-point precision model is the commonly used IEEE-754 double precision standard. Designing algorithms for standard arithmetic in both these models have been studied extensively~\citep{knuth2014art,brent2010modern}. Following~\citep{aggarwal2021icml}, we refer to the arbitrary precision arithmetic model as $\mathsf{APA}$ and floating point  arithmetic model with $\phi$ bits as $\mathsf{FPA}(\phi)$. 
% For simplicity, we assume in the $\mathsf{FPA}(\phi)$ model we have $1$ bit for sign, $(\phi-1)/2$ bits for the exponent and $(\phi-1)/2$ bits for the fractional part (mantissa). This assumption can be relaxed to accommodate $\phi_a > 0$ bits for the exponent and $\phi_b > 0$ bits for the fractional part where $\phi_a + \phi_b = \phi-1$.

% \abhi{Zekun, can you please convert the notations in this section from $f:\{0,1\}^N \times \Theta \to \mathbb{R}$ to $f: \{0,1\}^N \times \Theta \to \mathbb{R}$?}

% Our results on codomain separability hold under both these models of arithmetic. 
We begin by observing that Definition~\ref{def:codomain_separability} does not take into account fixed arithmetic precision (i.e., deals with the case where we have arbitrary precision arithmetic). Finite floating-point precision has an effect on separability, as bits of precision places a bound on the resolution. For example, even if $f(\sigma_1,\theta) \neq f(\sigma_2,\theta)$ in the $\mathsf{APA}$ model, with only $\phi$ bits of precision, this difference may not be observable. This leads to notion of separability in the $\mathsf{FPA}(\phi)$ model (formalized in Definition~\ref{def:FPA_codomain_separability}, Appendix~\ref{app:prelim}). 
Let $f_\phi$ be the representation of $f$ in the $\mathsf{FPA}(\phi)$ model.\!\footnote{Informally, representation in the $\mathsf{FPA}(\phi)$ model implies computing $f$ within the granularity defined by $\phi$, and reporting underflow/overflow when the results are out of range.} It is easy to show that if $f_\phi$ admits $\tau$-codomain separability using $\theta$, then $f$ also admits $\tau$-codomain separability in the $\mathsf{APA}$ model using $\theta$ (see Proposition~\ref{prop:FPAAPA}, Appendix~\ref{app:prelim}). The other direction is trickier, but we can establish that if $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using  $\theta$, then $f_\phi$ admits $\tau$-codomain separability using $\theta$ if $\phi\geq\max(2 \log_2 \tau  + 5,  -2\log_2\tau - 1)$ (see Proposition~\ref{prop:APAFPA}, Appendix~\ref{app:prelim}).   
% We examine the connection between separability in these two models as follows.
% \shiva{Add what Definition~\ref{def:codomain_separability} means in the $\textsc{FPA}(\phi)$ model in the appendix.}
% \noindent\textbf{Models of Computation.} We present our results in two models of arithmetic computation. The first model assumes \textit{arbitrary precision arithmetic}, which allows precise arithmetic results even with very large numbers. We refer to this as the 
% $\mathsf{APA}$ model. While this model results in considerably slower arithmetic~\citep{brent2010modern}, it helps an adversary to perform label inference with fewer queries.
% The second model is the more standard \textit{floating point precision model}, where the arithmetic is constrained by limited precision. We denote this model as $\mathsf{FPA}(\phi)$, where $\phi$ represents the number of bits of precision. We assume the following abstraction for the format for representing numbers in this model: 1 bit for sign, $(\phi-1)/2$ bits for the exponent and $(\phi-1)/2$ bits for the fractional part (mantissa).\footnote{More generally, one could allocate $\phi_a$ bits for the exponent and $\phi_b$ bits for the fractional part where $\phi_a + \phi_b = \phi-1$. This is the setting in our experiments.} This allows representing all numbers between $-2^{(\phi-1)/2}$ to $+2^{(\phi-1)/2}$, with a resolution of $2^{-(\phi-1)/2}$. The floating point precision model allows for more efficient arithmetic operations~\citep{brent2010modern}. We refer the reader to Chapter 4 in~\citep{ knuth2014art} for a detailed discussion on designing algorithms for standard arithmetic in these models.

% \begin{proposition} \label{prop:FPAAPA}
% Let $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$, $\theta \in \Theta$, and $\tau > 0$. Let $f_\phi$ be the representation of $f$ in the $\mathsf{FPA}(\phi)$ model\footnote{Informally, representation in the $\mathsf{FPA}(\phi)$ model implies computing $f$ within the granularity defined by $\phi$ (see the discussion before Proposition~\ref{prop:FPAAPA}), and reporting underflow/overflow when the results are out of range.}. If $f_\phi$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi)$ model (using $\theta$) for some $\phi > 0$, then $f$ also admits $\tau$-codomain separability in the $\mathsf{APA}$ model using $\theta$. Moreover, $f_{\phi'}$ also admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi')$ model using $\theta$ for all $\phi' > \phi$.
% \end{proposition}
% \begin{proof}
% Given $\theta$ and the fact that $f_\phi$ admits $\tau$-codomain separability using $\theta$ in the $\mathsf{FPA}(\phi)$ model, denote
% \begin{align*}
%     \Lambda_\theta(f_\phi) = \min_{\sigma_1,\sigma_2 \in \ZZZ_K^N} \abs{f_\phi(\sigma_1,\theta) - f_\phi(\sigma_2,\theta)} = b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} > 2\tau, 
% \end{align*}
% where each $b_i \in \{0,1\}$. Then, in the $\mathsf{FPA}(\phi+1)$ model, we can write (without loss of generality):
% \begin{align*}
%     \Lambda_\theta(f_{\phi+1}) &= \begin{cases}
%     0b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} &\ \ \text{if $\phi$ is even},\\
%     b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}}0&\ \ \text{if $\phi$ is odd}
%     \end{cases}\\
%      &= b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} > 2\tau,
% \end{align*}
% which establishes that $f_{\phi+1}$ is $\tau$-codomain separable using $\theta$ in the $\mathsf{FPA}(\phi+1)$ model. By induction, this implies that $f_{\phi'}$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi')$ model using $\theta$ for all $\phi' > \phi$. In the limit when $\phi \to \infty$, this is equivalent to saying that $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using $\theta$.
% \end{proof}

% \begin{proposition}
% For any function $f:\{0,1\}^N \times \Theta \to \mathbb{R}$ and $\theta \in \Theta$, it holds that for all $\tau \geq 0$, if $f$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi)$ model (using $\theta$) for some $\phi > 0$, then $f$ also admits $\tau$-codomain separability in the $\mathsf{APA}$ model using $\theta$. 

% Moreover, $f$ also admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi')$ model using $\theta$ for all $\phi' > \phi$.
% \end{proposition}
% \begin{proof}
% Given $\theta$ and the fact that $f$ admits $\tau$-codomain separability using $\theta$ in the $\mathsf{FPA}(\phi)$ model, denote
% \begin{align*}
%     \Lambda_\theta(f) = \min_{\sigma_1,\sigma_2} \abs{f(\sigma_1,\theta) - f(\sigma_2,\theta)} = b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} > 2\tau, 
% \end{align*}
% where each $b_i \in \{0,1\}$. Then, in the $\mathsf{FPA}(\phi+1)$ model, we can write (without loss of generality):
% \begin{align*}
%     \Lambda_\theta(f) &= \begin{cases}
%     0b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} &\ \ \text{if $\phi$ is even},\\
%     b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}}0&\ \ \text{if $\phi$ is odd}
%     \end{cases}\\
%      &= b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} > 2\tau,
% \end{align*}
% which establishes that $f$ is $\tau$-codomain separable using $\theta$ in the $\mathsf{FPA}(\phi+1)$ model. By induction, this implies that $f$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi')$ model using $\theta$ for all $\phi' > \phi$. In the limit when $\phi \to \infty$, this is equivalent to saying that $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using $\theta$.
% \end{proof}
% We establish the correspondence in the other direction, starting from separability in the $\mathsf{APA}$ model.
% \begin{proposition} \label{prop:APAFPA}
% Let $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$, $\theta \in \Theta$, and $\tau > 0$. Let $f_\phi$ be the representation of $f$ in the $\mathsf{FPA}(\phi)$ model.  If $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using some $\theta \in \Theta$ and for some $\tau > 0$, then $f_\phi$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi)$ model using $\theta$ for $\phi\geq\max(2 \log_2 \tau  + 5,  -2\log_2\tau - 1)$.
% \end{proposition}
% \begin{proposition} \label{prop:APAFPA}
% For any function $f:\{0,1\}^N \times \Theta \to \mathbb{R}$, it holds that, if $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using some $\theta \in \Theta$ and for some $\tau > 0$, then $f_\phi$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi)$ model using $\theta$ for $\phi\geq\max(2 \log_2 \tau  + 5,  -2\log_2\tau - 1)$.
% \end{proposition}
% \shiva{Not following the proof. There is some missing min in the condition on $\phi$?}
% Similar to the proof above, denote (in the $\mathsf{APA}$ model) the following:
% \begin{align*}
%     \Lambda_\theta(f) = b_m\cdots b_1 b_0\ .\ b_{-1}b_{-2}b_{-3} \cdots,
% \end{align*}
% for some finite $m > 0$ (\zeku{should we also capture the floating point precision after the decimal point, i.e. $0.b_{-1}b_{-2}...b_{-m}$?}). \abhi{In the APA model, we have infinite precision.\zeku{I see. For example, if $f$ is $\tau$-codomain separable in APA for some tiny $\tau$, where $\lfloor \log_2\tau\rfloor < -5$, does it mean it is also $\tau$-codomain separable in FPA(1)?}} \abhi{Hmm.. good point. We need to check this corner case. I will think more about it. Thanks!} Since $\Lambda_\theta(f) > 2\tau$, it must be the case that $m \geq \lfloor \log_2 (2\tau) \rfloor = 1 + \lfloor \log_2 \tau \rfloor$. Thus, if $f$ has to admit $\tau$-codomain separability in the $\mathsf{FPA}(\phi)$ model using $\theta$, we must have $\frac{\phi-3}{2} \geq m$, which gives $\frac{\phi-3}{2} \geq m \geq 1 + \lfloor \log_2 \tau \rfloor \Longrightarrow \phi \geq 2\lfloor \log_2 \tau \rfloor + 5$. \abhi{Shiva, please check this proof.}
% \end{proof}
% \shiva{it will be good to have an corollary about the condition on $\tau$ in terms of $\phi$}
% \abhi{Talk about polytime inference in FPA model vs. APA model.}
% \zeku{Proposed revised proof for Proposition 2.}
% \begin{proof}
% Suppose $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model. To establish $f_\phi$ as $\tau$-codomain separability in $\mathsf{FPA}(\phi)$, we need to split the two cases: $\tau>1$ and $\tau<1$.
% Represent $\Lambda_{\theta}(f_\phi)$ in $\mathsf{FPA}(\phi)$ as 
% $$b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}}.$$
% When $\tau>1$, a sufficient condition for $f_\phi$ to satisfy the $\tau$-codomain separability is to have enough precision before the decimal point,
% $$2^{\frac{\phi-3}{2}}\geq 2\tau,$$
% which gives $\frac{\phi-3}{2}  \geq 1 + \log_2 \tau  \Longrightarrow \phi \geq 2 \log_2 \tau  + 5$. When $\tau<1$, a sufficient condition for $f_\phi$ to satisfy $\tau$-codomain separability is to have enough precision after the decimal point,
% $$2^{-\frac{\phi-1}{2}}\leq 2\tau,$$
% which gives $-\frac{\phi-1}{2}\leq 1 +  \log_2 \tau \Longrightarrow \phi \geq -2\log_2\tau - 1$. The proposition follows from combining the two together to obtain $\phi\geq\max(2 \log_2 \tau  + 5,  -2\log_2\tau - 1)$.
% \end{proof}

% \abhi{I think this looks good. Thanks Zekun! Shiva, can you please proof read this as well? Thanks!}
% \begin{corollary} \label{cor:APAFPA}
% For any function $f_\phi:\ZZZ_K^N \times \Theta \to \mathbb{R}$, $f_\phi$ admits $\tau$-codomain separability using $\theta \in \Theta$ in the $\mathsf{FPA}(\phi)$ model for $\phi \geq 5$ if both the following two conditions hold:
% \begin{CompactEnumerate}
%     \item $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using some $\theta \in \Theta$, and
%     \item It holds that $2^{-\parfrac{\phi+1}{2}} \leq \tau \leq 2^{\parfrac{\phi-5}{2}}$.
% \end{CompactEnumerate}
% \end{corollary}
% \begin{corollary} \label{cor:APAFPA}
% For any function $f:\{0,1\}^N \times \Theta \to \mathbb{R}$, $f$ admits $\tau$-codomain separability using $\theta \in \Theta$ in the $\mathsf{FPA}(\phi)$ model for $\phi \geq 5$ if both the following two conditions hold:
% \begin{enumerate}
%     \item $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using some $\theta \in \Theta$, and
%     \item it holds that $2^{-\parfrac{\phi+1}{2}} \leq \tau \leq 2^{\parfrac{\phi-5}{2}}$.
% \end{enumerate}
% \end{corollary}
% \shiva{Misleading:
% Given these above conditions, it follows that an inference attack in the $\mathsf{APA}$ model outlined in Algorithm~\LabelInf, also succeeds in the $\mathsf{FPA}(\phi)$ model if $\max_\sigma |f(\sigma,\theta)|\leq 2^{\frac{\phi-3}{2}}$. \abhi{Zekun, please add one line to explain this.}}
% Now, given a $\tau$-robust label inference algorithm in $\mathsf{APA}$ model using $\theta$, if condition 2 in Corollary 1 holds,  then we can run the algorithm as is to perform $\tau$-robust label inference in $\mathsf{FPA}(\phi)$ model. 
% \abhi{Zekun, please verify that running the algorithm in FPA will not need any additional bits than what is required by Prop 2.}
% Given these above conditions, it follows that an inference attack in the $\mathsf{APA}$ model outlined in Algorithm~\LabelInf, also succeeds in the $\mathsf{FPA}(\phi)$ model. 
Moving to label inference, note that Algorithm~\LabelInf is also described in the $\textsc{APA}$ model. The above mentioned bound on $\phi$ may not suffice for $\tau$-robust label inference using Algorithm~\LabelInf in the $\mathsf{FPA}(\phi)$ model. This is because unlike codomain separability, Algorithm~\LabelInf requires the adversary to compute the loss function on all labelings of the datapoints, which may require additional bits. For example, the prediction vector we provide for multiclass cross-entropy loss in Theorem~\ref{thm:multi_class_proof} contains entries that are doubly-exponential in $N$ (number of  datapoints) and $K$ (number of classes). This would prohibit the correct computation of loss scores beyond some values of $N$ and $K$ in the $\mathsf{FPA}(\phi)$ model. However, this issue could be overcome by the ability to perform multiple queries that we utilize in our experimental evaluation in Section~\ref{sec:experiments}. For simplicity of description, we present our inference attacks under the $\mathsf{APA}$ model in the main body of this paper.

% \shiva{Say what this above corollary really means, and whether what can we expect Algorithm~\LabelInf to do in the $\mathsf{FPA}(\phi)$ model that is consistent with what we observe in expts.} \abhi{I'll need some help on the best way to frame this. Perhaps we can discuss in the meeting today.}
% For simplicity of description, we present our inference attacks under the $\mathsf{APA}$ model. Our experimental results, however, utilize standard double precision format arithmetic (IEEE 754 standard). 

% \subsection{Some Caveats about Single-query vs. Multi-query (Robust) Label Inference}
% In this section, we discuss some caveats associated with converting a single-query robust label inference algorithm into a multi-query algorithm. We also provide sufficient conditions under which this conversion can be done efficiently. \abhi{TODO.}

==> AISTATS'22/neurips2021/experiments.tex <==
%\begin{table}[h]
%\begin{tabular}{lllp{3.5cm}p{2.6cm}} 
%\hline
% Loss & Data & Noise & Max. vector length for perfect label inference & Mean run time per inference (ms) \\ \hline
% Cross-entropy & Titanic & 0.0001 & 10 (15 by ICML) & 1.71 \\
% Cross-entropy &Titanic & 0.01 & 7 (9 by ICML)  & 0.20 \\
% Cross-entropy &Titanic & 0.1 & 5 (6 by ICML)  & 0.07 \\
% Cross-entropy & Titanic & 1 & 4 (4 by ICML) & 0.04 \\
% Cross-entropy & Iris & 0.0001 & 6 & 0.94 \\
% Cross-entropy & Iris & 0.01 & 4 & 0.10 \\
% Cross-entropy & Iris & 0.1 & 3 & 0.04 \\
% Cross-entropy & Iris & 1 & 2 & 0.02 \\
% Cross-entropy & Satellite & 0.0001 & 3 & 0.26\\
% Cross-entropy & Satellite & 0.01 & 2 & 0.08 \\
% Cross-entropy & Satellite & 0.1 & 1 & 0.05 \\
% Cross-entropy & Satellite & 1 & 1 & 0.05\\
% Sigmoid cross-entropy & ... & ... & 0 & \\
% Softmax cross-entropy & Titanic & 0.0001 & 7 & 2.07 \\
% Softmax cross-entropy & Titanic & 0.01 & 3 & 0.12 \\
% Softmax cross-entropy & Titanic & 0.1 & 1 & 0.05 \\
% Softmax cross-entropy &  Titanic & 1 & 0 & \\
% Softmax cross-entropy & Iris & 0.0001 & 3 & 0.25 \\
% Softmax cross-entropy & Iris & 0.01 & 1 & 0.03 \\
% Softmax cross-entropy & Iris & 0.1 or 1 & 0 & \\
% Softmax cross-entropy & Satellite & & 0 & \\
% \hline
%\end{tabular}
%\label{exp1}
%\end{table}
We now present our empirical evaluation of label inference attacks on cross-entropy loss and its extensions (see Appendix~\ref{app:experiments} for additional results)\footnote{All experiments are run on a 64-bit machine with 2.6GHz 6-Core processor, using the standard IEEE-754 double precision format. For reproducibility, the code is included as part of the supplementary material.}. We use the following datasets for our analysis. As our attacks construct prediction vectors that are independent of the dataset contents, we ignore the dataset features in our experiments. All the labels of the dataset are considered for the attack.
%\shiva{Zekun: can you upload all the plots as individual files, like in the ICML submission? That way we can set the spacing correctly.}
%\zeku{The individual figures are uploaded in the individual\_figure folder, with intuitive filenames. Please double check and rearrange as appropriate.}
\begin{CompactItemize}
    \item {\bf{Titanic}}~\cite{titanic}: a binary classification dataset (2201 rows) on the survival status of passengers.
    % , fetched from  \url{https://www.openml.org/d/40704}
    \item {\bf{Iris}}~\cite{iris}: a three-class classification dataset (150 rows) on the Iris species.
    \item {\bf{Satellite}}~\cite{satellite}: a six-class classification dataset (6430 rows) on the satellite images of soil.
\end{CompactItemize}
We consider three common loss functions mentioned in Section~\ref{sec:logloss}: multiclass cross-entropy, softmax cross-entropy, and sigmoid cross-entropy (deferred to Appendix~\ref{app:experiments}). As a baseline, for the binary labeled dataset (Titanic) with the cross-entropy loss, we implemented the label inference attack of Aggarwal~\emph{et al.}\ \citep{aggarwal2021icml} (see Theorem~\ref{thm:from_icml}, Appendix~\ref{app:experiments} for a restatement of their main result).

We start with the distinction between our experiments and Algorithm~\LabelInf, which is presented in the $\textsc{APA}$ model. For example in the multiclass cross-entropy loss (\Klogloss) case, to simulate Algorithm~\LabelInf on a finite precision machine, we must be able to differentiate $\min_{i,k}\theta_{i,k}$ from 0 (or else the label inference will be ambiguous). A rough analysis (from Theorem~\ref{thm:multi_class_proof}) gives that 
% $\min_{i,k}\theta_{i,k}\approx \vartheta_{N,1}/\vartheta_{N,K} = 3^{2^{(N-1)K+1}N\tau}/3^{2^{(N-1)K+K}N\tau}=\Omega(3^{-2^{NK}N\tau})$, which requires a precision of 
$\phi=\Omega(2^{NK}N\tau)$ bits are required to make this distinction. This bound hides constant factors and is likely not tight, but gives an idea of how arithmetic precision  plays a role in our experiments. 

Figure~\ref{fig:singlequery} shows the number of datapoints $N$ recovered by Algorithm~\LabelInf as we increase the noise for various loss functions. We sample 1000 random sets of labels each of length $N$ from the dataset here. At error magnitude $\tau = 1$, the noise is comparable to the actual loss function values computed. We measure accuracy as the percentage of labels correctly inferred out of $N$.
% (since the largest N for at least 50\% accuracy is 8 for sigmoid and softmax cross-entropy), 
Figure~\ref{fig:singlequery}(a) shows that the number of datapoints ($N$) for which 100\% label inference accuracy is achieved for cross-entropy loss decreases as the noise magnitude ($\tau$) increases, which is expected. Moreover, at the same noise magnitude, the accuracy also drops as the number of classes ($K$) increases from 2 (in Titanic) to 6 (in Satellite), which is also expected. These happen because of the dependence on number of datapoints and number of classes in our prediction vector construction (Theorem~\ref{thm:multi_class_proof}), which given fixed machine precision runs into representation issues. We note that for the Titanic dataset, the construction from~\cite{aggarwal2021icml} works slightly better (especially at lower $\tau$ values) than ours due to a small difference in the exponent: it holds that $\min_{i \in [N]}(-\ln \theta_{i}) = \Omega(2^N N\tau)$ in~\cite{aggarwal2021icml} (see Theorem~\ref{thm:from_icml}, Appendix~\ref{app:experiments}), but $\Omega(2^{2N}N\tau)$ when using Theorem~\ref{thm:multi_class_proof} with $K=2$.
% However, our construction is very general and extends to multiclass cross-entropy loss and beyond, which the construction in~\cite{aggarwal2021icml} does not handle.}. 

% Using the prediction vectors from Section~\ref{sec:logloss}, on these 1000 samples of length 8 from Titanic, the mean loss value is 3.64 for cross-entropy, 0.51 for sigmoid cross-entropy, and 0.81 for softmax cross-entropy.

% We further observe that for the Titanic dataset, the construction from~\cite{aggarwal2021icml} works slightly better (especially at lower $\tau$ values) than our construction provided by Theorem~\ref{thm:multi_class_proof}. This is due to a small difference in the exponent: we have $\min_{i \in [N]}\theta_{i} = \Omega(3^{-2^N N\tau})$ in~\cite{aggarwal2021icml} (see Appendix~\ref{app:experiments}), but $\Omega(3^{-2^{2N}N\tau})$ when using Theorem~\ref{thm:multi_class_proof} with $K=2$ (as mentioned above).
% On the other hand our construction is very general and extends to multiclass cross-entropy loss and beyond, which the construction in~\cite{aggarwal2021icml} does not handle.  

Figures~\ref{fig:singlequery}(b)-(c) show the number of datapoints on which Algorithm~\LabelInf achieves at least 50\% accuracy for cross-entropy and softmax cross-entropy loss. We notice this number is smaller for softmax cross-entropy as compared to regular cross-entropy (see Figure~\ref{fig:singlequery}(a)), which is also not surprising. Through a similar argument as that above for the number of bits required for cross-entropy loss, one can show that computing the softmax cross-entropy loss will require an additional $\Omega(NK + \ln(N\tau))$ bits (see the discussion in Appendix~\ref{app:experiments} for details). This additional requirement further constraints the number of labels that can be recovered with softmax cross-entropy loss.



% Finally, the longest computation time for a single label inference across all the experiments with $N=10$ is below 10 milliseconds. 
% In summary, our empirical results attest that these attacks can be performed effectively on real datasets, and also highlight some technical nuances when running label inference on machines with finite floating-point precision. 


% At $N=10$, $K=2$, and $\tau=0.0001$, this implies $\phi > 1000$. However, this upper bound is not tight, as we see in Figure \ref{fig:singlequery}(a) -- our 64-bit machine can perform perfect label inference on the Titanic dataset at noise 0.0001 for length 10. 

% We also ran a baseline label inference experiments on the Titanic dataset for cross-entropy, where the calibrated prediction vector $\theta$ from step 1 in Algorithm~\LabelInf is replaced by a uniformly random vector. We repeat the experiment 1,000 times and the maximum vector length at which 100\% accuracy is achieved is 3 and 1 at noise magnitude 0.0001 and 0.01, which are smaller than 10 and 8 by Algorithm~\LabelInf. When the noise magnitude increases to 0.1 and 1, the randomly generated vector cannot correctly infer label vector even at length 1 with 100\% accuracy.
% \abhi{Moving this closer to Algorithm~\LabelInf in the paper.}


 
 


 



%The median loss in the experiments is about 2.4 for cross-entropy (log-loss), 0.6 for sigmoid cross-entropy loss, and 1.12 for softmax cross-entropy loss. The longest run time for a single label inference across all the experiments based on Algorithm~\LabelInf in this section is below 10 milliseconds.
%\shiva{we need also results in all the plots for the unnoised case, maybe by setting $\tau$ to be extremely small}
 
%The fraction of correctly inferred labelings with respect to the length of the private vector is computed by running the label inference algorithm on 1000 labelings of each specific length randomly sampled from the corresponding dataset. 
 
%\shiva{This needs more discussion. Why is there a drop? Why does  Corollary~\ref{cor:APAFPA} not apply?}
 
%\shiva{can we show $9$ is almost close to what we expect based on the values? Remember the question in the ICML reviews which asked for something like this?}
%\shiva{Comparison to ICML does not show good results for us? We need to revisit this one?}





%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.26]{accuracy.png}
%    \caption{Results on  label inference using Algorithm~\LabelInf on the three real datasets: Titanic, Iris, and Satellite. The first row shows the performance of the label inference from log-loss. The second row shows the performance from sigmoid cross-entropy loss. The third row shows the performance from softmax cross-entropy loss. }
%    \label{accuracy}
%\end{figure}


%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.2]{binary_vs_icml.png}
%    \caption{Results comparing binary log-loss label inference using Algorithm~\LabelInf versus Algorithm 2 in ICML paper on the Titanic dataset. }
%    \label{binary_vs_icml}
%\end{figure}

%
%%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.2]{accuracy_multiquery.png}
%    \caption{Results on the multi-query label inference using Algorithm %\textsc{LabelInf} in shards from log-loss on the three real datasets: Titanic, Iris, and Satellite. }
%    \label{accuracy_multiquery}
%\end{figure}

==> AISTATS'22/neurips2021/linearly_separable_analysis.tex <==
The analysis for cross-entropy loss and its extensions above can be generalized to determine $\tau$-codomain separability for a broad class of loss functions, defined as follows. Let $g:[0,1] \to \mathbb{R}$ be some deterministic function. We say that a binary loss function $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ is linearly-decomposable in $\{0,1\}$ using $g$ if it can be expressed in the following form:
\begin{align}
\label{eq:linear_separable}
f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i \in [N]:\sigma_i=1} g(\theta_i) + \sum_{i \in [N]:\sigma_i=0} g(1-\theta_i)}.    
\end{align}
Our ideas from the previous section can be used to establish the following separability result for linearly-decomposable loss functions, hence, enabling the use Algorithm~\LabelInf for $\tau$-robust label inference in these cases. Missing details are presented in Appendix~\ref{app:bregman}.
\begin{theorem}
\label{thm:linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Then, for any $\tau > 0$, the function $f$ is $2\tau$-codomain separable if there exists $\theta \in (0,1)^N$ so that $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$.
\end{theorem}

\noindent\textbf{Some Examples of Linearly-Decomposable Loss Functions.} Observe that the KL-divergence loss (which reduces to binary cross-entropy loss) is of this form, using $g(\theta_i) = -\ln \theta_i$ (see~\eqref{eq:KL}, Appendix~\ref{app:bregman}). Some other
common examples of linearly-decomposable losses include the (i) Itakura-Saito divergence loss, which can be expressed using $g(\theta_i) = 1/\theta_i + \ln \theta_i - 2$ (see~\eqref{eq:IS}, Appendix~\ref{app:bregman}); (ii) squared Euclidean loss, which can be expressed using $g(\theta_i) = (1-\theta_i)^2$, (see~\eqref{eq:sqEuc}, Appendix~\ref{app:bregman}); and, (iii) norm-like divergence loss, which can be expressed using $g(\theta_i) = 1 + (\alpha-1)\theta_i^\alpha - \alpha \theta_i^{\alpha-1} + (\alpha-1)(1-\theta_i)^\alpha$ for some $\alpha \ge 2$ (see~\eqref{eq:norm}, Appendix~\ref{app:bregman}).

\textbf{Connections to Bregman Divergence.} The loss functions mentioned in (i)-(iii) above are some popular instances of the general class of
Bregman divergence-based loss functions.
% \!\footnote{The  function $g$ is related but not the function associated with the defn.\ of the corresponding divergence.} 
Unlike the distance metrics for probability distributions, Bregman divergence~\citep{bregman1967relaxation} does not require its inputs to be necessarily distributions. Thus, to use these divergences as loss functions, one can directly compare the outputs of the ML model with the point distribution from the ground truth labels~\citep{liu2016clustering}. We defer the details on our general result for $\tau$-codomain separability on Bregman divergence, including that for the Mahalanobis divergence loss (which is not linearly-decomposable) to Appendix~\ref{app:breg_general}.

\textbf{Applying Theorem~\ref{thm:linear_separable}.} Observe that Theorem~\ref{thm:linear_separable} immediately allows constructing a vector that will make a given linearly-decomposable function $f$ admit $\tau$-codomain separability for a given $\tau > 0$: (1) Compute $x^*(y)$ as the solution to $g(x)-g(1-x) = y$; (2) If $x^*(y)$ exists, then set $\theta_i = x^*(2^iN\tau)$ for all $i \in [N]$. This vector $\theta$ can now be used for $\tau$-robust label inference from $f$ using Algorithm~\LabelInf. However, such a $\theta$ might not exist for all loss functions, e.g., it does not exist for squared Euclidean and norm-like divergence losses, and we will deal those loss functions later. It does exist though for the Itakura-Saito divergence loss (defined in~\eqref{eq:IS}, Appendix~\ref{app:bregman}).
% mentioned earlier can satisfy the required condition in Theorem~\ref{thm:linear_separable} on $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$.
\begin{corollary} \label{cor:IS}
The Itakura-Saito divergence loss is $2\tau$-codomain separable with $\theta_i = (1+3^{2^{i}N\tau})^{-1}$.
\end{corollary}


% For the Norm-like divergence loss, observe that $f(\sigma,\theta) < \alpha$ for all $\sigma,\theta$. Hence, this loss is not $\tau$-codomain separable for any $\tau \geq \alpha/(2N)$. Even when $\tau < \alpha/(2N)$, notice that for $\theta_i \in (0,1)$, we can write $g(\theta_i) - g(1-\theta_i) =  \alpha\paran{(1-\theta_i)^{\alpha-1} - \theta_i^{\alpha-1}} < \alpha$. Since $\alpha$ is a constant, there does not exist any $\theta_i$ for which $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$.

\noindent\textbf{Multi-Query Polynomial Time Attacks.} 
The linear-decomposability of $f$ allows for an efficient multi-query label inference algorithm for $f$. In particular, we could have a trade-off between the ability to perform  multiple queries with faster computation times for solving the optimization problem solved in Step 3 of Algorithm~\LabelInf. 
% As noted in Section~\ref{sec:prelim}, whereas the optimization problem in Algorithm~\LabelInf can be naively solved using an exponential search over $\sigma$. 
To see this, observe that setting $\theta_i = 1/2$ gives $g(\theta_i) - g(1-\theta_i) = 0$. Thus, if we want to infer the first $M < N$ labels in a single query, we can set $\theta = [\theta_1,\dots,\theta_M,1/2,\dots,1/2]$ to obtain: 
% so that the following holds:
% \begin{align*}
%     f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i\leq M: \sigma(i)=1} (g(\theta_i)-g(1-\theta_i)) + \sum_{i=1}^M g(1-\theta_i) + \frac{(N-M)g(1/2)}{M}}.
% \end{align*}
% From this, we immediately obtain that:
\begin{align*}
    \Lambda_\theta(f) &= \frac{1}{N} \min_{\sigma_1,\sigma_2 \in \{0,1\}^N} \abs{\sum_{i\leq M:\sigma_1(i)=1}\paran{g(\theta_i)-g(1-\theta_i)} - \sum_{j\leq M:\sigma_2(j)=1}\paran{g(\theta_j)-g(1-\theta_j)}}.
\end{align*}
Similar to Theorem~\ref{thm:linear_separable}, choosing $\theta_i$ that ensures $g(\theta_i)-g(1-\theta_i) > 2^iN\tau$ will ensure $\Lambda_\theta(f) > 2\tau$. Moreover, using this $\theta$ will ensure that if $f(\sigma_1,\theta) = f(\sigma_2,\theta)$, then $\sigma_1[:M] = \sigma_2[:M]$ must hold.  Note that after recovering the first $M$ labels, we can recover the next $M$ labels using $\theta = [1/2,\dots,1/2,\theta_{M+1},\dots,\theta_{2M},1/2,\dots,1/2]$, and so on. The result below immediately follows.

% \input{neurips2021/single_query_plot}

\begin{theorem}
\label{thm:multi_query_general} 
Let $g:[0,1] \to \mathbb{R}$ be some finite deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Then, for any $\tau > 0$ and integer $M \geq 1$, a sufficient condition for $f$ to admit $\tau$-robust label inference with $\lceil N/M \rceil$ queries is for the inequality $g(x) - g(1-x) > 2^iN\tau$ to have a solution for all $i \in [N]$.
% there exist $x_1,\dots,x_M \in (0,1)$ such that $g(x_i) - g(1-x_i) > 2^iN\tau$ for all $i \in [M]$.
\end{theorem}
Observe that an $\lceil N/M \rceil$-query algorithm for robust label inference will require $O(N2^M/M)$ local computations by the adversary (using Algorithm~\LabelInf in each query). Thus, while the single query case ($M = N$) required $O(2^N)$ computations, any multi-query algorithm using $M=O(\log N)$ requires only $O(\text{poly}(N))$ local computations, which allow a polynomial-time robust label inference. 

\noindent\textbf{Linearly-Decomposable Functions Not Covered by Theorem~\ref{thm:linear_separable}.} We now deal with linearly-decomposable functions for whom there exists no $\theta$ that could satisfy the condition required in Theorem~\ref{thm:linear_separable} (examples include, squared Euclidean and norm-like divergence loss). Here, we establish the weaker \zero-codomain separability, which as discussed earlier suffices for label inference in the unnoised case. 

% \noindent\textbf{A Note on the \zero-Codomain Separability of Linearly-Decomposable Functions.} Observe that in Theorem~\ref{thm:linear_separable}, the condition on the function $g$ has a linear dependence on $\tau$, which will not suffice for label inference in the un-noised setting (where $\tau=0$). We state the result for this special case in the Theorem below\footnote{Note that while it is true that any vector with respect to which a function is $\tau$-codomain separable (for $\tau>0$) also allows \zero-codomain separability, we mention Theorem~\ref{thm:zero_codomain_linear_separable} to cover cases where $\tau$-codomain separability is hard to demonstrate (see the discussion about Norm-Like loss following the statemnt of Theorem~\ref{thm:zero_codomain_linear_separable}).} and show how it can be used to achieve \zero-codomain separability for the Square-Euclidean loss and the Norm-Like loss. 

\begin{theorem}
\label{thm:zero_codomain_linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Let $\theta \in (0,1)^N$ be some vector and $S_\theta = \{g(\theta_i) - g(1-\theta_i)\}_{i=1}^N$. Then, the function $f$ is \zero-codomain separable with respect to $\theta$ if $\mu(S_\theta)>0$, i.e., all subset sums in the set $S_\theta$ are distinct.
\end{theorem}
\begin{corollary} \label{cor:eucl}
The squared Euclidean loss  is  \zero-codomain separable using $\theta_i = (1/2)\paran{1-\ln(p_i)/N}$, where $p_i$ is the $i$th prime number for $i \in [N]$. The norm-like divergence loss for $\alpha \geq 2$ is \zero-codomain separable using $\theta$ that satisfies $(1-\theta_i)^{\alpha-1}-\theta_i^{\alpha-1} = (\ln p_i)/(N\alpha)$.
\end{corollary}
Finally, the idea behind the multi-query attack mentioned in Theorem~\ref{thm:multi_query_general} also extends to loss functions covered by Theorem~\ref{thm:zero_codomain_linear_separable}, thus, providing a multi-query polynomial time inference here too. 

% \section{$\tau$-Robust Label Inference from Bregman Divergence-based Binary Losses}
% \label{sec:bregman}
% We now discuss label inference from another important class of distance metrics used across ML applications, known as the class of Bregman divergences~\citep{bregman1967relaxation}. Given a continuously differentiable strictly convex function $F:\mathcal{S} \to \mathbb{R}$ over some closed convex set $\mathcal{S} \subseteq \mathbb{R}^d$, the Bregman divergence $D_F: \mathcal{S} \times \mathcal{S} \to \mathbb{R}$ associated with $F$ is defined as $D_F(\mathbf{p},\mathbf{q}) = F(\mathbf{p})-F(\mathbf{q})-\langle \nabla F(\mathbf{q}), \mathbf{p}-\mathbf{q} \rangle$. Missing details from this section are collected in Appendix~\ref{app:bregman}.

% % Some examples of Bregman divergence are the squared Euclidean distance $D_F(x,y) = \|x-y\|_2$, generated by the convex function $F(x) = \|x\|^2$; the squared Mahalanobis distance $D_F(x,y) = \frac{1}{2}(x-y)^\top Q(x-y)$, generated by $F(x) = \frac{1}{2}x^\top Qx$ for some positive semi-definite matrix $Q$; and, the generalized Kullback-Leibler divergence $D_F(p,q) = \sum_i p(i) \log \frac{p(i)}{q(i)} - \sum_i p(i) + \sum_i q(i)$, generated by $F(x) = -\sum_i p(i)\log p(i)$. 

% Note that unlike the distance metrics for probability distributions, Bregman divergence does not require its inputs to be necessarily distributions. Thus, to use these divergences as loss functions, one can directly compare the outputs of the ML model with the point distribution from the ground truth labels~\citep{liu2016clustering}. We will focus on the binary case for our discussion in this section and assume that the domain of $F$ is the closed convex set $[0,1]^N$, the $N$-dimensional hypercube. 
% % The multiclass setting will immediately follow by modeling the $K$-ary classifier as an ensemble of $K$ one-vs-all binary classifiers using standard techniques. \shiva{I do not follow, why does the same not hold for log-loss then?}

% For starters, a common Bregman divergence loss on $N$ datapoints defined using (generalized) Kullback-Leibler (KL) divergence  $\text{KL}([x_1,x_2]) = \sum_{j=1}^2 (x_j \log x_j)$, in the binary
% %classification 
% setting~\citep{liu2016clustering}, 
% $$\frac{1}{N}\sum_{i=1}^N  D_{\text{KL}}([\sigma_i,1-\sigma_i],[\theta_i,1-\theta_i]) = \frac{-1}{N}  \sum_{i=1}^N \sigma_i \log \theta_i + (1-\sigma_i) \log(1-\theta_i),$$
% % \shiva{we have $\ln 0$? as $\sigma_i$ could be $0$? Should we say $0 \ln 0 = 0$?}
% is exactly the cross-entropy loss\footnote{Here, we adopt the notion that $0\ln 0=0$, so that KL divergence is well-defined.} and is therefore covered by results in Section~\ref{sec:logloss}. Similar to the general construction of robust label inference for linearly-decomposable functions in Section~\ref{sec:linearly_separable}, we now demonstrate $\tau$-robust label inference for a special class of Bregman divergences: the ones associated with functions $F$ that are additive on the elements of its input vector.
% \begin{theorem}
% \label{thm:bregman_general} Let $F:(0,1)^2 \to \mathbb{R}$ be a strictly convex function that can be written in the form $F(\mathbf{v}) = \sum_{i=1}^2 h(v_i)$ for some differentiable function $h:(0,1) \to \mathbb{R}$. Let $D_F$ denote the Bregman divergence associated with $F$, and $f_F:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be the corresponding loss function, defined as $f_F(\sigma,\theta) = (1/N)\sum_{i=1}^N D_F([1-\sigma_i,\sigma_i],[1-\theta_i,\theta_i])$. Then, for $\tau > 0$, the function $f_F$ is $2\tau$-codomain separable if there exists $\theta \in (0,1)^N$ that satisfies  $h'(\theta_i) + h'(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$, where $h'(x) = dh/dx$.
% \end{theorem}

% \shiva{This discussion is not clear? Do we have any loss where the above theorem works?}
% Some common examples of Bregman divergence that are additive, include the KL-divergence and the Ikatara-Saito divergence, that recall are also linearly decomposable (from Theorem~\ref{thm:linear_separable}). Thus, any vector constructed from either Theorems~\ref{thm:linear_separable} or~\ref{thm:bregman_general} will allow $\tau$-robust label inference for these corresponding losses. 

% However, not all Bregman divergences are additive. A popular example of a Bregman divergence that is not additive is the Mahalanobis divergence, the loss corresponding to which is defined as follows:
% $$\textsc{MHLoss}(\sigma, \theta) = \frac{1}{N}\sum_{i=1}^N ([\sigma_i,1-\sigma_i] - [\theta_i,1-\theta_i])^\top A ([\sigma_i,1-\sigma_i] - [\theta_i,1-\theta_i]) \mbox{ where} A \in \mathbb{R}^{2 \times 2}.$$
% We discuss $\tau$-robust label inference for the Mahalanobis loss function in the theorem below.
% \begin{theorem}
% \label{thm:mahalanobis}
% Let $A = \bigl[\begin{smallmatrix}
% a&b\\ c&d
% \end{smallmatrix}\bigr] \in \mathbb{R}^{2 \times 2}$ be a matrix with $(a+d)>(b+c)$. Denote $\alpha = a+d-(b+c)$ and let $\tau \in [0,\alpha/N)$. Then, for any $\tau > 0$, the Mahalanobis loss (defined above) 
% % defined by $$\textsc{MHLoss}(\sigma, \theta) = \frac{1}{N} \sum_{i=1}^N ([\sigma_i,1-\sigma_i] - [\theta_i,1-\theta_i])^\top A ([\sigma_i,1-\sigma_i] - [\theta_i,1-\theta_i]),$$ 
% is $\tau$-codomain separable using any $\theta \in (0,1)^N$ with $\|\theta\|_\infty < (1/2)\paran{1 - N\tau/\alpha}$.
% \end{theorem}

==> AISTATS'22/neurips2021/log_loss_analysis.tex <==
We start with establishing $\tau$-codomain separability for multiclass cross-entropy loss and its variants, for any $\tau > 0$. This implies that for these loss functions, Algorithm~\LabelInf succeeds in recovering all the labels when the loss scores are noised by less than $\tau$ in magnitude. We explain our main results at a high level and defer all missing details from this section to Appendix~\ref{app:logloss}. 
% This extends the results in~\citep{aggarwal2021icml}, where $\tau$-robust label inference in the binary case ($K=2$) was discussed. 
% Missing details from this section are collected in Appendix~\ref{app:logloss}.
% it is possible to design a prediction vector such that the multiclass cross-entropy loss scores differ by more than $2\tau$ on any two distinct labelings. Therefore, one could Algorithm~\LabelInf to perform 
% We begin by explaining the intuition behind our construction and then provide a formal proof of correctness. We also discuss how to generalize this approach to commonly used variants of the cross-entropy loss. We will end this section with a discussion around the computational hardness of label reconstruction for such losses, and show that this problem is in EXPTIME.

\noindent\textbf{Multiclass Cross-Entropy Loss.} We first recall the definition of multiclass cross-entropy (extending Definition~\ref{eq:log_loss_defn}). 
We assume $K \geq 2$ classes, and let $N$ and $\ZZZ_{K}$ denote the number of datapoints and the set of label classes, respectively. The $K$-ary cross-entropy loss on $\theta$ with respect to a labeling $\sigma \in \ZZZ_{K}^N$ is denoted by $\Klogloss\paran{\sigma, \theta}$ and defined as follows:
	\begin{align}
	\label{eq:multi_class_log_loss}
		\Klogloss\paran{\sigma, \theta} := \frac{-1}{N}\sum_{i=1}^N \sum_{k=0}^{K-1} \ \Big([\sigma_i = k] \cdot \ln \theta_{i,k} \Big),
	\end{align}
 where $[\sigma_i = k] = 1$ if $\sigma_i = k$ and $0$, otherwise.
Here, $\theta \in \Theta = [0,1]^{N \times K}$ is a matrix of prediction probabilities, where the $i$th row is the vector of prediction probabilities $\theta_{i,0},\dots,\theta_{i,K-1}$ (with $\sum_{k \in \ZZZ_K} \theta_{i,k} = 1$) for the $i$th datapoint on classes $0,\dots,K-1$ respectively. 

With this definition, we can now describe our construction of a matrix $\theta \in [0,1]^{N \times K}$ that makes $\Klogloss$ function $2\tau $-codomain separable for any $\tau >0$ (i.e., $\Lambda_{\theta}(\Klogloss) \geq 2 \tau $). At a high level, we obtain the required codomain separability for $\Klogloss$ by designing the entries in the matrix $\theta$ in such a way that the expression inside the logarithm in~\eqref{eq:multi_class_log_loss} reduces to a distinct integer in some set. This calibration allows us to control the minimum difference in the output of the cross-entropy loss on different labelings, which we can scale to the desired amount ($\geq 2\tau$) easily. The following theorem summarizes our construction.  
% (see the Appendix for a detailed proof). 
\begin{theorem}\label{thm:multi_class_proof}
Let $\tau > 0$. Define matrices $\vartheta, \theta \in \mathbb{R}^{N \times K}$ such that $\vartheta_{n,k} = 3^{\paran{2^{(n-1)K+k}N\tau}}$ and $\theta_{n,k} = \vartheta_{n,k} / \sum_{k=1}^K \vartheta_{n,k}$. Then, it holds that $\Klogloss$ is $2 \tau $-codomain separable using $\theta$.
\end{theorem}
% \abhi{$\phi = O\paran{2^{NK}N\tau}$.
% N = 5, K = 2, tau = 0.01 => phi = 51.2}

The following corollary follows by combining the above result with Theorem~\ref{thm:inf}. 
\begin{corollary}
Using $\theta$ from Theorem~\ref{thm:multi_class_proof}, Algorithm~\LabelInf performs $\tau$-robust label inference from the K-ary cross-entropy loss ($\Klogloss$).
\end{corollary}
Note that Theorem~\ref{thm:multi_class_proof} only holds for the error $\tau >0$. However, as mentioned in Remark~\ref{rem:first}, in the unnoised case it suffices to instantiate Theorem~\ref{thm:multi_class_proof} with an arbitrarily small positive value of $\tau$. 
We bring to the reader's attention the doubly-exponential nature of the entries used to construct the prediction vector in Theorem~\ref{thm:multi_class_proof}. This blowup is unfortunately unavoidable for constructing $\tau$-codomain separability, even for the binary case, as shown in \citep[Theorem~7]{aggarwal2021icml}.
% Clearly, this will limit the practicality of the attack on real datasets (see our experiments in Section~\ref{sec:experiments}) due to limited floating-point precision. 
% A natural question to ask if there is a way to avoid such large entries when constructing a matrix $\theta$ for $2\tau$-separability of $\logloss$. This question was answered in the negative for the binary case in~\citep{aggarwal2021icml}, where it was shown that for any vector $v \in \mathbb{Q}^N$, if the binary log-loss admits $2\tau$-separability using $v \mapsto \frac{v}{1+v}$ (element-wise), then $\|v\|_\infty = \Omega(e^{2^N N\tau})$ must hold. By an easy extension to the multiclass case, this lower bound also holds for our use case and establishes the optimality of our construction in Theorem~\ref{thm:multi_class_proof}.

\noindent\textbf{Extensions of Cross-Entropy Loss.} Often in practice, when using the cross-entropy loss to assess the performance of ML models (like CNNs), it is common to apply an activation function (such as softmax or sigmoid) before the cross-entropy loss calculation. 
% The former compresses arbitrary reals into the range $(0,1)$, while the latter can convert any sequence of real outputs into a probability distribution.
% The outputs from the model do not necessarily represent probability distributions. In such cases, transformations are applied to these outputs before they can be fed into the cross-entropy loss computation. 
For example, a common idea in multiclass classification is to apply the softmax function (to convert any sequence of real outputs into a probability distribution),
% $\textsc{Softmax}:\mathbb{R}^K \to [0,1]^K$, that modifies any vector $\mathbf{v} = (v_1,\dots,v_K) \in \mathbb{R}^K$ using the transformation $v_i \mapsto \exp(v_i)/\sum_{j=1}^K \exp(v_j)$. 
% This leads to the softmax cross-entropy loss, $\textsc{Softmax-K-LLoss}:\ZZZ_K^N \times \mathbb{R}^{N \times K} \to \mathbb{R}$, 
defined as follows for $\sigma \in \ZZZ_K^N$, $\theta \in [0,1]^{N \times K}$:
\begin{align*}
 \frac{-1}{N}\sum_{i=1}^N \sum_{k=0}^{K-1} \ \Big([\sigma_i = k] \cdot \ln \textsc{softmax}(\theta_{i,k}) \Big), \mbox{ where } 
 \textsc{softmax}(\theta_{i,k}) = \exp(\theta_{i,k})/\sum_{j=1}^K \exp(\theta_{i,j}).
\end{align*}
We explain how to extend Theorem~\ref{thm:multi_class_proof} to obtain separability in this setting. Our idea is the following: (1) Let $\theta \in [0,1]^{N \times K}$ be the matrix from Theorem~\ref{thm:multi_class_proof}. Recall that by definition, $\theta$ is such that for each $i \in [N]$, the vector $\theta_i \in [0,1]^K$ is a probability distribution; (2) For each $i \in [N]$, solve the following (fully specified) system of equations for $\theta'_{i,k}$'s: for all $k \in \ZZZ_K , i \in [N]$: $\exp\paran{\theta'_{i,k}}/\sum_{j=1}^K \exp\paran{\theta'_{i,j}} = \theta_{i,k}$.
% \begin{align}
% \exp\paran{\theta'_{i,k}}/\sum_{j=1}^K \exp\paran{\theta'_{i,j}} = \theta_{i,k}.    
% \end{align}
This is a system of linear equations in the variables $\exp\paran{\theta'_{i,j}}$, for each $i \in [N]$, hence, can be solved in polynomial time using standard techniques. Once $\theta'$ is obtained, since $\textsc{softmax}(\theta'_{i,k}) = \theta_{i,k}$, from Theorem~\ref{thm:multi_class_proof}, we get that softmax cross-entropy loss is $2\tau $-codomain separable using $\theta'$; Algorithm~\LabelInf can now be used for $\tau$-label inference.

The separability from Theorem~\ref{thm:multi_class_proof} also holds if we apply any bijective activation function before applying the cross-entropy loss. As an example, consider the sigmoid cross-entropy commonly used in the binary classification setting (to compresses arbitrary reals into the range $(0,1)$), defined as follows for $\sigma \in \{0,1\}^N$, $\theta \in (0,1)^N$:
% 	\textsc{Sig-LLoss}\paran{\sigma, \theta} :=
\begin{align}
\label{eq:sigmoid_definition}
	 \frac{-1}{N}\sum_{i=1}^N \ \Big( \sigma_i \ln \paran{\textsc{Sigmoid}(\theta_i)} + (1-\sigma_i)\ln \paran{1-\textsc{Sigmoid}(\theta_i)} \Big),
\end{align}
where $\textsc{Sigmoid}(x) = \paran{1+e^{-x}}^{-1}$ is the sigmoid function. Since $\textsc{Sigmoid}:\mathbb{R} \to (0,1)$ is a bijection (and hence, invertible), given $\textsc{Sigmoid}(x) = y$, we can obtain $x = \ln (y/(1-y))$. Thus, given the matrix $\theta \in [0,1]^{N \times 2}$ from Theorem~\ref{thm:multi_class_proof}, we can construct $\theta' \in (0,1)^{N}$ such that $\theta'_{i} = \ln (\theta_{i,1}/(1-\theta_{i,1}))$ for all $i \in [N]$.
% respect to which   is $\tau$-codomain separable, we can obtain the vector $\theta'$ such that $\theta'_i = \ln (\theta_i/(1-\theta_i))$. 
 Once $\theta'$ is obtained, since $\textsc{Sigmoid}(\theta_{i}) = \theta_{i,1}$ and $1-\textsc{Sigmoid}(\theta_{i}) = \theta_{i,2}$  we get that sigmoid cross-entropy loss is $2\tau $-codomain separable using $\theta'$, and hence Algorithm~\LabelInf can be used for $\tau$-robust label inference.
 

% The bijection will ensure that the sigmoid cross-entropy loss is $\tau$-codomain separable with respect to $\theta'$, and hence, allows robust label inference. More generally, replacing $\textsc{Sig}$ with any injective function will behave similarly.

% Two commonly used examples of these transformations are the sigmoid activation and the Softmax computation. The former compresses arbitrary reals into the range $(0,1)$, while the latter can convert any sequence of real outputs into a probability distribution. We discuss the separability of cross-entropy scores obtained from such use cases and show, through a reduction to the multiclass case above, that robust label inference is possible for any amount of noise, as before.
% We consider extensions of this $\Klogloss$ to 

% \noindent\textbf{Softmax (Categorical) Cross-Entropy Loss.} For multiclass classification problems, often the outputs of the model are real numbers that do not necessarily form a probability distribution. The softmax function, denoted as $\textsc{Softmax}:\mathbb{R}^N \to [0,1]^N$, modifies any vector $\mathbf{v} = (v_1,\dots,v_N) \in \mathbb{R}^N$ using the transformation $v_i \mapsto \exp(v_i)/\sum_{j=1}^N \exp(v_j)$. Formally, $\textsc{SoftmaxLoss}:\{0,1\}^N \times \mathbb{R}^N \to \mathbb{R}$, is defined as:
% \begin{align}
% 	\label{eq:softmax_loss}
% 		\textsc{SoftmaxLoss}(\sigma,\theta) := \logloss\paran{\sigma;\{\textsc{Softmax}(\theta_i)\}_{i=1}^N}.
% \end{align}
% Now, to design a vector $\theta' \in \mathbb{R}^{N \times K}$ with respect to which $\textsc{SoftmaxLoss}(\sigma,\theta)$ is $\tau$-codomain separable (and hence, admits $\tau$-robust label inference by Proposition~\ref{prop:bound_on_tau_for_label_inference}), we provide the following general steps: (1) Let $\theta \in [0,1]^{N \times K}$ be the matrix from Theorem~\ref{thm:multi_class_proof}. Recall that by definition, $\theta$ is such that for each $i \in [N]$, the vector $\theta_i \in [0,1]^K$ is a probability distribution; (2) For each $i \in [N]$, solve the following (fully specified) system of equations: $\forall k \in \ZZZ_K.\ \ \ \frac{\exp\paran{\theta'_{i,k}}}{\sum_{k=1}^K \exp\paran{\theta'_{i,k}}} = \theta_{i,k}$. Note that this is a system of linear equations in the variables $\exp\paran{\theta'_{i,k}}$, which, for each $i \in [N]$, can be solved in polynomial time using standard techniques. Once $\theta'$ is obtained, robust label inference can be done using Algorithm~\LabelInf.



% \noindent\textbf{sigmoid (Cross-Entropy) Loss.} We discuss the binary case to explain the main idea behind our construction for this loss function. For the multiclass case, it is common to use Softmax instead of the sigmoid -- we will discuss the Softmax Loss in the next subsection. The sigmoid loss for the binary case, denoted $\textsc{SigLoss}:\{0,1\}^N \times \mathbb{R}^N \to \mathbb{R}$, is defined as follows:
% \begin{align}
% 	\label{eq:sigmoid_log_loss}
% 		\textsc{SigLoss}\paran{\sigma, \theta} := \frac{-1}{N}\sum_{i=1}^N \ \Big( \sigma_i \ln \paran{\textsc{Sigmoid}(\theta_i)} + (1-\sigma_i)\ln \paran{1-\textsc{Sigmoid}(\theta_i)} \Big),
% \end{align}

% \subsection{Computational Hardness of Robust Label Inference for Cross-Entropy Loss}

% \abhi{Use the lower bound in the ICML paper to argue that RLI is in EXP-TIME.}

% In this section, we prove that Robust-Label Inference for Cross-Entropy Loss is NP-Hard. We show this by reduction from the \textsc{Subset-Sum} problem. Note that it suffices to prove this hardness result for the binary case. This is in contrast to the polynomial time label inference algorithm provided in~\citep{aggarwal2021icml} for the un-noised setting, where the authors used a construction using prime numbers. 

% We begin by reminding the reader of the \textsc{Subset-Sum} problem. In this problem, we are given a set $S$ and a target sum $T$. The task is to output a subset of $S$ such that the sum of the elements in this subset is at most $T$. This problem is well known to be NP-complete. Thus, it suffices to provide a polynomial time reduction from the \textsc{Subset-Sum} problem into Robust Label Inference.

% We first perform some algebraic manipulation on the expression for Robust Label Inference from $\logloss$. For a fixed bound on the noise $\tau$, prediction vector $\theta$ (with respect to which the function $\logloss$ is $2\tau$-codomain separable) and observed loss $\ell$, we know that true labeling $\sigma \in \{0,1\}^N$ satisfies the condition 
% $\abs{\logloss(\sigma, \theta) - \ell} \leq \tau$. Moreover, $\sigma$ is the only labeling that satisfies this condition (from Proposition~\ref{prop:bound_on_tau_for_label_inference}). This inequality can be written as $\ell - \tau \leq \logloss(\sigma, \theta) \leq \tau + \ell$, and on expanding the $\logloss$ term, becomes the following:
% \begin{align*}
%     &\ell - \tau \leq -\frac{1}{N}\sum_{i=1}^N \paran{\sigma_i \ln \theta_i + (1-\sigma_i)\ln (1-\theta_i)} \leq \tau + \ell\\
%     \implies & \ell - \tau \leq \frac{1}{N}\sum_{i=1}^N \ln \parfrac{1}{1-\theta_i} +\frac{1}{N}\sum_{i=1}^N \sigma_i \ln \parfrac{1-\theta_i}{\theta_i} \leq \tau + \ell\\
%     \implies & N(\ell - \tau) - \ln \parfrac{1}{1-\theta_i} \leq \sum_{i=1}^N \sigma_i \ln \parfrac{1-\theta_i}{\theta_i} \leq N(\tau + \ell) - \ln \parfrac{1}{1-\theta_i}.
% \end{align*}
% It suffices to focus only on the inequality on the right above:
% $$\sum_{i=1}^N \sigma_i \ln \parfrac{1-\theta_i}{\theta_i} \leq N(\tau + \ell) - \ln \parfrac{1}{1-\theta_i}.$$
% To reduce the \textsc{Subset-Sum} problem for a given set $S = \{s_1,\dots,s_N\}$ and threshold $T$, we first set $\ln \parfrac{1-\theta_i}{\theta_i} = s_i$ to obtain $\theta_i = 1/(1+\exp(s_i))$. This will make $\sum_{i=1}^N \sigma_i s_i$ equivalent to selecting a subset from $S$, since $\sigma_i \in \{0,1\}^N$. Next, we set $T = N(\tau + \ell) - \ln \parfrac{1}{1-\theta_i}$, to obtain the following:
% $$\tau + \ell = \paran{T - s_i + \ln \paran{1+e^{s_i}}}/N.$$

% \abhi{Complete details here -- be careful about setting tau and ell -- ell must be such that (1) theta gives the required 2 tau separability and (2) ell must not be more than tau far away from the true loss. Mention that an FPTAS can be used for approximation here, but will need to work out the details here.}

==> AISTATS'22/neurips2021/plots.tex <==
\captionsetup[subfloat]{labelformat=empty}
\begin{figure*}[t]
    \centering
    \vspace{-0.5em}
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/logloss_titanic.png}}
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/logloss_iris.png}} 
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/logloss_satellite.png}} 
    \\[-3ex]
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_titanic.png}}
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_iris.png}} 
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_satellite.png}} 
    % \newline
    % \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_titanic.png}}
    % \hspace{-0.1em}
    % \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_iris.png}} 
    % \hspace{-0.1em}
    % \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_satellite.png}} 
    \vspace*{-3ex}
    \caption{Label reconstruction accuracy with multi-query label inference attack by performing Algorithm~\LabelInf on $M$ datapoints at a time using a total of $\lceil N/M \rceil$ queries. Here, $N$ is the total number of rows in the corresponding dataset (2201 for Titanic, 150 for Iris, and 6430 for Satellite).}
    \label{fig:multiquery}
    \vspace{2ex}
\end{figure*}

==> AISTATS'22/neurips2021/short_paper_discussion.tex <==
Informally, a loss function $(\sigma,\theta)\mapsto \mathbb{R}$ takes as input a labeling $\sigma \in \{0,1\}^N$ and a prediction vector $\theta \in [0,1]^N$ to produce a loss score in $\mathbb{R}$. For some $\tau > 0$, we call this function $\tau$-codomain separable if there exists some vector $\theta$ such that the output of the loss function (keeping $\theta$ fixed) on any two labelings differs by at least $\tau$. Thus, when $\theta$ is known, the one-one correspondence between the function's output and the labelings can be exploited for label inference (for example, through an exhaustive enumeration as in Algorithm~\LabelInf, Appendix~\ref{sec:prelim}) to exactly recover all the labels from just observing the output, which we refer to as \emph{robust label inference} (see Definition~\ref{def:robust_label_inference} in Appendix~\ref{sec:prelim}). A necessary and sufficient condition for inferring all ground truth labels from a loss function, noised upto $\tau$, is for this function to admit $2\tau$ codomain separability (see Proposition~\ref{prop:bound_on_tau_for_label_inference}).  
% (see Section~\ref{sec:linearly_separable}).

We say that a binary loss function $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ is linearly-decomposable in $\{0,1\}^N$ using some function $g:(0,1) \to \mathbb{R}$ if it can be expressed in the following form:
\begin{align}
f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i \in [N]:\sigma_i=1} g(\theta_i) + \sum_{i \in [N]:\sigma_i=0} g(1-\theta_i)}.    
\end{align}
Observe that the KL-divergence loss (which reduces to binary cross-entropy loss) is of this form, using $g(\theta_i) = -\ln \theta_i$ (see~\eqref{eq:KL}, Appendix~\ref{app:bregman}). Some other
common examples of linearly-decomposable losses include the (i) Itakura-Saito divergence loss, which can be expressed using $g(\theta_i) = 1/\theta_i + \ln \theta_i - 2$ (see~\eqref{eq:IS}, Appendix~\ref{app:bregman}); (ii) squared Euclidean loss, which can be expressed using $g(\theta_i) = (1-\theta_i)^2$, (see~\eqref{eq:sqEuc}, Appendix~\ref{app:bregman}); and, (iii) norm-like divergence loss, which can be expressed using $g(\theta_i) = 1 + (\alpha-1)\theta_i^\alpha - \alpha \theta_i^{\alpha-1} + (\alpha-1)(1-\theta_i)^\alpha$ for some $\alpha \ge 2$ (see~\eqref{eq:norm}, Appendix~\ref{app:bregman}).

Our main result for linearly decomposable loss functions is that for any deterministic function $g:[0,1] \to \mathbb{R}$ and any bound $\tau > 0$ on the noise, the function $f$ is $2\tau$-codomain separable if there exists $\theta \in (0,1)^N$ so that $g(\theta_i) - g(1-\theta_i) > 2^{i}N\tau$ for all $i \in [N]$ (see Theorem~\ref{thm:linear_separable}). Constructing such a vector $\theta$ can be done as follows: (1) Compute $x^*(y)$ as the solution to $g(x)-g(1-x) = y$; (2) If $x^*(y)$ exists, then set $\theta_i = x^*(2^iN\tau)$ for all $i \in [N]$. This vector $\theta$ can now be used for $\tau$-robust label inference from $f$ using Algorithm~\LabelInf (see detailed examples in Appendix~\ref{app:linearly_separable}). 
% However, such a $\theta$ might not exist for all loss functions, e.g., it does not exist for squared Euclidean and norm-like divergence losses, and we will deal those loss functions later. It does exist though for the Itakura-Saito divergence loss (defined in~\eqref{eq:IS}, Appendix~\ref{app:bregman}) -- we show that this loss is $2\tau$-codomain separable with $\theta_i = (1+3^{2^{i}N\tau})^{-1}$ (see Corollary~\ref{cor:IS}).
% mentioned earlier can satisfy the required condition in Theorem~\ref{thm:linear_separable} on $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$.
% \begin{corollary} \label{cor:IS}
% The Itakura-Saito divergence loss is $2\tau$-codomain separable with $\theta_i = (1+3^{2^{i}N\tau})^{-1}$.
% \end{corollary}


% For the Norm-like divergence loss, observe that $f(\sigma,\theta) < \alpha$ for all $\sigma,\theta$. Hence, this loss is not $\tau$-codomain separable for any $\tau \geq \alpha/(2N)$. Even when $\tau < \alpha/(2N)$, notice that for $\theta_i \in (0,1)$, we can write $g(\theta_i) - g(1-\theta_i) =  \alpha\paran{(1-\theta_i)^{\alpha-1} - \theta_i^{\alpha-1}} < \alpha$. Since $\alpha$ is a constant, there does not exist any $\theta_i$ for which $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$.

\noindent\textbf{Multi-Query Polynomial Time Attacks.} 
The linear-decomposability of $f$ allows for an efficient multi-query label inference algorithm for $f$. In particular, we could have a trade-off between the ability to perform  multiple queries with faster computation times to avoid an exhaustive search in the space of all labelings. 
% As noted in Section~\ref{sec:prelim}, whereas the optimization problem in Algorithm~\LabelInf can be naively solved using an exponential search over $\sigma$. 
To see this, observe that setting $\theta_i = 1/2$ gives $g(\theta_i) - g(1-\theta_i) = 0$. Thus, if we want to infer the first $M < N$ labels in a single query, we can set $\theta = [\theta_1,\dots,\theta_M,1/2,\dots,1/2]$ to obtain the following (with $\Lambda_\theta(f) := \min_{\sigma_1,\sigma_2} \abs{f(\sigma_1,\theta) - f(\sigma_2,\theta)}$ for brevity): 
% so that the following holds:
% \begin{align*}
%     f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i\leq M: \sigma(i)=1} (g(\theta_i)-g(1-\theta_i)) + \sum_{i=1}^M g(1-\theta_i) + \frac{(N-M)g(1/2)}{M}}.
% \end{align*}
% From this, we immediately obtain that:
\begin{align*}
    \Lambda_\theta(f) &= \frac{1}{N} \min_{\sigma_1,\sigma_2 \in \{0,1\}^N} \abs{\sum_{i\leq M:\sigma_1(i)=1}\paran{g(\theta_i)-g(1-\theta_i)} - \sum_{j\leq M:\sigma_2(j)=1}\paran{g(\theta_j)-g(1-\theta_j)}}.
\end{align*}
Similar to the discussion above, choosing $\theta_i$ that ensures $g(\theta_i)-g(1-\theta_i) > 2^iN\tau$ will ensure $\Lambda_\theta(f) > 2\tau$. Moreover, using this $\theta$ will ensure that if $f(\sigma_1,\theta) = f(\sigma_2,\theta)$, then $\sigma_1[:M] = \sigma_2[:M]$ must hold, so that after recovering the first $M$ labels, we can recover the next $M$ labels using $\theta = [1/2,\dots,1/2,\theta_{M+1},\dots,\theta_{2M},1/2,\dots,1/2]$, and so on. It immediately follows that a sufficient condition for $f$ to admit $\tau$-robust label inference with $\lceil N/M \rceil$ queries is for the inequality $g(x) - g(1-x) > 2^iN\tau$ to have a solution for all $i \in [N]$ (see Theorem~\ref{thm:multi_query_general}).
% % \input{neurips2021/single_query_plot}
% \begin{theorem}
% \label{thm:multi_query_general} 
% Let $g:[0,1] \to \mathbb{R}$ be some finite deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Then, for any $\tau > 0$ and integer $M \geq 1$, a sufficient condition for $f$ to admit $\tau$-robust label inference with $\lceil N/M \rceil$ queries is for the inequality $g(x) - g(1-x) > 2^iN\tau$ to have a solution for all $i \in [N]$.
% % there exist $x_1,\dots,x_M \in (0,1)$ such that $g(x_i) - g(1-x_i) > 2^iN\tau$ for all $i \in [M]$.
% \end{theorem}
More importantly, observe that an $\lceil N/M \rceil$-query algorithm for robust label inference will require $O(N2^M/M)$ local computations by the adversary (using Algorithm~\LabelInf in each query). Thus, while the single query case ($M = N$) required $O(2^N)$ computations, any multi-query algorithm using $M=O(\log N)$ requires only $O(\text{poly}(N))$ local computations, which allow a polynomial-time robust label inference. 

==> AISTATS'22/neurips2021/short_paper_experiments.tex <==
%\begin{table}[h]
%\begin{tabular}{lllp{3.5cm}p{2.6cm}} 
%\hline
% Loss & Data & Noise & Max. vector length for perfect label inference & Mean run time per inference (ms) \\ \hline
% Cross-entropy & Titanic & 0.0001 & 10 (15 by ICML) & 1.71 \\
% Cross-entropy &Titanic & 0.01 & 7 (9 by ICML)  & 0.20 \\
% Cross-entropy &Titanic & 0.1 & 5 (6 by ICML)  & 0.07 \\
% Cross-entropy & Titanic & 1 & 4 (4 by ICML) & 0.04 \\
% Cross-entropy & Iris & 0.0001 & 6 & 0.94 \\
% Cross-entropy & Iris & 0.01 & 4 & 0.10 \\
% Cross-entropy & Iris & 0.1 & 3 & 0.04 \\
% Cross-entropy & Iris & 1 & 2 & 0.02 \\
% Cross-entropy & Satellite & 0.0001 & 3 & 0.26\\
% Cross-entropy & Satellite & 0.01 & 2 & 0.08 \\
% Cross-entropy & Satellite & 0.1 & 1 & 0.05 \\
% Cross-entropy & Satellite & 1 & 1 & 0.05\\
% Sigmoid cross-entropy & ... & ... & 0 & \\
% Softmax cross-entropy & Titanic & 0.0001 & 7 & 2.07 \\
% Softmax cross-entropy & Titanic & 0.01 & 3 & 0.12 \\
% Softmax cross-entropy & Titanic & 0.1 & 1 & 0.05 \\
% Softmax cross-entropy &  Titanic & 1 & 0 & \\
% Softmax cross-entropy & Iris & 0.0001 & 3 & 0.25 \\
% Softmax cross-entropy & Iris & 0.01 & 1 & 0.03 \\
% Softmax cross-entropy & Iris & 0.1 or 1 & 0 & \\
% Softmax cross-entropy & Satellite & & 0 & \\
% \hline
%\end{tabular}
%\label{exp1}
%\end{table}
We now present our empirical evaluation of label inference attacks on cross-entropy loss and its extensions (see Appendix~\ref{app:experiments} for additional results)\footnote{All experiments are run on a 64-bit machine with 2.6GHz 6-Core processor, using the standard IEEE-754 double precision format. For reproducibility, the code is included as part of the supplementary material.}. We use the following datasets for our analysis. As our attacks construct prediction vectors that are independent of the dataset contents, we ignore the dataset features in our experiments. All the labels of the dataset are considered for the attack.
%\shiva{Zekun: can you upload all the plots as individual files, like in the ICML submission? That way we can set the spacing correctly.}
%\zeku{The individual figures are uploaded in the individual\_figure folder, with intuitive filenames. Please double check and rearrange as appropriate.}
\begin{CompactItemize}
    \item {\bf{Titanic}}~\cite{titanic}: a binary classification dataset (2201 rows) on the survival status of passengers.
    % , fetched from  \url{https://www.openml.org/d/40704}
    \item {\bf{Iris}}~\cite{iris}: a three-class classification dataset (150 rows) on the Iris species.
    \item {\bf{Satellite}}~\cite{satellite}: a six-class classification dataset (6430 rows) on the satellite images of soil.
\end{CompactItemize}
We consider three common loss functions (formally defined in Appendix~\ref{sec:logloss}): multiclass cross-entropy, softmax cross-entropy, and sigmoid cross-entropy (deferred to Appendix~\ref{app:experiments}). As a baseline, for the binary labeled dataset (Titanic) with the cross-entropy loss, we implemented the label inference attack of Aggarwal~\emph{et al.}\ \citep{aggarwal2021icml} (see Theorem~\ref{thm:from_icml}, Appendix~\ref{app:experiments} for a restatement of their main result).

We start with the distinction between our experiments and Algorithm~\LabelInf, which is presented in the $\textsc{APA}$ model\footnote{APA stands for Arbitrary Precision Arithmetic model (see Appendix~\ref{sec:apa_fpa}).}. For example in the multiclass cross-entropy loss (\Klogloss) case, to simulate Algorithm~\LabelInf on a finite precision machine, we must be able to differentiate $\min_{i,k}\theta_{i,k}$ from 0 (or else the label inference will be ambiguous). A rough analysis (from Theorem~\ref{thm:multi_class_proof}) gives that 
% $\min_{i,k}\theta_{i,k}\approx \vartheta_{N,1}/\vartheta_{N,K} = 3^{2^{(N-1)K+1}N\tau}/3^{2^{(N-1)K+K}N\tau}=\Omega(3^{-2^{NK}N\tau})$, which requires a precision of 
$\phi=\Omega(2^{NK}N\tau)$ bits are required to make this distinction. This bound hides constant factors and is likely not tight, but gives an idea of how arithmetic precision  plays a role in our experiments. 

Figure~\ref{fig:singlequery} shows the number of datapoints $N$ recovered by Algorithm~\LabelInf as we increase the noise for various loss functions. We sample 1000 random sets of labels each of length $N$ from the dataset here. At error magnitude $\tau = 1$, the noise is comparable to the actual loss function values computed. We measure accuracy as the percentage of labels correctly inferred out of $N$.
% (since the largest N for at least 50\% accuracy is 8 for sigmoid and softmax cross-entropy), 
Figure~\ref{fig:singlequery}(a) shows that the number of datapoints ($N$) for which 100\% label inference accuracy is achieved for cross-entropy loss decreases as the noise magnitude ($\tau$) increases, which is expected. Moreover, at the same noise magnitude, the accuracy also drops as the number of classes ($K$) increases from 2 (in Titanic) to 6 (in Satellite), which is also expected. These happen because of the dependence on number of datapoints and number of classes in our prediction vector construction (Theorem~\ref{thm:multi_class_proof}), which given fixed machine precision runs into representation issues. We note that for the Titanic dataset, the construction from~\cite{aggarwal2021icml} works slightly better (especially at lower $\tau$ values) than ours due to a small difference in the exponent: it holds that $\min_{i \in [N]}(-\ln \theta_{i}) = \Omega(2^N N\tau)$ in~\cite{aggarwal2021icml} (see Theorem~\ref{thm:from_icml}, Appendix~\ref{app:experiments}), but $\Omega(2^{2N}N\tau)$ when using Theorem~\ref{thm:multi_class_proof} with $K=2$.
% However, our construction is very general and extends to multiclass cross-entropy loss and beyond, which the construction in~\cite{aggarwal2021icml} does not handle.}. 

% Using the prediction vectors from Section~\ref{sec:logloss}, on these 1000 samples of length 8 from Titanic, the mean loss value is 3.64 for cross-entropy, 0.51 for sigmoid cross-entropy, and 0.81 for softmax cross-entropy.

% We further observe that for the Titanic dataset, the construction from~\cite{aggarwal2021icml} works slightly better (especially at lower $\tau$ values) than our construction provided by Theorem~\ref{thm:multi_class_proof}. This is due to a small difference in the exponent: we have $\min_{i \in [N]}\theta_{i} = \Omega(3^{-2^N N\tau})$ in~\cite{aggarwal2021icml} (see Appendix~\ref{app:experiments}), but $\Omega(3^{-2^{2N}N\tau})$ when using Theorem~\ref{thm:multi_class_proof} with $K=2$ (as mentioned above).
% On the other hand our construction is very general and extends to multiclass cross-entropy loss and beyond, which the construction in~\cite{aggarwal2021icml} does not handle.  

Figures~\ref{fig:singlequery}(b)-(c) show the number of datapoints on which Algorithm~\LabelInf achieves at least 50\% accuracy for cross-entropy and softmax cross-entropy loss. We notice this number is smaller for softmax cross-entropy as compared to regular cross-entropy (see Figure~\ref{fig:singlequery}(a)), which is also not surprising. Through a similar argument as that above for the number of bits required for cross-entropy loss, one can show that computing the softmax cross-entropy loss will require an additional $\Omega(NK + \ln(N\tau))$ bits (see the discussion in Appendix~\ref{app:experiments} for details). This additional requirement further constraints the number of labels that can be recovered with softmax cross-entropy loss.



% Finally, the longest computation time for a single label inference across all the experiments with $N=10$ is below 10 milliseconds. 
% In summary, our empirical results attest that these attacks can be performed effectively on real datasets, and also highlight some technical nuances when running label inference on machines with finite floating-point precision. 


% At $N=10$, $K=2$, and $\tau=0.0001$, this implies $\phi > 1000$. However, this upper bound is not tight, as we see in Figure \ref{fig:singlequery}(a) -- our 64-bit machine can perform perfect label inference on the Titanic dataset at noise 0.0001 for length 10. 

% We also ran a baseline label inference experiments on the Titanic dataset for cross-entropy, where the calibrated prediction vector $\theta$ from step 1 in Algorithm~\LabelInf is replaced by a uniformly random vector. We repeat the experiment 1,000 times and the maximum vector length at which 100\% accuracy is achieved is 3 and 1 at noise magnitude 0.0001 and 0.01, which are smaller than 10 and 8 by Algorithm~\LabelInf. When the noise magnitude increases to 0.1 and 1, the randomly generated vector cannot correctly infer label vector even at length 1 with 100\% accuracy.
% \abhi{Moving this closer to Algorithm~\LabelInf in the paper.}


 
 


 



%The median loss in the experiments is about 2.4 for cross-entropy (log-loss), 0.6 for sigmoid cross-entropy loss, and 1.12 for softmax cross-entropy loss. The longest run time for a single label inference across all the experiments based on Algorithm~\LabelInf in this section is below 10 milliseconds.
%\shiva{we need also results in all the plots for the unnoised case, maybe by setting $\tau$ to be extremely small}
 
%The fraction of correctly inferred labelings with respect to the length of the private vector is computed by running the label inference algorithm on 1000 labelings of each specific length randomly sampled from the corresponding dataset. 
 
%\shiva{This needs more discussion. Why is there a drop? Why does  Corollary~\ref{cor:APAFPA} not apply?}
 
%\shiva{can we show $9$ is almost close to what we expect based on the values? Remember the question in the ICML reviews which asked for something like this?}
%\shiva{Comparison to ICML does not show good results for us? We need to revisit this one?}





%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.26]{accuracy.png}
%    \caption{Results on  label inference using Algorithm~\LabelInf on the three real datasets: Titanic, Iris, and Satellite. The first row shows the performance of the label inference from log-loss. The second row shows the performance from sigmoid cross-entropy loss. The third row shows the performance from softmax cross-entropy loss. }
%    \label{accuracy}
%\end{figure}


%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.2]{binary_vs_icml.png}
%    \caption{Results comparing binary log-loss label inference using Algorithm~\LabelInf versus Algorithm 2 in ICML paper on the Titanic dataset. }
%    \label{binary_vs_icml}
%\end{figure}

%
%%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.2]{accuracy_multiquery.png}
%    \caption{Results on the multi-query label inference using Algorithm %\textsc{LabelInf} in shards from log-loss on the three real datasets: Titanic, Iris, and Satellite. }
%    \label{accuracy_multiquery}
%\end{figure}

==> AISTATS'22/neurips2021/short_paper_introduction.tex <==
Consider a situation where a machine learning (ML) modeler is interacting with a data curator. The data curator owns a private dataset for a classification task, and the curator agrees to evaluate on this private dataset the prediction vector (or an ML model) that the modeler submits, and replies back with loss function values. Such a situation is commonly encountered in machine learning competition settings like Kaggle~\cite{kaggle}, KDDCup~\cite{kdd_cup}, and ILSVRC Challenges~\cite{ilsvrc}. In some competitions, the features of the private (hold-out) dataset are revealed but not its labels, and the modeler submits the prediction vector on those features. In some other competitions, no information about the private dataset is revealed (i.e., neither the features nor the labels). The modeler submits a model that is then evaluated on the private dataset. In these settings, it is common for the curator to return the loss scores to the modeler (such as for the purposes of fine-turning the models or ranking etc.). A similar situation also appears when dealing with sensitive datasets, where either labels, or, both features and labels could be considered sensitive, and again a modeler and curator interact through loss scores. 

In this paper, we investigate if it is possible for a (malicious) modeler to recover all the private labels using these interactions with the data curator. 
% which has been split into a publicly available subset and a private subset. The curator exposes the public dataset for modelers to solve a classification task, which they can assess through interacting with the curator on the private dataset. For this evaluation, the modeler can submit their model predictions on the private dataset and the curator will reply with how accurate these predictions were, to help the modeler fine tune their model, as required. The labels for private dataset are never revealed to the modeler. Such a situation is commonly encountered in machine learning competition settings like Kaggle, KDDCup, and ILSVRC Challengs, where the modelers can only access the features in the private dataset but not its labels. 
More broadly, we investigate the problem of (robust) label inference, where the goal is to infer the labels of a hidden dataset from just the (noisy) loss function queries evaluated on the dataset. Our focus will be on a particularly strong inference attack where the modeler gets  {\em just one} loss query output, which could be distorted by noise. Surprisingly, we show that even with just this single query (and no access to the private feature set), for many common ML loss functions, our label inference attack succeeds in exactly recovering {\em  all} the true labels. This has important ramifications; for example, our attacks could be used by:
% \begin{list}{{\bf (\alph{enumi})}}
% 	{\usecounter{enumi}
% 		\setlength{\leftmargin}{14pt}
% 		\setlength{\listparindent}{14pt}
% 		\setlength{\parsep}{1pt}	
% }
% \item 
a) an unscrupulous participant to an ML competition who could learn the labels of the hold-out test set in order to construct a fake model that achieves perfect classification; or b) an adversary to execute a privacy breach by learning labels associated with a sensitive dataset (see our Ethics and Malpractice statement at the end).
% \footnote{See our ethics and malpractice statement at the end of this paper.\\} 
% \end{list}

% Through a notion of {\em codomain separability}, we characterize necessary and sufficient conditions for a loss function under which single query label inference is possible even with noisy responses. None of the presented attacks require any access to the private feature set or to any model training.

==> AISTATS'22/neurips2021/single_query_plot.tex <==
\begin{figure*}[t]
    \centering
    \vspace{-0.5em}
    \subfloat[]{\includegraphics[width=130pt]{neurips2021/individual_figure/logloss_100_singlequery.png}}
    \hspace{-0.1em}
    \subfloat[]{\includegraphics[width=130pt]{neurips2021/individual_figure/logloss_50_singlequery.png}} 
    \hspace{-0.1em}
    \subfloat[]{\includegraphics[width=130pt]{neurips2021/individual_figure/softmax_50_singlequery.png}}
    % \hspace{-0.1em}
    % \subfloat[]{\includegraphics[width=95pt]{individual_figure/softmax_50_singlequery.png}} 
    \vspace*{-1ex}
    \caption{Results for $\tau$-robust label inference using Algorithm~\LabelInf. Figures (a)-(b) plots the length of vector ($N$) on which Algorithm~\LabelInf always succeeds with multiclass cross-entropy loss with 100\%  and at least 50\% accuracy respectively. Here, Titanic$^{\star\star}$ implements the binary label inference attack proposed in~\cite{aggarwal2021icml}. Figure (c) plots the same for the softmax cross-entropy loss at 50\% accuracy (wherever computable). The computation time per inference attack is roughly 10 seconds.} 
    % \abhi{Reiterating Shiva's question here: Did we do multiple runs in these plots or just one run?}}
    \label{fig:singlequery}
    \vspace*{2ex}
\end{figure*}

==> AISTATS'22/overview.tex <==
\subsection{Reducing Robust Label Inference to Codomain Separability}
\label{sec:reduce_label_inference_to_codomain_separability}

\subsubsection{Connections to Blatant Non-Privacy}
\subsection{Results for Classes of Loss Functions}
\begin{theorem}[Additively Linearly Separable Losses]
\label{thm:linearly_separable_additive}
Let $\mathcal{L}:[0,1]^N \times \{0,1\}^N \to \mathbb{R}$ be a loss function such that for some invertible function $g:[0,1] \to \mathbb{R}$ and $h:[0,1]^N \to \mathbb{R}$, we can write:
$$\mathcal{L}(\theta,\sigma) = h(\theta) + \sum_{i=1}^N \sigma_i g(\theta_i).$$
Then, for given $\tau > 0$, the loss $\mathcal{L}$ is $\tau$-codomain separable using $\theta \in [0,1]^N$ with $\theta_i = g^{-1}(\tau \ln p_i)$, where $p_i$ denotes the $i^{th}$ prime number and assuming this inverse exists within the domain of $g$.
\end{theorem}

% \begin{theorem}[Multiplicatively Separable Losses]
% \label{thm:separable_multiplicative}
% Let $\mathcal{L}:[0,1]^N \times \{0,1\}^N \to \mathbb{R}$ be a loss function such that for some invertible function $g:[0,1] \to \mathbb{R}$ and $h:[0,1]^N \to \mathbb{R}$, we can write:
% $$\mathcal{L}(\theta,\sigma) = \prod_{i=1}^N \sigma_i g(\theta_i) + h(\theta).$$
% Then, for given $\tau > 0$, the loss $\mathcal{L}$ is $\tau$-codomain separable using $\theta \in [0,1]^N$ with $\theta_i = g^{-1}(p_i\tau)$, where $p_i$ denotes the $i^{th}$ prime number and assuming this inverse exists within the domain of $g$.
% \end{theorem}

\begin{theorem}[Bregman Divergence Based Losses]
\label{thm:bregman_general_result}
Let $F:[0,1] \times [0,1] \to \mathbb{R}$ be a strongly convex function and $DF(p,q) = F(p) - F(q) - \langle \nabla F(q),p - q\rangle$ be the Bregman divergence associated with $F$. Let $\mathcal{L}_F(\theta,\sigma)$ be the corresponding loss function, defined as follows:
$$\mathcal{L}_F(\theta,\sigma) = \frac{1}{N}\sum_{i=1}^N D_F([\sigma_i,1-\sigma_i], [\theta_i,1-\theta_i]).$$  
Then, the Bregman loss $\mathcal{L}_F(\theta,\sigma)$ is $\tau$-codomain separable for $\tau > 0$ using $\theta = [\theta_1,\dots,\theta_N]$ with the following:
$$\theta_i = \frac{N\tau \ln p_i + A}{B},$$
where $A = F([0,1]) + \langle \nabla F([1,0]), [1,-1] \rangle - F([1,0])$, and $B = \langle \nabla F([1,0]), [1,-1] \rangle-\langle \nabla F([0,1]), [1,-1] \rangle$ (assuming it is non-zero), and $p_i$ is the $i^{th}$ prime number.
\end{theorem}

\begin{theorem}[Composition with Inverse-Lipschitz Functions]
\label{thm:inverse_lipschitz}
Let $f:[0,1]^N \times \{0,1\}^N \to \mathbb{R}$ be $\tau$-codomain separable for some $\tau>0$ with respect to some $\theta \in [0,1]^N$. Let $g:\mathbb{R} \to \mathbb{R}$ be $k$-inverse Lipschitz for some constant $k > 0$. Then, the composition $g \circ f : [0,1]^N \times \{0,1\}^N \to \mathbb{R}$ is $k\tau$-codomain separable with respect to $\theta$.
\end{theorem}

% \subsection{Negative Results}
% \begin{theorem}
% \label{thm:lp_loss}
% For any $p > 0$, the function $f: \{0,1\}^N \times \{0,1\}^N \to \mathbb{R}$ of the form $f(\sigma,\theta) = \pnorm{p}{\theta-\sigma}$ is not $\tau$-codomain separable for any $\tau > 0$.
% \end{theorem}

% \begin{theorem}
% \label{thm:separability_monotonic}
% Let $\Omega = \{s_1,\dots,s_N\}$ be a set. Let $f: 2^\Omega \times \Theta \to \mathbb{R}_+$ be a function and $\theta \in \mathbb{R}^N$ be such that $f(\cdot,\theta)$ is monotonic, i.e.,, for all $A \subseteq B \subseteq [N]$, it holds that $f(A,\theta) \leq f(B,\theta)$. Then, $f$ is not $\tau$-codomain separable using $\theta$ for any 
% $$\tau > \min_{B \subset [N]}\min_{j \not\in B} \parfrac{f(B \cup \{j\},\theta) - f(B,\theta)}{2}.$$
% In particular, if $f(\emptyset,\theta) = 0$, then $f$ is not $\tau$-codomain separable using $\theta$ for any $\tau > \frac{1}{2} \paran{\min_{j \in [N]} f(\{j\},\theta)}$.
% \end{theorem}

% \begin{theorem}
% \label{thm:separability_monotonic_bounded}
% Let $\Omega = \{s_1,\dots,s_N\}$ be a set. Let $f: 2^\Omega \times \Theta  \to \mathbb{R}_+$ be a function such that $f(\cdot,\theta)$ is monotonic and $f(\cdot,\theta) \leq \beta$ for all $\theta \in \mathbb{R}^N$ and for some finite $\beta > 0$. Then, $f$ is not $\tau$-codomain separable for any $\tau > \beta/N$.
% \end{theorem}

% \subsection{Results on Computational Complexity and Model-Based Reconstruction}
% \begin{theorem}
% \textsc{Codomain-Separability} is Co-NP Hard.
% \end{theorem}

% \subsection{Model Based Reconstruction}

==> AISTATS'22/plots.tex <==
\captionsetup[subfloat]{labelformat=empty}
\begin{figure*}[t]
    \centering
    \vspace{-0.5em}
    \subfloat[]{\includegraphics[width=120pt]{neurips2021/individual_figure/titanic_itakura.png}} 
     \hspace{0.1em}
     \subfloat[]{\includegraphics[width=120pt]{neurips2021/individual_figure/softmax_titanic.png}}
     \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{neurips2021/individual_figure/mnist_softmax.png}} 
    \\[-3ex]
     \vspace{-0.8em}
    \subfloat[]{\includegraphics[width=120pt]{neurips2021/individual_figure/IMDB_itakura.png}} 
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{neurips2021/individual_figure/softmax_satellite.png}}  
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{neurips2021/individual_figure/cifar_softmax.png}} 
    % \newline
    % \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_titanic.png}}
    % \hspace{-0.1em}
    % \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_iris.png}} 
    % \hspace{-0.1em}
    % \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_satellite.png}} 
    \vspace*{-4ex}
    \caption{Label reconstruction accuracy with the multi-query label inference attack. As discussed in the text, for a given loss-function, we expect similar plots for any two datasets with same number of classes, e.g., Itakura-Saito for Titanic and IMDB, Softmax cross-entropy for MNIST and CIFAR. }
    \label{fig:multiquery}
    \vspace{-1.7em}
\end{figure*}

==> AISTATS'22/single_query_plot.tex <==
\begin{figure*}[t]
    \centering
    \vspace{-0.5em}
    \subfloat[]{\includegraphics[width=120pt]{neurips2021/individual_figure/itakura_single.png}}
    \hspace{-0.1em}
    \subfloat[]{\includegraphics[width=120pt]{neurips2021/individual_figure/logloss_100_single.png}}
    \hspace{-0.1em}
    \subfloat[]{\includegraphics[width=120pt]{neurips2021/individual_figure/logloss_50_single.png}} 
    \hspace{-0.1em}
    \subfloat[]{\includegraphics[width=120pt]{neurips2021/individual_figure/softmax_50_single.png}}
    % \hspace{-0.1em}
    % \subfloat[]{\includegraphics[width=95pt]{individual_figure/softmax_50_singlequery.png}} 
    \vspace*{-1ex}
    \caption{Results for single-query label inference. The Y-axis in Figures (a) and (b) represents the number of datapoints that can be recovered with 100\% accuracy, while for Figures (c) and (d), it represents the number of datapoints that can be recovered at 50\% accuracy, i.e., we recover at least this length vector accurately in at least 50\% of the 1000 runs.
    % Figure (a) plots the length of vector ($N$) on which Algorithm~\LabelInf always succeeds with Itakura-Saito loss. 
    % The results Figures (b)-(c) plots the same for multiclass cross-entropy loss with 100\%  and at least 50\% accuracy respectively. Here, Titanic$^{\star\star}$ implements the binary label inference attack proposed in~\cite{aggarwal2021icml}. Figure (d) plots the same for the softmax cross-entropy loss at 50\% accuracy (wherever computable).
    The max computation time per inference attack is roughly 10 seconds.} 
    \label{fig:singlequery}
    \vspace*{-1em}
\end{figure*}

==> AISTATS'22/supplement_experiments.tex <==
\section{Missing Details from Section~\ref{sec:experiments}}
\label{app:experiments}

\captionsetup[subfloat]{labelformat=empty}
\begin{figure*}[t]
    \centering
    \vspace{-0.5em}
    \subfloat[]{\includegraphics[width=150pt]{neurips2021/individual_figure/logloss_titanic.png}}
    \hspace{0.1em}
    %\subfloat[]{\includegraphics[width=150pt]{neurips2021/individual_figure/logloss_iris.png}} 
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=150pt]{neurips2021/individual_figure/logloss_satellite.png}} 
    \\
    \subfloat[]{\includegraphics[width=150pt]{neurips2021/individual_figure/mnist_cross_entropy.png}} 
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=150pt]{neurips2021/individual_figure/cifar_cross_entropy.png}}
    \vspace*{-3ex}
    \caption{Label reconstruction accuracy with the multi-query label inference attack.}
    \label{fig:logloss}
    \vspace{2ex}
\end{figure*} 

\begin{figure}[t]
    \centering
    \vspace{-0.5em}
    \subfloat[(a)]{\includegraphics[width=160pt]{neurips2021/individual_figure/sigmoid_50_singlequery.png}} 
    \hspace{2em}
    \subfloat[(b)]{\includegraphics[width=160pt]{neurips2021/individual_figure/sigmoid_titanic.png}}
    \vspace{-1ex}
    \caption{The plot on the left shows the length of vector recovered (at 50\% accuracy) using single query. The plot on the right shows label reconstruction accuracy with the multi-query label inference attack.}
    \label{fig:sigmoid_experiments}
       \vspace{1ex}
\end{figure}
 




We now discuss the missing details from Section~\ref{sec:experiments} and present our results for label inference from the Sigmoid cross entropy loss function.

% We begin with examining a multi-query label inference algorithm in Figure \ref{fig:multiquery}. For these plots, we simulated Algorithm~\LabelInf on $M < N$ datapoints at a time (instead of all $N$ datapoints at once), to obtain a total of $\lceil N/M\rceil$ queries. The idea is to use Figure~\ref{fig:singlequery} to determine the maximum number of labels that can be correctly inferred in a single query for a given noise level, and then perform label inference on only those many datapoints at a time. As expected, we observed that the accuracy increases with the number of queries: for cross-entropy loss on Titanic, we achieved 100\% accuracy using $M \geq 220$ with $\tau=0.0001$, and $M \geq 550$ with $\tau = 1$. The accuracy is again lower for the softmax case again due to reasons mentioned above.

\noindent\textbf{Label Inference from Binary Cross-Entropy Loss.} In our experiments, for binary cross-entropy, we use the label inference attack of \citep{aggarwal2021icml} as a baseline (see Figures~\ref{fig:singlequery}(a) and (b)). 

\begin{theorem}[$\tau$-codomain Separability from Algorithm 2 in~\citep{aggarwal2021icml}]\label{thm:from_icml}
Let $\tau > 0$. For the binary case (with class labels $0$ and $1$), define $\theta_i = \parfrac{3^{2^i}N\tau}{1+3^{2^i}N\tau}$ for all $i \in [N]$. Then, $\logloss$ is $2 \tau$-codomain separable using $\theta$.
\end{theorem}

Next, we discuss some technical caveats about the results for the softmax cross entropy loss, as observed in Figure~\ref{fig:singlequery}(d).  

\noindent\textbf{Additional bits Needed for Softmax Cross-Entropy Loss.} Recall from our discussion in Section~\ref{sec:experiments} that computing the softmax cross-entropy loss will require an additional $\Omega(NK + \ln(N\tau))$ bits over those required for the multiclass cross-entropy loss. We now formally argue this result.

Observe that for label inference in the softmax case, it suffices to compute a vector $\theta' = [\theta'_1,\dots,\theta'_N]$ such that $\textsc{Softmax}(\theta'_i) = \theta$, where $\theta$ is our desired vector for label inference. This is equivalent to requiring: $e^{\theta'_i}/\sum_j e^{\theta'_j} = \theta_i$, which gives rise to:
\[\frac{e^{x_1}}{\theta_1} = \cdots = \frac{e^{x_N}}{\theta_N}.\] 
Thus, for any $i$ and $j$, we can write $\theta'_i = \theta'_j + \ln \parfrac{\theta_i}{\theta_j}$. Now, let 
$$i_{\shortuparrow} = \arg\max_{i \in [N]}\theta_i \mbox{ and } i_{\shortdownarrow} = \arg\min_{i \in [N]}\theta_i.$$ 
Then, we can write $x_{i_{\shortuparrow}} = x_{i_{\shortdownarrow}} + \ln \parfrac{\theta_{i_{\shortuparrow}}}{\theta_{i_{\shortdownarrow}}}$. Thus, the additional number of bits required to represent the entries in $x$ is $\Omega\paran{\ln \ln \parfrac{\theta_{i_{\shortuparrow}}}{\theta_{i_{\shortdownarrow}}} - \ln \theta_{i_{\shortuparrow}}} = \Omega\paran{\ln \ln \parfrac{\theta_{i_{\shortuparrow}}}{\theta_{i_{\shortdownarrow}}}}$. From our construction in Theorem~\ref{thm:multi_class_proof}, we know that the ratio 
$\frac{\theta_{i_{\shortuparrow}}}{\theta_{i_{\shortdownarrow}}} \approx 3^{2^{NK}N\tau}$. This means that we need an additional $\Omega\paran{\ln \ln 3^{2^{NK}N\tau}} = \Omega\paran{NK + \ln (N\tau)}$ bits for the softmax cross-entropy loss as compared to the (plain) multiclass cross-entropy loss.

\textbf{Additional Experimental Results.} Figure \ref{fig:logloss} presents the results with multiclass cross-entropy loss on Titanic, Satellite, MNIST, and CIFAR datasets, using the same setting as in the multi-query experiments in Figure~\ref{fig:multiquery}.


% Similar to the softmax cross-entropy loss, we empirically examine label inference from the sigmoid activation performed prior to the cross-entropy calculation (see Figure~\ref{fig:sigmoid_experiments}).

 Figure~\ref{fig:sigmoid_experiments} presents the results on sigmoid cross-entropy which is applicable only in the binary labeled setting (see~\eqref{eq:sigmoid_definition}) on the Titanic dataset. 
%  We note that while~\eqref{eq:sigmoid_definition} guarantees 100\% accurate inference theoretically, this was not observed during our experiments (Figure~\ref{fig:sigmoid_experiments}(a)). 
The results are worse compared to (plain) multiclass cross-entropy loss.
This is because the number of bits required to represent $\textsc{Sigmoid}^{-1}(\theta_i)$ (where $\theta_i$ is an element of $\theta$) is $\Omega\paran{\ln\abs{\ln (\theta_i/(1-\theta_i))}}$, which asymptotically dominates the $\Omega\paran{\abs{\ln \theta_i}}$ many bits required to represent $\theta_i$ for the (plain) multiclass cross-entropy loss.



==> bregman.tex <==


 

% \begin{proof}
% See Appendix.
% \end{proof}

% Thus, a separating vector for the Bregman loss is obtained by setting $g(\theta_i) = \tau \ln p_i$, where $p_i$ is the $i^{th}$ prime number, as follows:
% \begin{align*}
%     &\frac{1}{N}\paran{\theta_i (a-b)+\phi(1)- \phi(0)-a} = \tau \ln p_i \\
%     \implies & \theta_i = \frac{N\tau \ln p_i + \phi(0) + a - \phi(1)}{a-b}.
% \end{align*}

% \subsection{Examples of Bregman Losses: Norm-Like Divergence Loss}
% The norm-like divergence based loss is defined with respect to $F(x,y) = x^\alpha + y^\alpha$, for some given $\alpha \geq 2$. Note that for $\alpha = 2$, this is the same as the Squared-Euclidean divergence based loss. From the definition of $F$, we obtain $\nabla F(x,y) = [\alpha x^{\alpha-1}, \alpha y^{\alpha-1}]$, and the constants required for the prediction vector computation as follows:
% \begin{align*}
%     \phi(0) &= F(0,1) = 1 = \phi(1)\\
%     a &= \langle \nabla F([1,0]), [1,-1] \rangle = \alpha, \text{and}\\
%     b &= \langle \nabla F([0,1]), [1,-1] \rangle = -\alpha.
% \end{align*}
% From this, we obtain that setting the prediction vector as follows suffices:
% $$\theta_i = \paran{N\tau \ln p_i +\alpha}/(2\alpha).$$
% Robust label inference can now be performed using Algorithm~\ref{alg:linearly_separable} (steps 2 through 5).

==> linearly_seperable_copy.tex <==
We begin our analysis with the discussion of an important class of (binary) loss functions, which we refer to as \emph{linearly-decomposable}. Loss functions in this class can be expressed as a sum of two terms: one corresponding to the datapoints that have label $1$ and the other for the datapoints with label $0$. As we will see, this decomposition allows an efficient construction of prediction vectors for robust label inference from such functions. We refer the reader to Appendix~\ref{app:linearly_separable} for missing proofs and technical details from this section.

\begin{definition}
\label{def:linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function. We say that a binary loss function $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ is linearly-decomposable in $\{0,1\}^N$ using $g$ if it can be expressed as follows:
\begin{align}
\label{eq:linear_separable}
f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i:\sigma_i=1} g(\theta_i) + \sum_{i:\sigma_i=0} g(1-\theta_i)}.    
\end{align}
\end{definition}

Observe that the KL-divergence loss (which reduces to binary cross-entropy loss) is of this form, using $g(\theta_i) = -\ln \theta_i$, which allows our results to subsume those presented by~\citep{aggarwal2021icml}. Some other
common examples of linearly-decomposable loss functions include the (i) Itakura-Saito divergence based loss, which can be expressed using $g(\theta_i) = 1/\theta_i + \ln \theta_i - 2$; (ii) squared Euclidean loss, which can be expressed using $g(\theta_i) = (1-\theta_i)^2$; and, (iii) norm-like divergence loss, which can be expressed using $g(\theta_i) = 1 + (\alpha-1)\theta_i^\alpha - \alpha \theta_i^{\alpha-1} + (\alpha-1)(1-\theta_i)^\alpha$ for some $\alpha \ge 2$. These loss functions are some popular instances of the general class of
Bregman divergence-based loss functions. The following lemma shows a general result that all Bregman divergence-based loss functions will satisfy this linearly-decomposability property.
\begin{lemma}
\label{lem:bregman_is_linear}
Let $F:[0,1] \times [0,1] \to \mathbb{R}$ be a strongly convex function and $D_F(p,q) = F(p) - F(q) - \langle \nabla F(q),p - q\rangle$ be the Bregman divergence associated with $F$. Let $f_F(\sigma,\theta)$ be the corresponding loss function, defined as follows:
$$f_F(\sigma,\theta) = \frac{1}{N}\sum_{i=1}^N D_F\paran{[\sigma_i,1-\sigma_i],[\theta_i,1-\theta_i]}.$$
Then, $f_F(\sigma,\theta)$ is linearly-decomposable. 
\end{lemma}
Note that unlike the distance metrics for probability distributions, Bregman divergence does not require its inputs to be necessarily distributions~\citep{bregman1967relaxation}. Thus, to use these divergences as loss functions (as is common, e.g.,~\citep{liu2016clustering}) one can directly compare the outputs of the ML model with the point distribution from the ground truth labels as we do in the definition of $f_F(\sigma,\theta)$. 



% ~\citep{bregman1967relaxation}We defer the details on our general result for $\tau$-codomain separability on Bregman divergence, including that for the Mahalanobis divergence loss (which is not linearly-decomposable) to Appendices~\ref{app:bregman} and~\ref{app:breg_general}. We also prove that the class of linearly-decomposable functions also contains all Bregman divergence based losses (see Appendix~\ref{sec:bregman_decomposable}).



\subsection{Establishing Codomain Separability}

\begin{theorem}
\label{thm:linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Then, for any $\tau > 0$, the function $f$ is $2\tau$-codomain separable if there exists $\theta \in (0,1)^N$ so that $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$.
\end{theorem}

Observe that Theorem~\ref{thm:linear_separable} immediately allows constructing a vector that will make a given linearly-decomposable function $f$ admit $\tau$-codomain separability for a given $\tau > 0$: (1) Compute $x^*(y)$ as the solution to $g(x)-g(1-x) = y$; (2) If $x^*(y)$ exists, then set $\theta_i = x^*(2^iN\tau)$ for all $i \in [N]$. This vector $\theta$ can now be used for $\tau$-robust label inference from $f$ using Algorithm~\LabelInf. However, such a $\theta$ might not exist for all loss functions, e.g., it does not exist for squared Euclidean and norm-like divergence losses, and we will deal those loss functions later. It does exist though for the Itakura-Saito divergence loss (defined in~\eqref{eq:IS}, Appendix~\ref{app:bregman}).
% mentioned earlier can satisfy the required condition in Theorem~\ref{thm:linear_separable} on $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$.
\begin{corollary} \label{cor:IS}
The Itakura-Saito divergence loss is $2\tau$-codomain separable with $\theta_i = (1+3^{2^{i}N\tau})^{-1}$.
\end{corollary}

\noindent\textbf{Linearly-Decomposable Functions Not Covered by Theorem~\ref{thm:linear_separable}.} We now deal with linearly-decomposable functions for whom there exists no $\theta$ that could satisfy the condition required in Theorem~\ref{thm:linear_separable} (examples include, squared Euclidean and norm-like divergence loss). Here, we establish the weaker \zero-codomain separability, which as discussed earlier suffices for label inference in the unnoised case. 

% \noindent\textbf{A Note on the \zero-Codomain Separability of Linearly-Decomposable Functions.} Observe that in Theorem~\ref{thm:linear_separable}, the condition on the function $g$ has a linear dependence on $\tau$, which will not suffice for label inference in the un-noised setting (where $\tau=0$). We state the result for this special case in the Theorem below\footnote{Note that while it is true that any vector with respect to which a function is $\tau$-codomain separable (for $\tau>0$) also allows \zero-codomain separability, we mention Theorem~\ref{thm:zero_codomain_linear_separable} to cover cases where $\tau$-codomain separability is hard to demonstrate (see the discussion about Norm-Like loss following the statemnt of Theorem~\ref{thm:zero_codomain_linear_separable}).} and show how it can be used to achieve \zero-codomain separability for the Square-Euclidean loss and the Norm-Like loss. 

\begin{theorem}
\label{thm:zero_codomain_linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Let $\theta \in (0,1)^N$ be some vector and $S_\theta = \{g(\theta_i) - g(1-\theta_i)\}_{i=1}^N$. Then, the function $f$ is \zero-codomain separable with respect to $\theta$ if $\mu(S_\theta)>0$, i.e., all subset sums in the set $S_\theta$ are distinct.
\end{theorem}
\begin{corollary} \label{cor:eucl}
The squared Euclidean loss  is  \zero-codomain separable using $\theta_i = (1/2)\paran{1-\ln(p_i)/N}$, where $p_i$ is the $i$th prime number for $i \in [N]$. The norm-like divergence loss for $\alpha \geq 2$ is \zero-codomain separable using $\theta$ that satisfies $(1-\theta_i)^{\alpha-1}-\theta_i^{\alpha-1} = (\ln p_i)/(N\alpha)$.
\end{corollary}
Finally, the idea behind the multi-query attack mentioned in Theorem~\ref{thm:multi_query_general} also extends to loss functions covered by Theorem~\ref{thm:zero_codomain_linear_separable}, thus, providing a multi-query polynomial time inference here as well. 

\subsection{Optimizing Robust Label Inference using Square Free Prime Factorization}

Our approach for $\tau$-robust label inference in this section will be to first demonstrate $2\tau$-codomain separability (as before), and then reduce the reconstruction of the true labels from noised loss score (using the separating prediction vector) to computing the closest square free integer of some real value. This algorithm runs in sub-exponential time, which is much faster than Algorithm~\LabelInf that uses exhaustive search. The main steps of our construction are provided in Algorithm~\ref{alg:linearly_separable} and outlined as follows.

Observe that any loss function of the form $f(\theta,\sigma) = \sum_{i=1}^N \paran{\sigma_i g(\theta_i) + (1-\sigma_i)h(\theta_i)}$ can be rewritten as $f(\theta,\sigma) = \Sigma_{i=1}^N \sigma_i g'(\theta_i) + \sum_{i=1}^N h(\theta_i)$, where $g'(\theta_i) = g(\theta_i)-h(\theta_i)$. For this section, we will generalize Definition~\ref{def:linear_separable} slightly to say that a loss function $f: \{0,1\}^N \times [0,1]^N \to \mathbb{R}$ is said to be linearly-decomposable if there exists some invertible function $g:[0,1] \to \mathbb{R}$ and some function $h:[0,1]^N \to \mathbb{R}$, such that we can write:
\begin{align}
    \label{def:sqfree_linearly_separable}
    f(\sigma,\theta) &= h(\theta) + \sum_{i=1}^N \sigma_i g(\theta_i) = h(\theta) + \sum_{i:\sigma_i=1} g(\theta_i).
\end{align}
This reformulation not only extends to a larger set of loss functions than those covered by Definition~\ref{def:linear_separable}, but also allows us to express the minimum codomain separation in $f$ (given a prediction vector $\theta$) in a way that obviates the connection to distinct subset sums:
\begin{align}
\label{eq:sqfree_min_separation}
    \Lambda_\theta(f) = \min_{\sigma_1 \ne \sigma_2}\abs{\sum_{i:\sigma_1(i)=1} g(\theta_i) - \sum_{i:\sigma_2(i)=1} g(\theta_i)}.
\end{align}
We can now analyze for robust label inference (given some bound $\tau > 0$ on the error) by selecting the elements of the set $g(\theta) := \{g(\theta_1),\dots,g(\theta_N)\}$ in a way that it has distinct subset sums and that the minimum difference of these subset sums is at least $2\tau$ (using Proposition~\ref{prop:bound_on_tau_for_label_inference}). While there are many ways in which $g(\theta)$ can be constructed (for example, using powers of 2, as was done in Theorem~\ref{thm:linear_separable}), we choose to set $g(\theta_i) = 3P\tau  \ln p_i$ (if possible to do so within the domain of $g$), where $p_i$ is the $i^{th}$ prime number and $P=\prod_{i=1}^N p_i$, is the product of the first $N$ primes. This particular choice of $g(\theta_i)$ ensures that each subset sum in the set $g(\theta)$ corresponds to the logarithm of a unique integer (using its prime factorization). 
\begin{lemma}
\label{lem:linearly_decomposable_using_primes}
Let $p_i$ is the $i^{th}$ prime number and $P=\prod_{i=1}^N p_i$, is the product of the first $N$ primes. Then, for any $\tau > 0$, setting $g(\theta_i)=3P\tau  \ln p_i$ for loss functions in Equation~\ref{def:sqfree_linearly_separable} ensures that $\Lambda_\theta(f) \geq 2\tau$. 
\end{lemma}
\begin{proof}
We prove this by substituting $g(\theta_i) = 6P\tau \ln p_i$ in Equation~\ref{eq:sqfree_min_separation} as follows:
\begin{align*}
    \Lambda_\theta(f) &= \min_{\sigma_1 \ne \sigma_2}\abs{\sum_{i:\sigma_1(i)=1} g(\theta_i) - \sum_{j:\sigma_2(j)=1} g(\theta_j)}\\
    &= (3P\tau)\ \min_{\sigma_1 \ne \sigma_2}\abs{\sum_{i:\sigma_1(i)=1} \ln p_i - \sum_{j:\sigma_2(j)=1} \ln p_j}\\
    &= (3P\tau)\ \min_{\substack{S_1,S_2 \subseteq [N]\\S_1 \cap S_2 = \emptyset}} \abs{\ln \parfrac{\prod_{i \in S_1}p_i}{\prod_{s \in S_2}p_j}} \geq 2\tau.
\end{align*}
Too see why the last inequality holds, let $S_1^*$ and $S_2^*$ denote the sets of primes that achieve the minimum value above. Then, without loss of generality, it must hold that $\prod_{j \in S_2^*}p_j \leq P$ and $\prod_{j \in S_2^*}p_j \leq 1 + \prod_{i \in S_1^*}p_i$. Thus, using the fact that $1.5x\ln \parfrac{1+x}{x} > 1$ for all $x \geq 1$, we obtain that $1.5P$ times the log expression above is at least $1$. Further scaling by $2\tau$ gives $\Lambda_\theta(f) \geq 2\tau$.
\end{proof}

Now that we have the desired codomain separation needed for $\tau$-robust label inference\footnote{For the unnoised case ($\tau$=0), a similar argument to that in Lemma~\ref{lem:linearly_decomposable_using_primes} can be used to show that $g(\theta_i)=\ln p_i$ suffices.}, we demonstrate how our choice of $g(\theta_i)$ in this section allows for label inference in sub-exponential time. To see this, we simplify the expression for the loss function as follows:
\begin{align*}
    f(\sigma,\theta) = h(\theta) + 3P\tau \ln \paran{\prod_{i:\sigma_i = 1}p_i}.
\end{align*}
We know that due to codomain separation, the labeling that minimizes the distance between the observed loss $\ell$ and the true loss $f(\sigma,\theta)$ above is exactly the ground truth labeling $\sigma^*$:
\begin{align*}
    \sigma^* &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\ell - \paran{h(\theta) + 3P\tau \ln \paran{\prod_{i:\sigma_i = 1}p_i}}} \\
    &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\parfrac{\ell - h(\theta)}{3P\tau} - \ln \paran{\prod_{i:\sigma_i = 1}p_i}}\\
    &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\ln \parfrac{\exp\parfrac{\ell - h(\theta)}{3P\tau}}{\prod_{i:\sigma_i = 1}p_i}}\\
    &= \arg\min_{\sigma \in \{0,1\}^N} \abs{\exp\parfrac{\ell - h(\theta)}{3P\tau} - \paran{\prod_{i:\sigma_i = 1}p_i}}.
\end{align*}

To obtain $\sigma^*$ from the equation above without using an exhaustive search over $\{0,1\}^N$, we observe that the expression inside the argmin essentially seeks a \emph{square-free} integer closest to some known real quantity. Once such an integer is obtained, its prime factors are in 1-1 correspondence with the indices in $\sigma^*$ that have label $1$. The problem of label inference on linearly-decomposable loss functions is, thus, reduced to the calculation of the nearest square-free integer to a given real number, which we discuss as follows. We use the Booker-Hiary-Keating algorithm from~\citep{Booker_2015} for checking square-freeness of integers in sub-exponential time\footnote{Strictly speaking, the Booker-Hiary-Keating algorithm for checking square-freeness of integers relies on the validity of the Generalized Reimann Hypothesis for Dirichlet L-functions to relax the dependence on integer factorization~\citep{Booker_2015}.}.

Recall that a positive integer $M$ is square-free if it doesn't have any repeated prime factors. Extending this definition, we say that $M$ is $n$-square-free if $M$ is square free and the largest prime factor of $M$ is at most $n^{th}$ prime number $p_n$. For example, $105 = 3 \times 5 \times 7$ is 4-square-free, since the largest prime factor of 105 is the 4$^{th}$ prime number (7), but it is not 3-square-free. We denote by $\textsc{SqFree}(m) = \{x:\text{$x$ is $m$-square-free}\}$ to be the set of all $m$-square-free positive integers. We denote the closest m-square-free number to $x$ as follows: 
$$\textsc{CloSqFree}(x,m) = \arg\min_{y \in \textsc{SqFree}(m)} |x-y|.$$ 

\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}

\begin{algorithm}[t]
\caption{\textsc{CloSqFree}$(x,m)$}\label{alg:closest_square_Free}
\vspace{0.5em}
If $x \leq 2$ or $m=2$, then \textbf{return} 2.

Let $p_i$ be the $i^{th}$ prime number. If $x < p_i$ for some $i > 1$, then \textbf{return} \textsc{CloSqFree}$(x,i-1)$.

If $p_1\cdots p_m \leq x$, then \textbf{return} $\lfloor x \rfloor$.

\For{$k=0,1,2,\dots,\lfloor x \rfloor-1$}{
If $\lfloor x \rfloor - k \in \textsc{SqFree}(m)$, then \textbf{return} $\lfloor x \rfloor - k$.

If $\lceil x \rceil + k \in \textsc{SqFree}(m)$, then \textbf{return} $\lceil x \rceil + k$.
}
\end{algorithm}

\begin{algorithm}[t]
\caption{Sub-Exponential Time Robust Label Inference for Linearly-Decomposable Loss Functions}
\label{alg:linearly_separable}
\vspace{0.5em}
\KwInput{$N$: number of datapoints, $\tau$: error bound}
\KwOutput{Labeling $\hat{\sigma} \in \{0,1\}^N$}
\vspace{0.5em}
Set $\theta_i \gets g^{-1}(3P\tau \ln p_i)$ (assuming the inverse exists), where $p_i = i^{th}$ prime and $P=p_1p_2\cdots p_N$.

Obtain the loss score $\ell$ using the vector $\theta$.

Let $A \gets \textsc{CloSqFree}\paran{\exp\paran{\frac{\ell - h(\theta)}{3P\tau}},N}$.

For $i\in [N]$, set $\hat{\sigma}_i \gets 1$ if $p_i$ divides $A$, else $\hat{\sigma}_i \gets 0$.

\textbf{Return} $\hat{\sigma}$ as the labeling.

\end{algorithm}

\subsection{Multi-Query Polynomial Time Attacks} 
The linear-decomposability of $f$ allows for an efficient multi-query label inference algorithm for $f$. In particular, we could have a trade-off between the ability to perform  multiple queries with faster computation times for solving the optimization problem solved in Step 3 of Algorithm~\LabelInf. 
% As noted in Section~\ref{sec:prelim}, whereas the optimization problem in Algorithm~\LabelInf can be naively solved using an exponential search over $\sigma$. 
To see this, observe that setting $\theta_i = 1/2$ gives $g(\theta_i) - g(1-\theta_i) = 0$. Thus, if we want to infer the first $M < N$ labels in a single query, we can set $\theta = [\theta_1,\dots,\theta_M,1/2,\dots,1/2]$ to obtain: 
% so that the following holds:
% \begin{align*}
%     f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i\leq M: \sigma(i)=1} (g(\theta_i)-g(1-\theta_i)) + \sum_{i=1}^M g(1-\theta_i) + \frac{(N-M)g(1/2)}{M}}.
% \end{align*}
% From this, we immediately obtain that:
\begin{multline*}
        \Lambda_\theta(f) = \frac{1}{N} \min_{\sigma_1,\sigma_2} |\sum_{i\leq M:\sigma_1(i)=1}\paran{g(\theta_i)-g(1-\theta_i)}    \\ 
    - \sum_{j\leq M:\sigma_2(j)=1}\paran{g(\theta_j)-g(1-\theta_j)}|.
\end{multline*}

Similar to Theorem~\ref{thm:linear_separable}, choosing $\theta_i$ that ensures $g(\theta_i)-g(1-\theta_i) > 2^iN\tau$ will ensure $\Lambda_\theta(f) > 2\tau$. Moreover, using this $\theta$ will ensure that if $f(\sigma_1,\theta) = f(\sigma_2,\theta)$, then $\sigma_1[:M] = \sigma_2[:M]$ must hold.  Note that after recovering the first $M$ labels, we can recover the next $M$ labels using $\theta = [1/2,\dots,1/2,\theta_{M+1},\dots,\theta_{2M},1/2,\dots,1/2]$, and so on. The result below immediately follows.

% \input{neurips2021/single_query_plot}

\begin{theorem}
\label{thm:multi_query_general} 
Let $g:[0,1] \to \mathbb{R}$ be some finite deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable using $g$. Then, for $\tau > 0$ and integer $M \geq 1$, a sufficient condition for $f$ to admit $\tau$-robust label inference with $\lceil N/M \rceil$ queries is for the inequality $g(x) - g(1-x) > 2^iN\tau$ to have a solution for all $i \in [N]$.
% there exist $x_1,\dots,x_M \in (0,1)$ such that $g(x_i) - g(1-x_i) > 2^iN\tau$ for all $i \in [M]$.
\end{theorem}
Observe that an $\lceil N/M \rceil$-query algorithm for robust label inference will require $O(N2^M/M)$ local computations by the adversary (using Algorithm~\LabelInf in each query). Thus, while the single query case ($M = N$) required $O(2^N)$ computations, any multi-query algorithm using $M=O(\log N)$ requires only $O(\text{poly}(N))$ local computations, which allow a polynomial-time robust label inference.

% \subsection{Bregman Divergence Loss Functions are Linearly Decomposable}
% \label{sec:bregman_is_linearly_decomposable}
% \input{bregman}

==> neurips2021/codomain_intro.tex <==
We begin our discussion by formally defining the notion of codomain separability and its connections to the problem of label inference in the noised and unnoised settings (missing details in Appendix~\ref{app:prelim}). 
% We defer all missing details from this section to the Appendix~\ref{app:prelim}.  

Our objects of interest are functions whose domain is the Cartesian product of the space of all labelings (defined by the  $\ZZZ_K^N = \ZZZ_K \times \dots \times \ZZZ_K \ \text{($N$ times)} = \{0,\dots,K-1\}^N$) and an arbitrary set $\Theta \subseteq \mathbb{R}^N$. Here, $K \geq 2$ represents the number of label classes.
% , for e.g., in the binary case $K =2$. 
This formulation captures the common scenario in machine learning, where we evaluate a loss function using the true labeling in $\ZZZ_K^N$ for $N$ datapoints based on a (prediction) vector in $\mathbb{R}^N$ generated by an ML model. $\Theta$ is the space of prediction vectors, and for $\theta =[\theta_1,\dots,\theta_N] \in \Theta$, the value of $\theta_i$ encodes the label prediction for the $i$th datapoint. For example, in the case of binary cross-entropy loss (log-loss), we have a prediction probability vector $\theta \in [0,1]^N$ and a labeling $\sigma \in \{0,1\}^N$; the loss on $(\sigma,\theta)$ is given by:
\begin{align}
    \label{eq:log_loss_defn}
    \logloss\paran{\sigma,\theta} = \frac{-1}{N}\ln \paran{\prod_{i=1}^N \theta_i^{\sigma_i}(1-\theta_i)^{1-\sigma_i}}.
\end{align}
In this case, $\theta_i$ is the probability assigned to the event $\sigma_i = 1$ by the ML model.
% As another example, consider another common loss function ....
% \shiva{Add another example that we consider.}
% As another example, consider another common loss function, the Kullback-Leibler loss (or KL-loss in short), which is defined as follows for $\theta \in [0,1]^N$ and $\sigma \in \{0,1\}^N$ (see~\citep{van2014renyi} for a primer on R\'enyi divergences):
% \begin{align}
%     \label{eq:kl_loss_defn}
%     \textsc{KL-Loss}(\sigma,\theta) = \sum_{i=1}^N \paran{\sigma_i \ln \frac{\sigma_i}{\theta_i} + (1-\sigma_i) \ln \frac{(1-\sigma_i)}{(1-\theta_i)}}.
% \end{align}
% More generally, the R\'enyi-Loss of order $\alpha \in (0,\infty)$ can be defined for $\theta \in [0,1]^N$ and $\sigma \in \{0,1\}^N$ as follows (for $\alpha = 1$ this is the same as the KL-loss above):
% \begin{align}
%     \label{eq:R\'enyi_loss_defn}
%     \textsc{R\'enyi-Loss}_\alpha(\sigma,\theta) = \frac{1}{\alpha-1}  \sum_{i=1}^N \ln   \paran{\sigma_i^\alpha \theta_i^{1-\alpha} + (1-\sigma_i)^\alpha (1-\theta_i)^{1-\alpha}}.
% \end{align}
We work with different loss functions that place different restrictions on $\Theta$. For example, in the case of multiclass cross-entropy loss (with $K$ classes), we have $\Theta \in [0,1]^{N \times K}$.  
% Note that different loss functions place different restrictions on $\Theta$ (i.e., $\Theta \in [0,1]^{N\times K}$, $\Theta \in \{0,1\}^N$, etc.). For the binary label case that we consider in this paper, we can convert $\theta \in [0,\infty)^N$ to $\theta' \in [0,1]^N$ by using the transformation $\theta_i' = \theta_i/(1+\theta_i)$. This is equivalent to saying that for the $i$th datapoint, the probability that it belongs to class $1$, as predicted by $\theta'$ is $\theta_i'$, and that for class $0$ is $1 - \theta_i' = 1/(1+\theta_i)$.

\noindent\textbf{Codomain Separability.} Informally, we call a function codomain separable if there exists some vector $\theta \in \Theta$ such that the function output on each $\ZZZ_K^N$  is distinct (keeping $\theta$ fixed). Thus, when $\theta$ is known, this one-one correspondence between the function's output and the labelings in $\ZZZ_K^N$ can be exploited to exactly recover all the labels from just observing the output.
% \footnote{Codomain separability differs from other notions of separability defined in the literature for functional analysis.}
% For example, multiplicatively separable functions $f(x,y)$ can be expressed as a product of two functions $f(x,y) = g(x)h(y)$, and additively separable functions satisfy $f(x,y) = g(x) 
% + h(y)$. Another important distinction we make is with hyperplane separability over sets of points in $\mathbb{R}^N$, which is a common notion in non-negative matrix factorization and image segmentation literature~\citep{arora2016computing,donoho2004does}.
% \shiva{Using \emph{\zero-codomain separability} to separate it from $\tau$-codomain separability?}
\begin{definition} [$\tau$-codomain separability]
\label{def:codomain_separability}
Let $f: \ZZZ_K^N \times \Theta \to \mathbb{R}$ be a function. For $\theta \in \Theta$, define $\Lambda_{\theta}(f) := \min_{\sigma_1,\sigma_2 \in \ZZZ_K^N} \abs{f(\sigma_1,\theta) - f(\sigma_2,\theta)}$ to be the minimum difference in the function output keeping $\theta$ fixed. For a fixed $\tau > 0$, we say that $f$ admits \emph{$\tau$-codomain separability} using $\theta$ if $\Lambda_{\theta}(f) \geq \tau$. In particular, we say that $f$ admits \emph{\zero-codomain separability} using $\theta$ if there exists any $\tau > 0$ such that $\Lambda_{\theta}(f) \geq \tau$. 
\end{definition}
Note that, for a fixed $\theta$, if a function is $\tau$-codomain separable, then it is also $\tau'$-codomain separable for $0 < \tau' < \tau$. Compared to $\tau$-codomain separability for $\tau >0$, the \zero-codomain separability is weaker as it only requires $\Lambda_{\theta}(f) > 0$. This condition is used for label inference in the unnoised case. 

As an example for $\tau$-codomain separability, consider the function 
% $f:\{0,1\}^N \times \mathbb{R}^N \to \mathbb{R}$, defined as 
$f(\sigma,\theta) = \langle \sigma, \theta \rangle$ for $\sigma \in \{0,1\}^N$. To demonstrate $\tau$-codomain separability, it suffices to set $\theta = [1,2,4,\dots,2^{N-1}]$. Using this, the output $f(\sigma,\theta)$ is the integer whose binary representation (in reverse) is given by the \emph{bits} defined in $\sigma$. Moreover, since the difference between any two integers that can be represented this way is one, it also holds that $\Lambda_\theta(f) = 1$, which makes $f$ admit $1$-codomain separability using $\theta$. Multiplying each entry in $\theta$ by $\tau$ will, thus, make $f$ admit $\tau$-codomain separability for any $\tau > 0$.

% As another example, consider the binary cross-entropy loss from~\eqref{eq:log_loss_defn}. The result \citep[Theorem~5]{aggarwal2020logloss} demonstrates a construction that for any $\tau > 0$ makes this loss $\tau$-codomain separable.

We highlight that in general, determining whether a loss function is codomain separable is co-NP-hard 
% (see Appendix~\ref{app:hardness_results}, where we provide a Karp reduction from the Tautology problem).
However, in the upcoming sections, we discuss our constructions that make many popular loss functions separable. In Appendix~\ref{sec:negative_results}, we present some function classes that are provably not $\tau$-codomain separable.   
% Our general goal will be to construct $\theta$'s that allows for separability with larger values of $\tau$ as that translates into label reconstruction attacks that can handle more noise.    
% Depending, on $f$, Note that $f$ may not be codomain separable using some other $\theta\in\Theta$. 
% Furthermore, for $\theta_1, \theta_2 \in \Theta$, each of which makes $f$ codomain separable, the corresponding $\tau$ can be different.

\noindent\textbf{Robust Label Inference.} Next, we formally define the problem of (robust) label inference from functions defined over the domain $\ZZZ_K^N \times \Theta$. Informally, the goal here is to recover some true labeling (in $\ZZZ_K^N$) upon observing only the function output, even if noised. We consider recovery from noised (perturbed) function outputs in this paper, and the results trivially holds for the unnoised case. 
% A particular focus will be on the binary label case.
%, when the latter is perturbed using some noise.
\begin{definition}[$\tau$-Robust Label Inference]
\label{def:robust_label_inference}
Let $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$ be a function. Let $\sigma^\star \in \ZZZ_K^N$ be an unknown true labeling. For a given $\tau > 0$, we say that $f$ admits $\tau$-robust label inference if there exists $\theta \in \Theta$ and an algorithm (Turing machine) $\mathcal{A}$ that can recover $\sigma^\star$ given any $\ell \in \mathbb{R}$ where $\abs{f(\sigma^\star,\theta) - \ell} < \tau$, \emph{i.e.,} for all $\sigma^\star \in \ZZZ_K^N$, we have $\mathcal{A}\paran{\theta, N, \ell} = \sigma^\star$.
% When $\ell = f(\sigma^\star,\theta)$ (the unnoised case), we say that $f$ admits label inference if there exists $\theta \in \Theta$ and an algorithm (Turing Machine) $\mathcal{A}$ that can recover $\sigma^\star$ given  $f(\sigma,\theta)$.
\end{definition}
Observe that the above definition can also work for the unnoised case by setting $\tau$ arbitrarily small. An important point to note here is that $\tau$-robust label inference requires perfect reconstruction of $\sigma^\star$, which is a {\em stronger} notion than that required by notions like {\em blatant non-privacy}~\citep{dinur2003revealing}, where the goal is to only reconstruct a good fraction of $\sigma^\star$. Also, while the above definition is based on a single query, we will later relax this requirement to study $\tau$-robust label inference under a multi-query model.  


The following simple proposition formally establishes the connection between the above definitions of separability and robust label inference. The proposition is stated for the noised setting. 
% For label inferences in the unnoised setting, it suffices that $f$ admits \zero-codomain separability.

\begin{proposition}\label{prop:bound_on_tau_for_label_inference}
A function $f$ admits $\tau$-robust label inference using $\theta \in \Theta$ if and only if $\Lambda_{\theta}(f) \geq 2\tau$. 
\end{proposition}


In a typical ML setting, assume that we have a server (machine) that holds a private labeled dataset with labels in $\sigma^\star \in \ZZZ_K^N$. Let $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$ denote a (classification) loss function. In Algorithm~\LabelInf, we present a general label inference technique based on Proposition~\ref{prop:bound_on_tau_for_label_inference}. The adversary picks $\theta \in \Theta$ based on Definition~\ref{def:codomain_separability}, to query the server, and gets back the noisy loss function value. It then iterates over the labelings to recover the closest one to the loss value. Throughout this paper, we assume that the adversary knows the loss function, number of datapoints $N$ and an upper bound $\tau$ on the resulting error. We also assume that the loss is computed on all labels in $\sigma^\star$. 




% The algorithm $\mathcal{A}$ (the adversary) has the freedom on choosing $\theta \in \Theta$. The adversary sends a prediction vector $\theta$ to a machine (server) that holds the (private) dataset $\sigma \in \{0,1\}^N$ and gets back the noisy loss function. 
% In the setting where the scores are noised, we assume that the adversary knows an upper bound on the resulting error. Often the former can be inferred from the knowledge of the precision on the machine that returns the loss score to the adversary.

 





% \abhi{Add details on a general Algorithm for Robust-Label Inference in the $\mathsf{APA}$ model.}
\renewcommand{\thealgocf}{}
\SetAlgoCaptionSeparator{}
       \begin{algorithm}[t]
        \SetAlgoLined
        \SetKwInput{KwData}{Input}
        \SetKwInput{KwResult}{Output}
        \SetKwInOut{Model}{Model Setting}
        \KwData{Number of datapoints $N$, bound on error (noise) $\tau > 0$}
        \KwResult{Recovered labels $\hat{\sigma}$}
        \Model{A server (oracle) with private dataset with true labels $\sigma^\star$}
        
        \smallskip
        Design a vector $\theta\in \Theta$ with respect to which $f$ admits $2\tau$-codomain separability (Definition~\ref{def:codomain_separability}).\\
        Query the server using $\theta$ as the prediction vector and observe output $\ell$ with $\abs{f(\sigma^\star,\theta) - \ell } < \tau$.\\
         \textbf{Return} $\hat{\sigma} \gets \arg\min_{\sigma\in \ZZZ_K^N} \abs{f(\sigma,\theta) -\ell}$.
        \caption{\LabelInf: Robust Label Inference for function $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$}
        \label{alg:general_label_inference}
        \end{algorithm}

\begin{remark} \label{rem:first}
A special case of Algorithm~\LabelInf is the unnoised setting, wherein $\ell = f(\sigma^\star,\theta)$. In that case, in Algorithm~\LabelInf, it suffices to design a vector  $\theta \in \Theta$ with respect to which $f$ admits \zero-codomain separability and $\tau$ plays no role (i.e., can be set to an arbitrarily small positive constant).
\end{remark}

An important feature about Algorithm~\LabelInf is that it makes just one call to the server to retrieve the (loss) function $f$ evaluated at a single $\theta$, but still reconstructs the entire private vector (see theorem below).\!\footnote{To baseline Algorithm~\LabelInf with a naive exponential search over the space of all labelings, we simulated label inference on the Titanic dataset (see Section~\ref{sec:experiments}) for the cross-entropy loss, by replacing the prediction vector $\theta$ from Step 1 in Algorithm~\LabelInf by a uniformly random vector in $[0,1]^N$. We observed that over 1000 independent runs, the randomly generated vector failed to correctly infer the true label for even a single datapoint at even mild noise levels ($\tau=0.1$ and higher).\\} We also note that the optimization problem $\arg\min_{\sigma\in \ZZZ_K^N} \abs{f(\sigma,\theta) -\ell}$ can be solved naively by an exponential search over all $\sigma$ in general, and  faster for certain functions under multiple-queries as we discuss in Section~\ref{sec:linearly_separable}. Even the exponential search is a local computation for the adversary.
% repeat the experiment 1,000 times and the maximum vector length at which 100\% accuracy is achieved is 3 and 1 at noise magnitude 0.0001 and 0.01, which are smaller than 10 and 8 by Algorithm~\LabelInf. When the noise magnitude increases to 0.1 and 1, the randomly generated vector cannot correctly infer label vector even at length 1 with 100\% accuracy.\\}. 
% The following theorem follows from the above discussion.
\begin{theorem} \label{thm:inf}
Let $f :\ZZZ_K^N \times \Theta \to \mathbb{R}$.
Algorithm~\LabelInf performs $\tau$-robust label inference on $f$, in that it recovers $\sigma^\star$ (i.e., $\hat{\sigma} = \sigma^\star$) from $
\ell$ where $\abs{f(\sigma^\star,\theta) - \ell } < \tau$.
\end{theorem}
\vspace*{-0.9ex}

\subsection{Separability in Arbitrary Precision vs.\ Finite Floating-Point Precision} 
\label{sec:apa_fpa}
One important consideration in our label inference attacks is the precision of arithmetic that is required at the adversary. In this context, there are two natural models of arithmetic computation: a) arbitrary precision and b) finite floating-point precision. Arbitrary precision arithmetic model allows precise arithmetic results even with very large numbers. In the floating-point precision model, the arithmetic is constrained by limited precision. An example of the floating-point precision model is the commonly used IEEE-754 double precision standard. Designing algorithms for standard arithmetic in both these models have been studied extensively~\citep{knuth2014art,brent2010modern}. Following~\citep{aggarwal2021icml}, we refer to the arbitrary precision arithmetic model as $\mathsf{APA}$ and floating point  arithmetic model with $\phi$ bits as $\mathsf{FPA}(\phi)$. 
% For simplicity, we assume in the $\mathsf{FPA}(\phi)$ model we have $1$ bit for sign, $(\phi-1)/2$ bits for the exponent and $(\phi-1)/2$ bits for the fractional part (mantissa). This assumption can be relaxed to accommodate $\phi_a > 0$ bits for the exponent and $\phi_b > 0$ bits for the fractional part where $\phi_a + \phi_b = \phi-1$.

% \abhi{Zekun, can you please convert the notations in this section from $f:\{0,1\}^N \times \Theta \to \mathbb{R}$ to $f: \{0,1\}^N \times \Theta \to \mathbb{R}$?}

% Our results on codomain separability hold under both these models of arithmetic. 
We begin by observing that Definition~\ref{def:codomain_separability} does not take into account fixed arithmetic precision (i.e., deals with the case where we have arbitrary precision arithmetic). Finite floating-point precision has an effect on separability, as bits of precision places a bound on the resolution. For example, even if $f(\sigma_1,\theta) \neq f(\sigma_2,\theta)$ in the $\mathsf{APA}$ model, with only $\phi$ bits of precision, this difference may not be observable. This leads to notion of separability in the $\mathsf{FPA}(\phi)$ model (formalized in Definition~\ref{def:FPA_codomain_separability}, Appendix~\ref{app:prelim}). 
Let $f_\phi$ be the representation of $f$ in the $\mathsf{FPA}(\phi)$ model.\!\footnote{Informally, representation in the $\mathsf{FPA}(\phi)$ model implies computing $f$ within the granularity defined by $\phi$, and reporting underflow/overflow when the results are out of range.} It is easy to show that if $f_\phi$ admits $\tau$-codomain separability using $\theta$, then $f$ also admits $\tau$-codomain separability in the $\mathsf{APA}$ model using $\theta$ (see Proposition~\ref{prop:FPAAPA}, Appendix~\ref{app:prelim}). The other direction is trickier, but we can establish that if $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using  $\theta$, then $f_\phi$ admits $\tau$-codomain separability using $\theta$ if $\phi\geq\max(2 \log_2 \tau  + 5,  -2\log_2\tau - 1)$ (see Proposition~\ref{prop:APAFPA}, Appendix~\ref{app:prelim}).   
% We examine the connection between separability in these two models as follows.
% \shiva{Add what Definition~\ref{def:codomain_separability} means in the $\textsc{FPA}(\phi)$ model in the appendix.}
% \noindent\textbf{Models of Computation.} We present our results in two models of arithmetic computation. The first model assumes \textit{arbitrary precision arithmetic}, which allows precise arithmetic results even with very large numbers. We refer to this as the 
% $\mathsf{APA}$ model. While this model results in considerably slower arithmetic~\citep{brent2010modern}, it helps an adversary to perform label inference with fewer queries.
% The second model is the more standard \textit{floating point precision model}, where the arithmetic is constrained by limited precision. We denote this model as $\mathsf{FPA}(\phi)$, where $\phi$ represents the number of bits of precision. We assume the following abstraction for the format for representing numbers in this model: 1 bit for sign, $(\phi-1)/2$ bits for the exponent and $(\phi-1)/2$ bits for the fractional part (mantissa).\footnote{More generally, one could allocate $\phi_a$ bits for the exponent and $\phi_b$ bits for the fractional part where $\phi_a + \phi_b = \phi-1$. This is the setting in our experiments.} This allows representing all numbers between $-2^{(\phi-1)/2}$ to $+2^{(\phi-1)/2}$, with a resolution of $2^{-(\phi-1)/2}$. The floating point precision model allows for more efficient arithmetic operations~\citep{brent2010modern}. We refer the reader to Chapter 4 in~\citep{ knuth2014art} for a detailed discussion on designing algorithms for standard arithmetic in these models.

% \begin{proposition} \label{prop:FPAAPA}
% Let $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$, $\theta \in \Theta$, and $\tau > 0$. Let $f_\phi$ be the representation of $f$ in the $\mathsf{FPA}(\phi)$ model\footnote{Informally, representation in the $\mathsf{FPA}(\phi)$ model implies computing $f$ within the granularity defined by $\phi$ (see the discussion before Proposition~\ref{prop:FPAAPA}), and reporting underflow/overflow when the results are out of range.}. If $f_\phi$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi)$ model (using $\theta$) for some $\phi > 0$, then $f$ also admits $\tau$-codomain separability in the $\mathsf{APA}$ model using $\theta$. Moreover, $f_{\phi'}$ also admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi')$ model using $\theta$ for all $\phi' > \phi$.
% \end{proposition}
% \begin{proof}
% Given $\theta$ and the fact that $f_\phi$ admits $\tau$-codomain separability using $\theta$ in the $\mathsf{FPA}(\phi)$ model, denote
% \begin{align*}
%     \Lambda_\theta(f_\phi) = \min_{\sigma_1,\sigma_2 \in \ZZZ_K^N} \abs{f_\phi(\sigma_1,\theta) - f_\phi(\sigma_2,\theta)} = b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} > 2\tau, 
% \end{align*}
% where each $b_i \in \{0,1\}$. Then, in the $\mathsf{FPA}(\phi+1)$ model, we can write (without loss of generality):
% \begin{align*}
%     \Lambda_\theta(f_{\phi+1}) &= \begin{cases}
%     0b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} &\ \ \text{if $\phi$ is even},\\
%     b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}}0&\ \ \text{if $\phi$ is odd}
%     \end{cases}\\
%      &= b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} > 2\tau,
% \end{align*}
% which establishes that $f_{\phi+1}$ is $\tau$-codomain separable using $\theta$ in the $\mathsf{FPA}(\phi+1)$ model. By induction, this implies that $f_{\phi'}$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi')$ model using $\theta$ for all $\phi' > \phi$. In the limit when $\phi \to \infty$, this is equivalent to saying that $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using $\theta$.
% \end{proof}

% \begin{proposition}
% For any function $f:\{0,1\}^N \times \Theta \to \mathbb{R}$ and $\theta \in \Theta$, it holds that for all $\tau \geq 0$, if $f$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi)$ model (using $\theta$) for some $\phi > 0$, then $f$ also admits $\tau$-codomain separability in the $\mathsf{APA}$ model using $\theta$. 

% Moreover, $f$ also admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi')$ model using $\theta$ for all $\phi' > \phi$.
% \end{proposition}
% \begin{proof}
% Given $\theta$ and the fact that $f$ admits $\tau$-codomain separability using $\theta$ in the $\mathsf{FPA}(\phi)$ model, denote
% \begin{align*}
%     \Lambda_\theta(f) = \min_{\sigma_1,\sigma_2} \abs{f(\sigma_1,\theta) - f(\sigma_2,\theta)} = b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} > 2\tau, 
% \end{align*}
% where each $b_i \in \{0,1\}$. Then, in the $\mathsf{FPA}(\phi+1)$ model, we can write (without loss of generality):
% \begin{align*}
%     \Lambda_\theta(f) &= \begin{cases}
%     0b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} &\ \ \text{if $\phi$ is even},\\
%     b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}}0&\ \ \text{if $\phi$ is odd}
%     \end{cases}\\
%      &= b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}} > 2\tau,
% \end{align*}
% which establishes that $f$ is $\tau$-codomain separable using $\theta$ in the $\mathsf{FPA}(\phi+1)$ model. By induction, this implies that $f$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi')$ model using $\theta$ for all $\phi' > \phi$. In the limit when $\phi \to \infty$, this is equivalent to saying that $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using $\theta$.
% \end{proof}
% We establish the correspondence in the other direction, starting from separability in the $\mathsf{APA}$ model.
% \begin{proposition} \label{prop:APAFPA}
% Let $f:\ZZZ_K^N \times \Theta \to \mathbb{R}$, $\theta \in \Theta$, and $\tau > 0$. Let $f_\phi$ be the representation of $f$ in the $\mathsf{FPA}(\phi)$ model.  If $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using some $\theta \in \Theta$ and for some $\tau > 0$, then $f_\phi$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi)$ model using $\theta$ for $\phi\geq\max(2 \log_2 \tau  + 5,  -2\log_2\tau - 1)$.
% \end{proposition}
% \begin{proposition} \label{prop:APAFPA}
% For any function $f:\{0,1\}^N \times \Theta \to \mathbb{R}$, it holds that, if $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using some $\theta \in \Theta$ and for some $\tau > 0$, then $f_\phi$ admits $\tau$-codomain separability in the $\mathsf{FPA}(\phi)$ model using $\theta$ for $\phi\geq\max(2 \log_2 \tau  + 5,  -2\log_2\tau - 1)$.
% \end{proposition}
% \shiva{Not following the proof. There is some missing min in the condition on $\phi$?}
% Similar to the proof above, denote (in the $\mathsf{APA}$ model) the following:
% \begin{align*}
%     \Lambda_\theta(f) = b_m\cdots b_1 b_0\ .\ b_{-1}b_{-2}b_{-3} \cdots,
% \end{align*}
% for some finite $m > 0$ (\zeku{should we also capture the floating point precision after the decimal point, i.e. $0.b_{-1}b_{-2}...b_{-m}$?}). \abhi{In the APA model, we have infinite precision.\zeku{I see. For example, if $f$ is $\tau$-codomain separable in APA for some tiny $\tau$, where $\lfloor \log_2\tau\rfloor < -5$, does it mean it is also $\tau$-codomain separable in FPA(1)?}} \abhi{Hmm.. good point. We need to check this corner case. I will think more about it. Thanks!} Since $\Lambda_\theta(f) > 2\tau$, it must be the case that $m \geq \lfloor \log_2 (2\tau) \rfloor = 1 + \lfloor \log_2 \tau \rfloor$. Thus, if $f$ has to admit $\tau$-codomain separability in the $\mathsf{FPA}(\phi)$ model using $\theta$, we must have $\frac{\phi-3}{2} \geq m$, which gives $\frac{\phi-3}{2} \geq m \geq 1 + \lfloor \log_2 \tau \rfloor \Longrightarrow \phi \geq 2\lfloor \log_2 \tau \rfloor + 5$. \abhi{Shiva, please check this proof.}
% \end{proof}
% \shiva{it will be good to have an corollary about the condition on $\tau$ in terms of $\phi$}
% \abhi{Talk about polytime inference in FPA model vs. APA model.}
% \zeku{Proposed revised proof for Proposition 2.}
% \begin{proof}
% Suppose $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model. To establish $f_\phi$ as $\tau$-codomain separability in $\mathsf{FPA}(\phi)$, we need to split the two cases: $\tau>1$ and $\tau<1$.
% Represent $\Lambda_{\theta}(f_\phi)$ in $\mathsf{FPA}(\phi)$ as 
% $$b_{\frac{\phi-3}{2}}\cdots b_1 b_0\ .\ b_{-1}b_{-2} \cdots b_{-\frac{\phi-1}{2}}.$$
% When $\tau>1$, a sufficient condition for $f_\phi$ to satisfy the $\tau$-codomain separability is to have enough precision before the decimal point,
% $$2^{\frac{\phi-3}{2}}\geq 2\tau,$$
% which gives $\frac{\phi-3}{2}  \geq 1 + \log_2 \tau  \Longrightarrow \phi \geq 2 \log_2 \tau  + 5$. When $\tau<1$, a sufficient condition for $f_\phi$ to satisfy $\tau$-codomain separability is to have enough precision after the decimal point,
% $$2^{-\frac{\phi-1}{2}}\leq 2\tau,$$
% which gives $-\frac{\phi-1}{2}\leq 1 +  \log_2 \tau \Longrightarrow \phi \geq -2\log_2\tau - 1$. The proposition follows from combining the two together to obtain $\phi\geq\max(2 \log_2 \tau  + 5,  -2\log_2\tau - 1)$.
% \end{proof}

% \abhi{I think this looks good. Thanks Zekun! Shiva, can you please proof read this as well? Thanks!}
% \begin{corollary} \label{cor:APAFPA}
% For any function $f_\phi:\ZZZ_K^N \times \Theta \to \mathbb{R}$, $f_\phi$ admits $\tau$-codomain separability using $\theta \in \Theta$ in the $\mathsf{FPA}(\phi)$ model for $\phi \geq 5$ if both the following two conditions hold:
% \begin{CompactEnumerate}
%     \item $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using some $\theta \in \Theta$, and
%     \item It holds that $2^{-\parfrac{\phi+1}{2}} \leq \tau \leq 2^{\parfrac{\phi-5}{2}}$.
% \end{CompactEnumerate}
% \end{corollary}
% \begin{corollary} \label{cor:APAFPA}
% For any function $f:\{0,1\}^N \times \Theta \to \mathbb{R}$, $f$ admits $\tau$-codomain separability using $\theta \in \Theta$ in the $\mathsf{FPA}(\phi)$ model for $\phi \geq 5$ if both the following two conditions hold:
% \begin{enumerate}
%     \item $f$ admits $\tau$-codomain separability in the $\mathsf{APA}$ model using some $\theta \in \Theta$, and
%     \item it holds that $2^{-\parfrac{\phi+1}{2}} \leq \tau \leq 2^{\parfrac{\phi-5}{2}}$.
% \end{enumerate}
% \end{corollary}
% \shiva{Misleading:
% Given these above conditions, it follows that an inference attack in the $\mathsf{APA}$ model outlined in Algorithm~\LabelInf, also succeeds in the $\mathsf{FPA}(\phi)$ model if $\max_\sigma |f(\sigma,\theta)|\leq 2^{\frac{\phi-3}{2}}$. \abhi{Zekun, please add one line to explain this.}}
% Now, given a $\tau$-robust label inference algorithm in $\mathsf{APA}$ model using $\theta$, if condition 2 in Corollary 1 holds,  then we can run the algorithm as is to perform $\tau$-robust label inference in $\mathsf{FPA}(\phi)$ model. 
% \abhi{Zekun, please verify that running the algorithm in FPA will not need any additional bits than what is required by Prop 2.}
% Given these above conditions, it follows that an inference attack in the $\mathsf{APA}$ model outlined in Algorithm~\LabelInf, also succeeds in the $\mathsf{FPA}(\phi)$ model. 
Moving to label inference, note that Algorithm~\LabelInf is also described in the $\textsc{APA}$ model. The above mentioned bound on $\phi$ may not suffice for $\tau$-robust label inference using Algorithm~\LabelInf in the $\mathsf{FPA}(\phi)$ model. This is because unlike codomain separability, Algorithm~\LabelInf requires the adversary to compute the loss function on all labelings of the datapoints, which may require additional bits. For example, the prediction vector we provide for multiclass cross-entropy loss in Theorem~\ref{thm:multi_class_proof} contains entries that are doubly-exponential in $N$ (number of  datapoints) and $K$ (number of classes). This would prohibit the correct computation of loss scores beyond some values of $N$ and $K$ in the $\mathsf{FPA}(\phi)$ model. However, this issue could be overcome by the ability to perform multiple queries that we utilize in our experimental evaluation in Section~\ref{sec:experiments}. For simplicity of description, we present our inference attacks under the $\mathsf{APA}$ model in the main body of this paper.

% \shiva{Say what this above corollary really means, and whether what can we expect Algorithm~\LabelInf to do in the $\mathsf{FPA}(\phi)$ model that is consistent with what we observe in expts.} \abhi{I'll need some help on the best way to frame this. Perhaps we can discuss in the meeting today.}
% For simplicity of description, we present our inference attacks under the $\mathsf{APA}$ model. Our experimental results, however, utilize standard double precision format arithmetic (IEEE 754 standard). 

% \subsection{Some Caveats about Single-query vs. Multi-query (Robust) Label Inference}
% In this section, we discuss some caveats associated with converting a single-query robust label inference algorithm into a multi-query algorithm. We also provide sufficient conditions under which this conversion can be done efficiently. \abhi{TODO.}

==> neurips2021/experiments.tex <==
%\begin{table}[h]
%\begin{tabular}{lllp{3.5cm}p{2.6cm}} 
%\hline
% Loss & Data & Noise & Max. vector length for perfect label inference & Mean run time per inference (ms) \\ \hline
% Cross-entropy & Titanic & 0.0001 & 10 (15 by ICML) & 1.71 \\
% Cross-entropy &Titanic & 0.01 & 7 (9 by ICML)  & 0.20 \\
% Cross-entropy &Titanic & 0.1 & 5 (6 by ICML)  & 0.07 \\
% Cross-entropy & Titanic & 1 & 4 (4 by ICML) & 0.04 \\
% Cross-entropy & Iris & 0.0001 & 6 & 0.94 \\
% Cross-entropy & Iris & 0.01 & 4 & 0.10 \\
% Cross-entropy & Iris & 0.1 & 3 & 0.04 \\
% Cross-entropy & Iris & 1 & 2 & 0.02 \\
% Cross-entropy & Satellite & 0.0001 & 3 & 0.26\\
% Cross-entropy & Satellite & 0.01 & 2 & 0.08 \\
% Cross-entropy & Satellite & 0.1 & 1 & 0.05 \\
% Cross-entropy & Satellite & 1 & 1 & 0.05\\
% Sigmoid cross-entropy & ... & ... & 0 & \\
% Softmax cross-entropy & Titanic & 0.0001 & 7 & 2.07 \\
% Softmax cross-entropy & Titanic & 0.01 & 3 & 0.12 \\
% Softmax cross-entropy & Titanic & 0.1 & 1 & 0.05 \\
% Softmax cross-entropy &  Titanic & 1 & 0 & \\
% Softmax cross-entropy & Iris & 0.0001 & 3 & 0.25 \\
% Softmax cross-entropy & Iris & 0.01 & 1 & 0.03 \\
% Softmax cross-entropy & Iris & 0.1 or 1 & 0 & \\
% Softmax cross-entropy & Satellite & & 0 & \\
% \hline
%\end{tabular}
%\label{exp1}
%\end{table}
We now present our empirical evaluation of label inference attacks on cross-entropy loss and its extensions (see Appendix~\ref{app:experiments} for additional results)\footnote{All experiments are run on a 64-bit machine with 2.6GHz 6-Core processor, using the standard IEEE-754 double precision format. For reproducibility, the code is included as part of the supplementary material.}. We use the following datasets for our analysis. As our attacks construct prediction vectors that are independent of the dataset contents, we ignore the dataset features in our experiments. All the labels of the dataset are considered for the attack.
%\shiva{Zekun: can you upload all the plots as individual files, like in the ICML submission? That way we can set the spacing correctly.}
%\zeku{The individual figures are uploaded in the individual\_figure folder, with intuitive filenames. Please double check and rearrange as appropriate.}
\begin{CompactItemize}
    \item {\bf{Titanic}}~\cite{titanic}: a binary classification dataset (2201 rows) on the survival status of passengers.
    % , fetched from  \url{https://www.openml.org/d/40704}
    \item {\bf{Iris}}~\cite{iris}: a three-class classification dataset (150 rows) on the Iris species.
    \item {\bf{Satellite}}~\cite{satellite}: a six-class classification dataset (6430 rows) on the satellite images of soil.
\end{CompactItemize}
We consider three common loss functions mentioned in Section~\ref{sec:logloss}: multiclass cross-entropy, softmax cross-entropy, and sigmoid cross-entropy (deferred to Appendix~\ref{app:experiments}). As a baseline, for the binary labeled dataset (Titanic) with the cross-entropy loss, we implemented the label inference attack of Aggarwal~\emph{et al.}\ \citep{aggarwal2021icml} (see Theorem~\ref{thm:from_icml}, Appendix~\ref{app:experiments} for a restatement of their main result).

We start with the distinction between our experiments and Algorithm~\LabelInf, which is presented in the $\textsc{APA}$ model. For example in the multiclass cross-entropy loss (\Klogloss) case, to simulate Algorithm~\LabelInf on a finite precision machine, we must be able to differentiate $\min_{i,k}\theta_{i,k}$ from 0 (or else the label inference will be ambiguous). A rough analysis (from Theorem~\ref{thm:multi_class_proof}) gives that 
% $\min_{i,k}\theta_{i,k}\approx \vartheta_{N,1}/\vartheta_{N,K} = 3^{2^{(N-1)K+1}N\tau}/3^{2^{(N-1)K+K}N\tau}=\Omega(3^{-2^{NK}N\tau})$, which requires a precision of 
$\phi=\Omega(2^{NK}N\tau)$ bits are required to make this distinction. This bound hides constant factors and is likely not tight, but gives an idea of how arithmetic precision  plays a role in our experiments. 

Figure~\ref{fig:singlequery} shows the number of datapoints $N$ recovered by Algorithm~\LabelInf as we increase the noise for various loss functions. We sample 1000 random sets of labels each of length $N$ from the dataset here. At error magnitude $\tau = 1$, the noise is comparable to the actual loss function values computed. We measure accuracy as the percentage of labels correctly inferred out of $N$.
% (since the largest N for at least 50\% accuracy is 8 for sigmoid and softmax cross-entropy), 
Figure~\ref{fig:singlequery}(a) shows that the number of datapoints ($N$) for which 100\% label inference accuracy is achieved for cross-entropy loss decreases as the noise magnitude ($\tau$) increases, which is expected. Moreover, at the same noise magnitude, the accuracy also drops as the number of classes ($K$) increases from 2 (in Titanic) to 6 (in Satellite), which is also expected. These happen because of the dependence on number of datapoints and number of classes in our prediction vector construction (Theorem~\ref{thm:multi_class_proof}), which given fixed machine precision runs into representation issues. We note that for the Titanic dataset, the construction from~\cite{aggarwal2021icml} works slightly better (especially at lower $\tau$ values) than ours due to a small difference in the exponent: it holds that $\min_{i \in [N]}(-\ln \theta_{i}) = \Omega(2^N N\tau)$ in~\cite{aggarwal2021icml} (see Theorem~\ref{thm:from_icml}, Appendix~\ref{app:experiments}), but $\Omega(2^{2N}N\tau)$ when using Theorem~\ref{thm:multi_class_proof} with $K=2$.
% However, our construction is very general and extends to multiclass cross-entropy loss and beyond, which the construction in~\cite{aggarwal2021icml} does not handle.}. 

% Using the prediction vectors from Section~\ref{sec:logloss}, on these 1000 samples of length 8 from Titanic, the mean loss value is 3.64 for cross-entropy, 0.51 for sigmoid cross-entropy, and 0.81 for softmax cross-entropy.

% We further observe that for the Titanic dataset, the construction from~\cite{aggarwal2021icml} works slightly better (especially at lower $\tau$ values) than our construction provided by Theorem~\ref{thm:multi_class_proof}. This is due to a small difference in the exponent: we have $\min_{i \in [N]}\theta_{i} = \Omega(3^{-2^N N\tau})$ in~\cite{aggarwal2021icml} (see Appendix~\ref{app:experiments}), but $\Omega(3^{-2^{2N}N\tau})$ when using Theorem~\ref{thm:multi_class_proof} with $K=2$ (as mentioned above).
% On the other hand our construction is very general and extends to multiclass cross-entropy loss and beyond, which the construction in~\cite{aggarwal2021icml} does not handle.  

Figures~\ref{fig:singlequery}(b)-(c) show the number of datapoints on which Algorithm~\LabelInf achieves at least 50\% accuracy for cross-entropy and softmax cross-entropy loss. We notice this number is smaller for softmax cross-entropy as compared to regular cross-entropy (see Figure~\ref{fig:singlequery}(a)), which is also not surprising. Through a similar argument as that above for the number of bits required for cross-entropy loss, one can show that computing the softmax cross-entropy loss will require an additional $\Omega(NK + \ln(N\tau))$ bits (see the discussion in Appendix~\ref{app:experiments} for details). This additional requirement further constraints the number of labels that can be recovered with softmax cross-entropy loss.



% Finally, the longest computation time for a single label inference across all the experiments with $N=10$ is below 10 milliseconds. 
% In summary, our empirical results attest that these attacks can be performed effectively on real datasets, and also highlight some technical nuances when running label inference on machines with finite floating-point precision. 


% At $N=10$, $K=2$, and $\tau=0.0001$, this implies $\phi > 1000$. However, this upper bound is not tight, as we see in Figure \ref{fig:singlequery}(a) -- our 64-bit machine can perform perfect label inference on the Titanic dataset at noise 0.0001 for length 10. 

% We also ran a baseline label inference experiments on the Titanic dataset for cross-entropy, where the calibrated prediction vector $\theta$ from step 1 in Algorithm~\LabelInf is replaced by a uniformly random vector. We repeat the experiment 1,000 times and the maximum vector length at which 100\% accuracy is achieved is 3 and 1 at noise magnitude 0.0001 and 0.01, which are smaller than 10 and 8 by Algorithm~\LabelInf. When the noise magnitude increases to 0.1 and 1, the randomly generated vector cannot correctly infer label vector even at length 1 with 100\% accuracy.
% \abhi{Moving this closer to Algorithm~\LabelInf in the paper.}


 
 


 



%The median loss in the experiments is about 2.4 for cross-entropy (log-loss), 0.6 for sigmoid cross-entropy loss, and 1.12 for softmax cross-entropy loss. The longest run time for a single label inference across all the experiments based on Algorithm~\LabelInf in this section is below 10 milliseconds.
%\shiva{we need also results in all the plots for the unnoised case, maybe by setting $\tau$ to be extremely small}
 
%The fraction of correctly inferred labelings with respect to the length of the private vector is computed by running the label inference algorithm on 1000 labelings of each specific length randomly sampled from the corresponding dataset. 
 
%\shiva{This needs more discussion. Why is there a drop? Why does  Corollary~\ref{cor:APAFPA} not apply?}
 
%\shiva{can we show $9$ is almost close to what we expect based on the values? Remember the question in the ICML reviews which asked for something like this?}
%\shiva{Comparison to ICML does not show good results for us? We need to revisit this one?}





%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.26]{accuracy.png}
%    \caption{Results on  label inference using Algorithm~\LabelInf on the three real datasets: Titanic, Iris, and Satellite. The first row shows the performance of the label inference from log-loss. The second row shows the performance from sigmoid cross-entropy loss. The third row shows the performance from softmax cross-entropy loss. }
%    \label{accuracy}
%\end{figure}


%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.2]{binary_vs_icml.png}
%    \caption{Results comparing binary log-loss label inference using Algorithm~\LabelInf versus Algorithm 2 in ICML paper on the Titanic dataset. }
%    \label{binary_vs_icml}
%\end{figure}

%
%%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.2]{accuracy_multiquery.png}
%    \caption{Results on the multi-query label inference using Algorithm %\textsc{LabelInf} in shards from log-loss on the three real datasets: Titanic, Iris, and Satellite. }
%    \label{accuracy_multiquery}
%\end{figure}

==> neurips2021/linearly_separable_analysis.tex <==
The analysis for cross-entropy loss and its extensions above can be generalized to determine $\tau$-codomain separability for a broad class of loss functions, defined as follows. Let $g:[0,1] \to \mathbb{R}$ be some deterministic function. We say that a binary loss function $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ is linearly-decomposable in $\{0,1\}$ using $g$ if it can be expressed in the following form:
\begin{align}
\label{eq:linear_separable}
f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i \in [N]:\sigma_i=1} g(\theta_i) + \sum_{i \in [N]:\sigma_i=0} g(1-\theta_i)}.    
\end{align}
Our ideas from the previous section can be used to establish the following separability result for linearly-decomposable loss functions, hence, enabling the use Algorithm~\LabelInf for $\tau$-robust label inference in these cases. Missing details are presented in Appendix~\ref{app:bregman}.
\begin{theorem}
\label{thm:linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Then, for any $\tau > 0$, the function $f$ is $2\tau$-codomain separable if there exists $\theta \in (0,1)^N$ so that $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$.
\end{theorem}

\noindent\textbf{Some Examples of Linearly-Decomposable Loss Functions.} Observe that the KL-divergence loss (which reduces to binary cross-entropy loss) is of this form, using $g(\theta_i) = -\ln \theta_i$ (see~\eqref{eq:KL}, Appendix~\ref{app:bregman}). Some other
common examples of linearly-decomposable losses include the (i) Itakura-Saito divergence loss, which can be expressed using $g(\theta_i) = 1/\theta_i + \ln \theta_i - 2$ (see~\eqref{eq:IS}, Appendix~\ref{app:bregman}); (ii) squared Euclidean loss, which can be expressed using $g(\theta_i) = (1-\theta_i)^2$, (see~\eqref{eq:sqEuc}, Appendix~\ref{app:bregman}); and, (iii) norm-like divergence loss, which can be expressed using $g(\theta_i) = 1 + (\alpha-1)\theta_i^\alpha - \alpha \theta_i^{\alpha-1} + (\alpha-1)(1-\theta_i)^\alpha$ for some $\alpha \ge 2$ (see~\eqref{eq:norm}, Appendix~\ref{app:bregman}).

\textbf{Connections to Bregman Divergence.} The loss functions mentioned in (i)-(iii) above are some popular instances of the general class of
Bregman divergence-based loss functions.
% \!\footnote{The  function $g$ is related but not the function associated with the defn.\ of the corresponding divergence.} 
Unlike the distance metrics for probability distributions, Bregman divergence~\citep{bregman1967relaxation} does not require its inputs to be necessarily distributions. Thus, to use these divergences as loss functions, one can directly compare the outputs of the ML model with the point distribution from the ground truth labels~\citep{liu2016clustering}. We defer the details on our general result for $\tau$-codomain separability on Bregman divergence, including that for the Mahalanobis divergence loss (which is not linearly-decomposable) to Appendix~\ref{app:breg_general}.

\textbf{Applying Theorem~\ref{thm:linear_separable}.} Observe that Theorem~\ref{thm:linear_separable} immediately allows constructing a vector that will make a given linearly-decomposable function $f$ admit $\tau$-codomain separability for a given $\tau > 0$: (1) Compute $x^*(y)$ as the solution to $g(x)-g(1-x) = y$; (2) If $x^*(y)$ exists, then set $\theta_i = x^*(2^iN\tau)$ for all $i \in [N]$. This vector $\theta$ can now be used for $\tau$-robust label inference from $f$ using Algorithm~\LabelInf. However, such a $\theta$ might not exist for all loss functions, e.g., it does not exist for squared Euclidean and norm-like divergence losses, and we will deal those loss functions later. It does exist though for the Itakura-Saito divergence loss (defined in~\eqref{eq:IS}, Appendix~\ref{app:bregman}).
% mentioned earlier can satisfy the required condition in Theorem~\ref{thm:linear_separable} on $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$.
\begin{corollary} \label{cor:IS}
The Itakura-Saito divergence loss is $2\tau$-codomain separable with $\theta_i = (1+3^{2^{i}N\tau})^{-1}$.
\end{corollary}


% For the Norm-like divergence loss, observe that $f(\sigma,\theta) < \alpha$ for all $\sigma,\theta$. Hence, this loss is not $\tau$-codomain separable for any $\tau \geq \alpha/(2N)$. Even when $\tau < \alpha/(2N)$, notice that for $\theta_i \in (0,1)$, we can write $g(\theta_i) - g(1-\theta_i) =  \alpha\paran{(1-\theta_i)^{\alpha-1} - \theta_i^{\alpha-1}} < \alpha$. Since $\alpha$ is a constant, there does not exist any $\theta_i$ for which $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$.

\noindent\textbf{Multi-Query Polynomial Time Attacks.} 
The linear-decomposability of $f$ allows for an efficient multi-query label inference algorithm for $f$. In particular, we could have a trade-off between the ability to perform  multiple queries with faster computation times for solving the optimization problem solved in Step 3 of Algorithm~\LabelInf. 
% As noted in Section~\ref{sec:prelim}, whereas the optimization problem in Algorithm~\LabelInf can be naively solved using an exponential search over $\sigma$. 
To see this, observe that setting $\theta_i = 1/2$ gives $g(\theta_i) - g(1-\theta_i) = 0$. Thus, if we want to infer the first $M < N$ labels in a single query, we can set $\theta = [\theta_1,\dots,\theta_M,1/2,\dots,1/2]$ to obtain: 
% so that the following holds:
% \begin{align*}
%     f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i\leq M: \sigma(i)=1} (g(\theta_i)-g(1-\theta_i)) + \sum_{i=1}^M g(1-\theta_i) + \frac{(N-M)g(1/2)}{M}}.
% \end{align*}
% From this, we immediately obtain that:
\begin{align*}
    \Lambda_\theta(f) &= \frac{1}{N} \min_{\sigma_1,\sigma_2 \in \{0,1\}^N} \abs{\sum_{i\leq M:\sigma_1(i)=1}\paran{g(\theta_i)-g(1-\theta_i)} - \sum_{j\leq M:\sigma_2(j)=1}\paran{g(\theta_j)-g(1-\theta_j)}}.
\end{align*}
Similar to Theorem~\ref{thm:linear_separable}, choosing $\theta_i$ that ensures $g(\theta_i)-g(1-\theta_i) > 2^iN\tau$ will ensure $\Lambda_\theta(f) > 2\tau$. Moreover, using this $\theta$ will ensure that if $f(\sigma_1,\theta) = f(\sigma_2,\theta)$, then $\sigma_1[:M] = \sigma_2[:M]$ must hold.  Note that after recovering the first $M$ labels, we can recover the next $M$ labels using $\theta = [1/2,\dots,1/2,\theta_{M+1},\dots,\theta_{2M},1/2,\dots,1/2]$, and so on. The result below immediately follows.

% \input{neurips2021/single_query_plot}

\begin{theorem}
\label{thm:multi_query_general} 
Let $g:[0,1] \to \mathbb{R}$ be some finite deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Then, for any $\tau > 0$ and integer $M \geq 1$, a sufficient condition for $f$ to admit $\tau$-robust label inference with $\lceil N/M \rceil$ queries is for the inequality $g(x) - g(1-x) > 2^iN\tau$ to have a solution for all $i \in [N]$.
% there exist $x_1,\dots,x_M \in (0,1)$ such that $g(x_i) - g(1-x_i) > 2^iN\tau$ for all $i \in [M]$.
\end{theorem}
Observe that an $\lceil N/M \rceil$-query algorithm for robust label inference will require $O(N2^M/M)$ local computations by the adversary (using Algorithm~\LabelInf in each query). Thus, while the single query case ($M = N$) required $O(2^N)$ computations, any multi-query algorithm using $M=O(\log N)$ requires only $O(\text{poly}(N))$ local computations, which allow a polynomial-time robust label inference. 

\noindent\textbf{Linearly-Decomposable Functions Not Covered by Theorem~\ref{thm:linear_separable}.} We now deal with linearly-decomposable functions for whom there exists no $\theta$ that could satisfy the condition required in Theorem~\ref{thm:linear_separable} (examples include, squared Euclidean and norm-like divergence loss). Here, we establish the weaker \zero-codomain separability, which as discussed earlier suffices for label inference in the unnoised case. 

% \noindent\textbf{A Note on the \zero-Codomain Separability of Linearly-Decomposable Functions.} Observe that in Theorem~\ref{thm:linear_separable}, the condition on the function $g$ has a linear dependence on $\tau$, which will not suffice for label inference in the un-noised setting (where $\tau=0$). We state the result for this special case in the Theorem below\footnote{Note that while it is true that any vector with respect to which a function is $\tau$-codomain separable (for $\tau>0$) also allows \zero-codomain separability, we mention Theorem~\ref{thm:zero_codomain_linear_separable} to cover cases where $\tau$-codomain separability is hard to demonstrate (see the discussion about Norm-Like loss following the statemnt of Theorem~\ref{thm:zero_codomain_linear_separable}).} and show how it can be used to achieve \zero-codomain separability for the Square-Euclidean loss and the Norm-Like loss. 

\begin{theorem}
\label{thm:zero_codomain_linear_separable}
Let $g:[0,1] \to \mathbb{R}$ be some deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Let $\theta \in (0,1)^N$ be some vector and $S_\theta = \{g(\theta_i) - g(1-\theta_i)\}_{i=1}^N$. Then, the function $f$ is \zero-codomain separable with respect to $\theta$ if $\mu(S_\theta)>0$, i.e., all subset sums in the set $S_\theta$ are distinct.
\end{theorem}
\begin{corollary} \label{cor:eucl}
The squared Euclidean loss  is  \zero-codomain separable using $\theta_i = (1/2)\paran{1-\ln(p_i)/N}$, where $p_i$ is the $i$th prime number for $i \in [N]$. The norm-like divergence loss for $\alpha \geq 2$ is \zero-codomain separable using $\theta$ that satisfies $(1-\theta_i)^{\alpha-1}-\theta_i^{\alpha-1} = (\ln p_i)/(N\alpha)$.
\end{corollary}
Finally, the idea behind the multi-query attack mentioned in Theorem~\ref{thm:multi_query_general} also extends to loss functions covered by Theorem~\ref{thm:zero_codomain_linear_separable}, thus, providing a multi-query polynomial time inference here too. 

% \section{$\tau$-Robust Label Inference from Bregman Divergence-based Binary Losses}
% \label{sec:bregman}
% We now discuss label inference from another important class of distance metrics used across ML applications, known as the class of Bregman divergences~\citep{bregman1967relaxation}. Given a continuously differentiable strictly convex function $F:\mathcal{S} \to \mathbb{R}$ over some closed convex set $\mathcal{S} \subseteq \mathbb{R}^d$, the Bregman divergence $D_F: \mathcal{S} \times \mathcal{S} \to \mathbb{R}$ associated with $F$ is defined as $D_F(\mathbf{p},\mathbf{q}) = F(\mathbf{p})-F(\mathbf{q})-\langle \nabla F(\mathbf{q}), \mathbf{p}-\mathbf{q} \rangle$. Missing details from this section are collected in Appendix~\ref{app:bregman}.

% % Some examples of Bregman divergence are the squared Euclidean distance $D_F(x,y) = \|x-y\|_2$, generated by the convex function $F(x) = \|x\|^2$; the squared Mahalanobis distance $D_F(x,y) = \frac{1}{2}(x-y)^\top Q(x-y)$, generated by $F(x) = \frac{1}{2}x^\top Qx$ for some positive semi-definite matrix $Q$; and, the generalized Kullback-Leibler divergence $D_F(p,q) = \sum_i p(i) \log \frac{p(i)}{q(i)} - \sum_i p(i) + \sum_i q(i)$, generated by $F(x) = -\sum_i p(i)\log p(i)$. 

% Note that unlike the distance metrics for probability distributions, Bregman divergence does not require its inputs to be necessarily distributions. Thus, to use these divergences as loss functions, one can directly compare the outputs of the ML model with the point distribution from the ground truth labels~\citep{liu2016clustering}. We will focus on the binary case for our discussion in this section and assume that the domain of $F$ is the closed convex set $[0,1]^N$, the $N$-dimensional hypercube. 
% % The multiclass setting will immediately follow by modeling the $K$-ary classifier as an ensemble of $K$ one-vs-all binary classifiers using standard techniques. \shiva{I do not follow, why does the same not hold for log-loss then?}

% For starters, a common Bregman divergence loss on $N$ datapoints defined using (generalized) Kullback-Leibler (KL) divergence  $\text{KL}([x_1,x_2]) = \sum_{j=1}^2 (x_j \log x_j)$, in the binary
% %classification 
% setting~\citep{liu2016clustering}, 
% $$\frac{1}{N}\sum_{i=1}^N  D_{\text{KL}}([\sigma_i,1-\sigma_i],[\theta_i,1-\theta_i]) = \frac{-1}{N}  \sum_{i=1}^N \sigma_i \log \theta_i + (1-\sigma_i) \log(1-\theta_i),$$
% % \shiva{we have $\ln 0$? as $\sigma_i$ could be $0$? Should we say $0 \ln 0 = 0$?}
% is exactly the cross-entropy loss\footnote{Here, we adopt the notion that $0\ln 0=0$, so that KL divergence is well-defined.} and is therefore covered by results in Section~\ref{sec:logloss}. Similar to the general construction of robust label inference for linearly-decomposable functions in Section~\ref{sec:linearly_separable}, we now demonstrate $\tau$-robust label inference for a special class of Bregman divergences: the ones associated with functions $F$ that are additive on the elements of its input vector.
% \begin{theorem}
% \label{thm:bregman_general} Let $F:(0,1)^2 \to \mathbb{R}$ be a strictly convex function that can be written in the form $F(\mathbf{v}) = \sum_{i=1}^2 h(v_i)$ for some differentiable function $h:(0,1) \to \mathbb{R}$. Let $D_F$ denote the Bregman divergence associated with $F$, and $f_F:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be the corresponding loss function, defined as $f_F(\sigma,\theta) = (1/N)\sum_{i=1}^N D_F([1-\sigma_i,\sigma_i],[1-\theta_i,\theta_i])$. Then, for $\tau > 0$, the function $f_F$ is $2\tau$-codomain separable if there exists $\theta \in (0,1)^N$ that satisfies  $h'(\theta_i) + h'(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$, where $h'(x) = dh/dx$.
% \end{theorem}

% \shiva{This discussion is not clear? Do we have any loss where the above theorem works?}
% Some common examples of Bregman divergence that are additive, include the KL-divergence and the Ikatara-Saito divergence, that recall are also linearly decomposable (from Theorem~\ref{thm:linear_separable}). Thus, any vector constructed from either Theorems~\ref{thm:linear_separable} or~\ref{thm:bregman_general} will allow $\tau$-robust label inference for these corresponding losses. 

% However, not all Bregman divergences are additive. A popular example of a Bregman divergence that is not additive is the Mahalanobis divergence, the loss corresponding to which is defined as follows:
% $$\textsc{MHLoss}(\sigma, \theta) = \frac{1}{N}\sum_{i=1}^N ([\sigma_i,1-\sigma_i] - [\theta_i,1-\theta_i])^\top A ([\sigma_i,1-\sigma_i] - [\theta_i,1-\theta_i]) \mbox{ where} A \in \mathbb{R}^{2 \times 2}.$$
% We discuss $\tau$-robust label inference for the Mahalanobis loss function in the theorem below.
% \begin{theorem}
% \label{thm:mahalanobis}
% Let $A = \bigl[\begin{smallmatrix}
% a&b\\ c&d
% \end{smallmatrix}\bigr] \in \mathbb{R}^{2 \times 2}$ be a matrix with $(a+d)>(b+c)$. Denote $\alpha = a+d-(b+c)$ and let $\tau \in [0,\alpha/N)$. Then, for any $\tau > 0$, the Mahalanobis loss (defined above) 
% % defined by $$\textsc{MHLoss}(\sigma, \theta) = \frac{1}{N} \sum_{i=1}^N ([\sigma_i,1-\sigma_i] - [\theta_i,1-\theta_i])^\top A ([\sigma_i,1-\sigma_i] - [\theta_i,1-\theta_i]),$$ 
% is $\tau$-codomain separable using any $\theta \in (0,1)^N$ with $\|\theta\|_\infty < (1/2)\paran{1 - N\tau/\alpha}$.
% \end{theorem}

==> neurips2021/log_loss_analysis.tex <==
We start with establishing $\tau$-codomain separability for multiclass cross-entropy loss and its variants, for any $\tau > 0$. This implies that for these loss functions, Algorithm~\LabelInf succeeds in recovering all the labels when the loss scores are noised by less than $\tau$ in magnitude. We explain our main results at a high level and defer all missing details from this section to Appendix~\ref{app:logloss}. 
% This extends the results in~\citep{aggarwal2021icml}, where $\tau$-robust label inference in the binary case ($K=2$) was discussed. 
% Missing details from this section are collected in Appendix~\ref{app:logloss}.
% it is possible to design a prediction vector such that the multiclass cross-entropy loss scores differ by more than $2\tau$ on any two distinct labelings. Therefore, one could Algorithm~\LabelInf to perform 
% We begin by explaining the intuition behind our construction and then provide a formal proof of correctness. We also discuss how to generalize this approach to commonly used variants of the cross-entropy loss. We will end this section with a discussion around the computational hardness of label reconstruction for such losses, and show that this problem is in EXPTIME.

\noindent\textbf{Multiclass Cross-Entropy Loss.} We first recall the definition of multiclass cross-entropy (extending Definition~\ref{eq:log_loss_defn}). 
We assume $K \geq 2$ classes, and let $N$ and $\ZZZ_{K}$ denote the number of datapoints and the set of label classes, respectively. The $K$-ary cross-entropy loss on $\theta$ with respect to a labeling $\sigma \in \ZZZ_{K}^N$ is denoted by $\Klogloss\paran{\sigma, \theta}$ and defined as follows:
	\begin{align}
	\label{eq:multi_class_log_loss}
		\Klogloss\paran{\sigma, \theta} := \frac{-1}{N}\sum_{i=1}^N \sum_{k=0}^{K-1} \ \Big([\sigma_i = k] \cdot \ln \theta_{i,k} \Big),
	\end{align}
 where $[\sigma_i = k] = 1$ if $\sigma_i = k$ and $0$, otherwise.
Here, $\theta \in \Theta = [0,1]^{N \times K}$ is a matrix of prediction probabilities, where the $i$th row is the vector of prediction probabilities $\theta_{i,0},\dots,\theta_{i,K-1}$ (with $\sum_{k \in \ZZZ_K} \theta_{i,k} = 1$) for the $i$th datapoint on classes $0,\dots,K-1$ respectively. 

With this definition, we can now describe our construction of a matrix $\theta \in [0,1]^{N \times K}$ that makes $\Klogloss$ function $2\tau $-codomain separable for any $\tau >0$ (i.e., $\Lambda_{\theta}(\Klogloss) \geq 2 \tau $). At a high level, we obtain the required codomain separability for $\Klogloss$ by designing the entries in the matrix $\theta$ in such a way that the expression inside the logarithm in~\eqref{eq:multi_class_log_loss} reduces to a distinct integer in some set. This calibration allows us to control the minimum difference in the output of the cross-entropy loss on different labelings, which we can scale to the desired amount ($\geq 2\tau$) easily. The following theorem summarizes our construction.  
% (see the Appendix for a detailed proof). 
\begin{theorem}\label{thm:multi_class_proof}
Let $\tau > 0$. Define matrices $\vartheta, \theta \in \mathbb{R}^{N \times K}$ such that $\vartheta_{n,k} = 3^{\paran{2^{(n-1)K+k}N\tau}}$ and $\theta_{n,k} = \vartheta_{n,k} / \sum_{k=1}^K \vartheta_{n,k}$. Then, it holds that $\Klogloss$ is $2 \tau $-codomain separable using $\theta$.
\end{theorem}
% \abhi{$\phi = O\paran{2^{NK}N\tau}$.
% N = 5, K = 2, tau = 0.01 => phi = 51.2}

The following corollary follows by combining the above result with Theorem~\ref{thm:inf}. 
\begin{corollary}
Using $\theta$ from Theorem~\ref{thm:multi_class_proof}, Algorithm~\LabelInf performs $\tau$-robust label inference from the K-ary cross-entropy loss ($\Klogloss$).
\end{corollary}
Note that Theorem~\ref{thm:multi_class_proof} only holds for the error $\tau >0$. However, as mentioned in Remark~\ref{rem:first}, in the unnoised case it suffices to instantiate Theorem~\ref{thm:multi_class_proof} with an arbitrarily small positive value of $\tau$. 
We bring to the reader's attention the doubly-exponential nature of the entries used to construct the prediction vector in Theorem~\ref{thm:multi_class_proof}. This blowup is unfortunately unavoidable for constructing $\tau$-codomain separability, even for the binary case, as shown in \citep[Theorem~7]{aggarwal2021icml}.
% Clearly, this will limit the practicality of the attack on real datasets (see our experiments in Section~\ref{sec:experiments}) due to limited floating-point precision. 
% A natural question to ask if there is a way to avoid such large entries when constructing a matrix $\theta$ for $2\tau$-separability of $\logloss$. This question was answered in the negative for the binary case in~\citep{aggarwal2021icml}, where it was shown that for any vector $v \in \mathbb{Q}^N$, if the binary log-loss admits $2\tau$-separability using $v \mapsto \frac{v}{1+v}$ (element-wise), then $\|v\|_\infty = \Omega(e^{2^N N\tau})$ must hold. By an easy extension to the multiclass case, this lower bound also holds for our use case and establishes the optimality of our construction in Theorem~\ref{thm:multi_class_proof}.

\noindent\textbf{Extensions of Cross-Entropy Loss.} Often in practice, when using the cross-entropy loss to assess the performance of ML models (like CNNs), it is common to apply an activation function (such as softmax or sigmoid) before the cross-entropy loss calculation. 
% The former compresses arbitrary reals into the range $(0,1)$, while the latter can convert any sequence of real outputs into a probability distribution.
% The outputs from the model do not necessarily represent probability distributions. In such cases, transformations are applied to these outputs before they can be fed into the cross-entropy loss computation. 
For example, a common idea in multiclass classification is to apply the softmax function (to convert any sequence of real outputs into a probability distribution),
% $\textsc{Softmax}:\mathbb{R}^K \to [0,1]^K$, that modifies any vector $\mathbf{v} = (v_1,\dots,v_K) \in \mathbb{R}^K$ using the transformation $v_i \mapsto \exp(v_i)/\sum_{j=1}^K \exp(v_j)$. 
% This leads to the softmax cross-entropy loss, $\textsc{Softmax-K-LLoss}:\ZZZ_K^N \times \mathbb{R}^{N \times K} \to \mathbb{R}$, 
defined as follows for $\sigma \in \ZZZ_K^N$, $\theta \in [0,1]^{N \times K}$:
\begin{align*}
 \frac{-1}{N}\sum_{i=1}^N \sum_{k=0}^{K-1} \ \Big([\sigma_i = k] \cdot \ln \textsc{softmax}(\theta_{i,k}) \Big), \mbox{ where } 
 \textsc{softmax}(\theta_{i,k}) = \exp(\theta_{i,k})/\sum_{j=1}^K \exp(\theta_{i,j}).
\end{align*}
We explain how to extend Theorem~\ref{thm:multi_class_proof} to obtain separability in this setting. Our idea is the following: (1) Let $\theta \in [0,1]^{N \times K}$ be the matrix from Theorem~\ref{thm:multi_class_proof}. Recall that by definition, $\theta$ is such that for each $i \in [N]$, the vector $\theta_i \in [0,1]^K$ is a probability distribution; (2) For each $i \in [N]$, solve the following (fully specified) system of equations for $\theta'_{i,k}$'s: for all $k \in \ZZZ_K , i \in [N]$: $\exp\paran{\theta'_{i,k}}/\sum_{j=1}^K \exp\paran{\theta'_{i,j}} = \theta_{i,k}$.
% \begin{align}
% \exp\paran{\theta'_{i,k}}/\sum_{j=1}^K \exp\paran{\theta'_{i,j}} = \theta_{i,k}.    
% \end{align}
This is a system of linear equations in the variables $\exp\paran{\theta'_{i,j}}$, for each $i \in [N]$, hence, can be solved in polynomial time using standard techniques. Once $\theta'$ is obtained, since $\textsc{softmax}(\theta'_{i,k}) = \theta_{i,k}$, from Theorem~\ref{thm:multi_class_proof}, we get that softmax cross-entropy loss is $2\tau $-codomain separable using $\theta'$; Algorithm~\LabelInf can now be used for $\tau$-label inference.

The separability from Theorem~\ref{thm:multi_class_proof} also holds if we apply any bijective activation function before applying the cross-entropy loss. As an example, consider the sigmoid cross-entropy commonly used in the binary classification setting (to compresses arbitrary reals into the range $(0,1)$), defined as follows for $\sigma \in \{0,1\}^N$, $\theta \in (0,1)^N$:
% 	\textsc{Sig-LLoss}\paran{\sigma, \theta} :=
\begin{align}
\label{eq:sigmoid_definition}
	 \frac{-1}{N}\sum_{i=1}^N \ \Big( \sigma_i \ln \paran{\textsc{Sigmoid}(\theta_i)} + (1-\sigma_i)\ln \paran{1-\textsc{Sigmoid}(\theta_i)} \Big),
\end{align}
where $\textsc{Sigmoid}(x) = \paran{1+e^{-x}}^{-1}$ is the sigmoid function. Since $\textsc{Sigmoid}:\mathbb{R} \to (0,1)$ is a bijection (and hence, invertible), given $\textsc{Sigmoid}(x) = y$, we can obtain $x = \ln (y/(1-y))$. Thus, given the matrix $\theta \in [0,1]^{N \times 2}$ from Theorem~\ref{thm:multi_class_proof}, we can construct $\theta' \in (0,1)^{N}$ such that $\theta'_{i} = \ln (\theta_{i,1}/(1-\theta_{i,1}))$ for all $i \in [N]$.
% respect to which   is $\tau$-codomain separable, we can obtain the vector $\theta'$ such that $\theta'_i = \ln (\theta_i/(1-\theta_i))$. 
 Once $\theta'$ is obtained, since $\textsc{Sigmoid}(\theta_{i}) = \theta_{i,1}$ and $1-\textsc{Sigmoid}(\theta_{i}) = \theta_{i,2}$  we get that sigmoid cross-entropy loss is $2\tau $-codomain separable using $\theta'$, and hence Algorithm~\LabelInf can be used for $\tau$-robust label inference.
 

% The bijection will ensure that the sigmoid cross-entropy loss is $\tau$-codomain separable with respect to $\theta'$, and hence, allows robust label inference. More generally, replacing $\textsc{Sig}$ with any injective function will behave similarly.

% Two commonly used examples of these transformations are the sigmoid activation and the Softmax computation. The former compresses arbitrary reals into the range $(0,1)$, while the latter can convert any sequence of real outputs into a probability distribution. We discuss the separability of cross-entropy scores obtained from such use cases and show, through a reduction to the multiclass case above, that robust label inference is possible for any amount of noise, as before.
% We consider extensions of this $\Klogloss$ to 

% \noindent\textbf{Softmax (Categorical) Cross-Entropy Loss.} For multiclass classification problems, often the outputs of the model are real numbers that do not necessarily form a probability distribution. The softmax function, denoted as $\textsc{Softmax}:\mathbb{R}^N \to [0,1]^N$, modifies any vector $\mathbf{v} = (v_1,\dots,v_N) \in \mathbb{R}^N$ using the transformation $v_i \mapsto \exp(v_i)/\sum_{j=1}^N \exp(v_j)$. Formally, $\textsc{SoftmaxLoss}:\{0,1\}^N \times \mathbb{R}^N \to \mathbb{R}$, is defined as:
% \begin{align}
% 	\label{eq:softmax_loss}
% 		\textsc{SoftmaxLoss}(\sigma,\theta) := \logloss\paran{\sigma;\{\textsc{Softmax}(\theta_i)\}_{i=1}^N}.
% \end{align}
% Now, to design a vector $\theta' \in \mathbb{R}^{N \times K}$ with respect to which $\textsc{SoftmaxLoss}(\sigma,\theta)$ is $\tau$-codomain separable (and hence, admits $\tau$-robust label inference by Proposition~\ref{prop:bound_on_tau_for_label_inference}), we provide the following general steps: (1) Let $\theta \in [0,1]^{N \times K}$ be the matrix from Theorem~\ref{thm:multi_class_proof}. Recall that by definition, $\theta$ is such that for each $i \in [N]$, the vector $\theta_i \in [0,1]^K$ is a probability distribution; (2) For each $i \in [N]$, solve the following (fully specified) system of equations: $\forall k \in \ZZZ_K.\ \ \ \frac{\exp\paran{\theta'_{i,k}}}{\sum_{k=1}^K \exp\paran{\theta'_{i,k}}} = \theta_{i,k}$. Note that this is a system of linear equations in the variables $\exp\paran{\theta'_{i,k}}$, which, for each $i \in [N]$, can be solved in polynomial time using standard techniques. Once $\theta'$ is obtained, robust label inference can be done using Algorithm~\LabelInf.



% \noindent\textbf{sigmoid (Cross-Entropy) Loss.} We discuss the binary case to explain the main idea behind our construction for this loss function. For the multiclass case, it is common to use Softmax instead of the sigmoid -- we will discuss the Softmax Loss in the next subsection. The sigmoid loss for the binary case, denoted $\textsc{SigLoss}:\{0,1\}^N \times \mathbb{R}^N \to \mathbb{R}$, is defined as follows:
% \begin{align}
% 	\label{eq:sigmoid_log_loss}
% 		\textsc{SigLoss}\paran{\sigma, \theta} := \frac{-1}{N}\sum_{i=1}^N \ \Big( \sigma_i \ln \paran{\textsc{Sigmoid}(\theta_i)} + (1-\sigma_i)\ln \paran{1-\textsc{Sigmoid}(\theta_i)} \Big),
% \end{align}

% \subsection{Computational Hardness of Robust Label Inference for Cross-Entropy Loss}

% \abhi{Use the lower bound in the ICML paper to argue that RLI is in EXP-TIME.}

% In this section, we prove that Robust-Label Inference for Cross-Entropy Loss is NP-Hard. We show this by reduction from the \textsc{Subset-Sum} problem. Note that it suffices to prove this hardness result for the binary case. This is in contrast to the polynomial time label inference algorithm provided in~\citep{aggarwal2021icml} for the un-noised setting, where the authors used a construction using prime numbers. 

% We begin by reminding the reader of the \textsc{Subset-Sum} problem. In this problem, we are given a set $S$ and a target sum $T$. The task is to output a subset of $S$ such that the sum of the elements in this subset is at most $T$. This problem is well known to be NP-complete. Thus, it suffices to provide a polynomial time reduction from the \textsc{Subset-Sum} problem into Robust Label Inference.

% We first perform some algebraic manipulation on the expression for Robust Label Inference from $\logloss$. For a fixed bound on the noise $\tau$, prediction vector $\theta$ (with respect to which the function $\logloss$ is $2\tau$-codomain separable) and observed loss $\ell$, we know that true labeling $\sigma \in \{0,1\}^N$ satisfies the condition 
% $\abs{\logloss(\sigma, \theta) - \ell} \leq \tau$. Moreover, $\sigma$ is the only labeling that satisfies this condition (from Proposition~\ref{prop:bound_on_tau_for_label_inference}). This inequality can be written as $\ell - \tau \leq \logloss(\sigma, \theta) \leq \tau + \ell$, and on expanding the $\logloss$ term, becomes the following:
% \begin{align*}
%     &\ell - \tau \leq -\frac{1}{N}\sum_{i=1}^N \paran{\sigma_i \ln \theta_i + (1-\sigma_i)\ln (1-\theta_i)} \leq \tau + \ell\\
%     \implies & \ell - \tau \leq \frac{1}{N}\sum_{i=1}^N \ln \parfrac{1}{1-\theta_i} +\frac{1}{N}\sum_{i=1}^N \sigma_i \ln \parfrac{1-\theta_i}{\theta_i} \leq \tau + \ell\\
%     \implies & N(\ell - \tau) - \ln \parfrac{1}{1-\theta_i} \leq \sum_{i=1}^N \sigma_i \ln \parfrac{1-\theta_i}{\theta_i} \leq N(\tau + \ell) - \ln \parfrac{1}{1-\theta_i}.
% \end{align*}
% It suffices to focus only on the inequality on the right above:
% $$\sum_{i=1}^N \sigma_i \ln \parfrac{1-\theta_i}{\theta_i} \leq N(\tau + \ell) - \ln \parfrac{1}{1-\theta_i}.$$
% To reduce the \textsc{Subset-Sum} problem for a given set $S = \{s_1,\dots,s_N\}$ and threshold $T$, we first set $\ln \parfrac{1-\theta_i}{\theta_i} = s_i$ to obtain $\theta_i = 1/(1+\exp(s_i))$. This will make $\sum_{i=1}^N \sigma_i s_i$ equivalent to selecting a subset from $S$, since $\sigma_i \in \{0,1\}^N$. Next, we set $T = N(\tau + \ell) - \ln \parfrac{1}{1-\theta_i}$, to obtain the following:
% $$\tau + \ell = \paran{T - s_i + \ln \paran{1+e^{s_i}}}/N.$$

% \abhi{Complete details here -- be careful about setting tau and ell -- ell must be such that (1) theta gives the required 2 tau separability and (2) ell must not be more than tau far away from the true loss. Mention that an FPTAS can be used for approximation here, but will need to work out the details here.}

==> neurips2021/plots.tex <==
\captionsetup[subfloat]{labelformat=empty}
\begin{figure*}[t]
    \centering
    \vspace{-0.5em}
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/logloss_titanic.png}}
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/logloss_iris.png}} 
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/logloss_satellite.png}} 
    \\[-3ex]
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_titanic.png}}
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_iris.png}} 
    \hspace{0.1em}
    \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_satellite.png}} 
    % \newline
    % \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_titanic.png}}
    % \hspace{-0.1em}
    % \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_iris.png}} 
    % \hspace{-0.1em}
    % \subfloat[]{\includegraphics[width=120pt]{individual_figure/softmax_satellite.png}} 
    \vspace*{-3ex}
    \caption{Label reconstruction accuracy with multi-query label inference attack by performing Algorithm~\LabelInf on $M$ datapoints at a time using a total of $\lceil N/M \rceil$ queries. Here, $N$ is the total number of rows in the corresponding dataset (2201 for Titanic, 150 for Iris, and 6430 for Satellite).}
    \label{fig:multiquery}
    \vspace{2ex}
\end{figure*}

==> neurips2021/short_paper_discussion.tex <==
Informally, a loss function $(\sigma,\theta)\mapsto \mathbb{R}$ takes as input a labeling $\sigma \in \{0,1\}^N$ and a prediction vector $\theta \in [0,1]^N$ to produce a loss score in $\mathbb{R}$. For some $\tau > 0$, we call this function $\tau$-codomain separable if there exists some vector $\theta$ such that the output of the loss function (keeping $\theta$ fixed) on any two labelings differs by at least $\tau$. Thus, when $\theta$ is known, the one-one correspondence between the function's output and the labelings can be exploited for label inference (for example, through an exhaustive enumeration as in Algorithm~\LabelInf, Appendix~\ref{sec:prelim}) to exactly recover all the labels from just observing the output, which we refer to as \emph{robust label inference} (see Definition~\ref{def:robust_label_inference} in Appendix~\ref{sec:prelim}). A necessary and sufficient condition for inferring all ground truth labels from a loss function, noised upto $\tau$, is for this function to admit $2\tau$ codomain separability (see Proposition~\ref{prop:bound_on_tau_for_label_inference}).  
% (see Section~\ref{sec:linearly_separable}).

We say that a binary loss function $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ is linearly-decomposable in $\{0,1\}^N$ using some function $g:(0,1) \to \mathbb{R}$ if it can be expressed in the following form:
\begin{align}
f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i \in [N]:\sigma_i=1} g(\theta_i) + \sum_{i \in [N]:\sigma_i=0} g(1-\theta_i)}.    
\end{align}
Observe that the KL-divergence loss (which reduces to binary cross-entropy loss) is of this form, using $g(\theta_i) = -\ln \theta_i$ (see~\eqref{eq:KL}, Appendix~\ref{app:bregman}). Some other
common examples of linearly-decomposable losses include the (i) Itakura-Saito divergence loss, which can be expressed using $g(\theta_i) = 1/\theta_i + \ln \theta_i - 2$ (see~\eqref{eq:IS}, Appendix~\ref{app:bregman}); (ii) squared Euclidean loss, which can be expressed using $g(\theta_i) = (1-\theta_i)^2$, (see~\eqref{eq:sqEuc}, Appendix~\ref{app:bregman}); and, (iii) norm-like divergence loss, which can be expressed using $g(\theta_i) = 1 + (\alpha-1)\theta_i^\alpha - \alpha \theta_i^{\alpha-1} + (\alpha-1)(1-\theta_i)^\alpha$ for some $\alpha \ge 2$ (see~\eqref{eq:norm}, Appendix~\ref{app:bregman}).

Our main result for linearly decomposable loss functions is that for any deterministic function $g:[0,1] \to \mathbb{R}$ and any bound $\tau > 0$ on the noise, the function $f$ is $2\tau$-codomain separable if there exists $\theta \in (0,1)^N$ so that $g(\theta_i) - g(1-\theta_i) > 2^{i}N\tau$ for all $i \in [N]$ (see Theorem~\ref{thm:linear_separable}). Constructing such a vector $\theta$ can be done as follows: (1) Compute $x^*(y)$ as the solution to $g(x)-g(1-x) = y$; (2) If $x^*(y)$ exists, then set $\theta_i = x^*(2^iN\tau)$ for all $i \in [N]$. This vector $\theta$ can now be used for $\tau$-robust label inference from $f$ using Algorithm~\LabelInf (see detailed examples in Appendix~\ref{app:linearly_separable}). 
% However, such a $\theta$ might not exist for all loss functions, e.g., it does not exist for squared Euclidean and norm-like divergence losses, and we will deal those loss functions later. It does exist though for the Itakura-Saito divergence loss (defined in~\eqref{eq:IS}, Appendix~\ref{app:bregman}) -- we show that this loss is $2\tau$-codomain separable with $\theta_i = (1+3^{2^{i}N\tau})^{-1}$ (see Corollary~\ref{cor:IS}).
% mentioned earlier can satisfy the required condition in Theorem~\ref{thm:linear_separable} on $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$.
% \begin{corollary} \label{cor:IS}
% The Itakura-Saito divergence loss is $2\tau$-codomain separable with $\theta_i = (1+3^{2^{i}N\tau})^{-1}$.
% \end{corollary}


% For the Norm-like divergence loss, observe that $f(\sigma,\theta) < \alpha$ for all $\sigma,\theta$. Hence, this loss is not $\tau$-codomain separable for any $\tau \geq \alpha/(2N)$. Even when $\tau < \alpha/(2N)$, notice that for $\theta_i \in (0,1)$, we can write $g(\theta_i) - g(1-\theta_i) =  \alpha\paran{(1-\theta_i)^{\alpha-1} - \theta_i^{\alpha-1}} < \alpha$. Since $\alpha$ is a constant, there does not exist any $\theta_i$ for which $g(\theta_i) - g(1-\theta_i) > 2^iN\tau$ for all $i \in [N]$.

\noindent\textbf{Multi-Query Polynomial Time Attacks.} 
The linear-decomposability of $f$ allows for an efficient multi-query label inference algorithm for $f$. In particular, we could have a trade-off between the ability to perform  multiple queries with faster computation times to avoid an exhaustive search in the space of all labelings. 
% As noted in Section~\ref{sec:prelim}, whereas the optimization problem in Algorithm~\LabelInf can be naively solved using an exponential search over $\sigma$. 
To see this, observe that setting $\theta_i = 1/2$ gives $g(\theta_i) - g(1-\theta_i) = 0$. Thus, if we want to infer the first $M < N$ labels in a single query, we can set $\theta = [\theta_1,\dots,\theta_M,1/2,\dots,1/2]$ to obtain the following (with $\Lambda_\theta(f) := \min_{\sigma_1,\sigma_2} \abs{f(\sigma_1,\theta) - f(\sigma_2,\theta)}$ for brevity): 
% so that the following holds:
% \begin{align*}
%     f(\sigma,\theta) &= \frac{1}{N}\paran{\sum_{i\leq M: \sigma(i)=1} (g(\theta_i)-g(1-\theta_i)) + \sum_{i=1}^M g(1-\theta_i) + \frac{(N-M)g(1/2)}{M}}.
% \end{align*}
% From this, we immediately obtain that:
\begin{align*}
    \Lambda_\theta(f) &= \frac{1}{N} \min_{\sigma_1,\sigma_2 \in \{0,1\}^N} \abs{\sum_{i\leq M:\sigma_1(i)=1}\paran{g(\theta_i)-g(1-\theta_i)} - \sum_{j\leq M:\sigma_2(j)=1}\paran{g(\theta_j)-g(1-\theta_j)}}.
\end{align*}
Similar to the discussion above, choosing $\theta_i$ that ensures $g(\theta_i)-g(1-\theta_i) > 2^iN\tau$ will ensure $\Lambda_\theta(f) > 2\tau$. Moreover, using this $\theta$ will ensure that if $f(\sigma_1,\theta) = f(\sigma_2,\theta)$, then $\sigma_1[:M] = \sigma_2[:M]$ must hold, so that after recovering the first $M$ labels, we can recover the next $M$ labels using $\theta = [1/2,\dots,1/2,\theta_{M+1},\dots,\theta_{2M},1/2,\dots,1/2]$, and so on. It immediately follows that a sufficient condition for $f$ to admit $\tau$-robust label inference with $\lceil N/M \rceil$ queries is for the inequality $g(x) - g(1-x) > 2^iN\tau$ to have a solution for all $i \in [N]$ (see Theorem~\ref{thm:multi_query_general}).
% % \input{neurips2021/single_query_plot}
% \begin{theorem}
% \label{thm:multi_query_general} 
% Let $g:[0,1] \to \mathbb{R}$ be some finite deterministic function and $f:\{0,1\}^N \times (0,1)^N \to \mathbb{R}$ be a loss function that is linearly-decomposable in $\{0,1\}$ using $g$. Then, for any $\tau > 0$ and integer $M \geq 1$, a sufficient condition for $f$ to admit $\tau$-robust label inference with $\lceil N/M \rceil$ queries is for the inequality $g(x) - g(1-x) > 2^iN\tau$ to have a solution for all $i \in [N]$.
% % there exist $x_1,\dots,x_M \in (0,1)$ such that $g(x_i) - g(1-x_i) > 2^iN\tau$ for all $i \in [M]$.
% \end{theorem}
More importantly, observe that an $\lceil N/M \rceil$-query algorithm for robust label inference will require $O(N2^M/M)$ local computations by the adversary (using Algorithm~\LabelInf in each query). Thus, while the single query case ($M = N$) required $O(2^N)$ computations, any multi-query algorithm using $M=O(\log N)$ requires only $O(\text{poly}(N))$ local computations, which allow a polynomial-time robust label inference. 

==> neurips2021/short_paper_experiments.tex <==
%\begin{table}[h]
%\begin{tabular}{lllp{3.5cm}p{2.6cm}} 
%\hline
% Loss & Data & Noise & Max. vector length for perfect label inference & Mean run time per inference (ms) \\ \hline
% Cross-entropy & Titanic & 0.0001 & 10 (15 by ICML) & 1.71 \\
% Cross-entropy &Titanic & 0.01 & 7 (9 by ICML)  & 0.20 \\
% Cross-entropy &Titanic & 0.1 & 5 (6 by ICML)  & 0.07 \\
% Cross-entropy & Titanic & 1 & 4 (4 by ICML) & 0.04 \\
% Cross-entropy & Iris & 0.0001 & 6 & 0.94 \\
% Cross-entropy & Iris & 0.01 & 4 & 0.10 \\
% Cross-entropy & Iris & 0.1 & 3 & 0.04 \\
% Cross-entropy & Iris & 1 & 2 & 0.02 \\
% Cross-entropy & Satellite & 0.0001 & 3 & 0.26\\
% Cross-entropy & Satellite & 0.01 & 2 & 0.08 \\
% Cross-entropy & Satellite & 0.1 & 1 & 0.05 \\
% Cross-entropy & Satellite & 1 & 1 & 0.05\\
% Sigmoid cross-entropy & ... & ... & 0 & \\
% Softmax cross-entropy & Titanic & 0.0001 & 7 & 2.07 \\
% Softmax cross-entropy & Titanic & 0.01 & 3 & 0.12 \\
% Softmax cross-entropy & Titanic & 0.1 & 1 & 0.05 \\
% Softmax cross-entropy &  Titanic & 1 & 0 & \\
% Softmax cross-entropy & Iris & 0.0001 & 3 & 0.25 \\
% Softmax cross-entropy & Iris & 0.01 & 1 & 0.03 \\
% Softmax cross-entropy & Iris & 0.1 or 1 & 0 & \\
% Softmax cross-entropy & Satellite & & 0 & \\
% \hline
%\end{tabular}
%\label{exp1}
%\end{table}
We now present our empirical evaluation of label inference attacks on cross-entropy loss and its extensions (see Appendix~\ref{app:experiments} for additional results)\footnote{All experiments are run on a 64-bit machine with 2.6GHz 6-Core processor, using the standard IEEE-754 double precision format. For reproducibility, the code is included as part of the supplementary material.}. We use the following datasets for our analysis. As our attacks construct prediction vectors that are independent of the dataset contents, we ignore the dataset features in our experiments. All the labels of the dataset are considered for the attack.
%\shiva{Zekun: can you upload all the plots as individual files, like in the ICML submission? That way we can set the spacing correctly.}
%\zeku{The individual figures are uploaded in the individual\_figure folder, with intuitive filenames. Please double check and rearrange as appropriate.}
\begin{CompactItemize}
    \item {\bf{Titanic}}~\cite{titanic}: a binary classification dataset (2201 rows) on the survival status of passengers.
    % , fetched from  \url{https://www.openml.org/d/40704}
    \item {\bf{Iris}}~\cite{iris}: a three-class classification dataset (150 rows) on the Iris species.
    \item {\bf{Satellite}}~\cite{satellite}: a six-class classification dataset (6430 rows) on the satellite images of soil.
\end{CompactItemize}
We consider three common loss functions (formally defined in Appendix~\ref{sec:logloss}): multiclass cross-entropy, softmax cross-entropy, and sigmoid cross-entropy (deferred to Appendix~\ref{app:experiments}). As a baseline, for the binary labeled dataset (Titanic) with the cross-entropy loss, we implemented the label inference attack of Aggarwal~\emph{et al.}\ \citep{aggarwal2021icml} (see Theorem~\ref{thm:from_icml}, Appendix~\ref{app:experiments} for a restatement of their main result).

We start with the distinction between our experiments and Algorithm~\LabelInf, which is presented in the $\textsc{APA}$ model\footnote{APA stands for Arbitrary Precision Arithmetic model (see Appendix~\ref{sec:apa_fpa}).}. For example in the multiclass cross-entropy loss (\Klogloss) case, to simulate Algorithm~\LabelInf on a finite precision machine, we must be able to differentiate $\min_{i,k}\theta_{i,k}$ from 0 (or else the label inference will be ambiguous). A rough analysis (from Theorem~\ref{thm:multi_class_proof}) gives that 
% $\min_{i,k}\theta_{i,k}\approx \vartheta_{N,1}/\vartheta_{N,K} = 3^{2^{(N-1)K+1}N\tau}/3^{2^{(N-1)K+K}N\tau}=\Omega(3^{-2^{NK}N\tau})$, which requires a precision of 
$\phi=\Omega(2^{NK}N\tau)$ bits are required to make this distinction. This bound hides constant factors and is likely not tight, but gives an idea of how arithmetic precision  plays a role in our experiments. 

Figure~\ref{fig:singlequery} shows the number of datapoints $N$ recovered by Algorithm~\LabelInf as we increase the noise for various loss functions. We sample 1000 random sets of labels each of length $N$ from the dataset here. At error magnitude $\tau = 1$, the noise is comparable to the actual loss function values computed. We measure accuracy as the percentage of labels correctly inferred out of $N$.
% (since the largest N for at least 50\% accuracy is 8 for sigmoid and softmax cross-entropy), 
Figure~\ref{fig:singlequery}(a) shows that the number of datapoints ($N$) for which 100\% label inference accuracy is achieved for cross-entropy loss decreases as the noise magnitude ($\tau$) increases, which is expected. Moreover, at the same noise magnitude, the accuracy also drops as the number of classes ($K$) increases from 2 (in Titanic) to 6 (in Satellite), which is also expected. These happen because of the dependence on number of datapoints and number of classes in our prediction vector construction (Theorem~\ref{thm:multi_class_proof}), which given fixed machine precision runs into representation issues. We note that for the Titanic dataset, the construction from~\cite{aggarwal2021icml} works slightly better (especially at lower $\tau$ values) than ours due to a small difference in the exponent: it holds that $\min_{i \in [N]}(-\ln \theta_{i}) = \Omega(2^N N\tau)$ in~\cite{aggarwal2021icml} (see Theorem~\ref{thm:from_icml}, Appendix~\ref{app:experiments}), but $\Omega(2^{2N}N\tau)$ when using Theorem~\ref{thm:multi_class_proof} with $K=2$.
% However, our construction is very general and extends to multiclass cross-entropy loss and beyond, which the construction in~\cite{aggarwal2021icml} does not handle.}. 

% Using the prediction vectors from Section~\ref{sec:logloss}, on these 1000 samples of length 8 from Titanic, the mean loss value is 3.64 for cross-entropy, 0.51 for sigmoid cross-entropy, and 0.81 for softmax cross-entropy.

% We further observe that for the Titanic dataset, the construction from~\cite{aggarwal2021icml} works slightly better (especially at lower $\tau$ values) than our construction provided by Theorem~\ref{thm:multi_class_proof}. This is due to a small difference in the exponent: we have $\min_{i \in [N]}\theta_{i} = \Omega(3^{-2^N N\tau})$ in~\cite{aggarwal2021icml} (see Appendix~\ref{app:experiments}), but $\Omega(3^{-2^{2N}N\tau})$ when using Theorem~\ref{thm:multi_class_proof} with $K=2$ (as mentioned above).
% On the other hand our construction is very general and extends to multiclass cross-entropy loss and beyond, which the construction in~\cite{aggarwal2021icml} does not handle.  

Figures~\ref{fig:singlequery}(b)-(c) show the number of datapoints on which Algorithm~\LabelInf achieves at least 50\% accuracy for cross-entropy and softmax cross-entropy loss. We notice this number is smaller for softmax cross-entropy as compared to regular cross-entropy (see Figure~\ref{fig:singlequery}(a)), which is also not surprising. Through a similar argument as that above for the number of bits required for cross-entropy loss, one can show that computing the softmax cross-entropy loss will require an additional $\Omega(NK + \ln(N\tau))$ bits (see the discussion in Appendix~\ref{app:experiments} for details). This additional requirement further constraints the number of labels that can be recovered with softmax cross-entropy loss.



% Finally, the longest computation time for a single label inference across all the experiments with $N=10$ is below 10 milliseconds. 
% In summary, our empirical results attest that these attacks can be performed effectively on real datasets, and also highlight some technical nuances when running label inference on machines with finite floating-point precision. 


% At $N=10$, $K=2$, and $\tau=0.0001$, this implies $\phi > 1000$. However, this upper bound is not tight, as we see in Figure \ref{fig:singlequery}(a) -- our 64-bit machine can perform perfect label inference on the Titanic dataset at noise 0.0001 for length 10. 

% We also ran a baseline label inference experiments on the Titanic dataset for cross-entropy, where the calibrated prediction vector $\theta$ from step 1 in Algorithm~\LabelInf is replaced by a uniformly random vector. We repeat the experiment 1,000 times and the maximum vector length at which 100\% accuracy is achieved is 3 and 1 at noise magnitude 0.0001 and 0.01, which are smaller than 10 and 8 by Algorithm~\LabelInf. When the noise magnitude increases to 0.1 and 1, the randomly generated vector cannot correctly infer label vector even at length 1 with 100\% accuracy.
% \abhi{Moving this closer to Algorithm~\LabelInf in the paper.}


 
 


 



%The median loss in the experiments is about 2.4 for cross-entropy (log-loss), 0.6 for sigmoid cross-entropy loss, and 1.12 for softmax cross-entropy loss. The longest run time for a single label inference across all the experiments based on Algorithm~\LabelInf in this section is below 10 milliseconds.
%\shiva{we need also results in all the plots for the unnoised case, maybe by setting $\tau$ to be extremely small}
 
%The fraction of correctly inferred labelings with respect to the length of the private vector is computed by running the label inference algorithm on 1000 labelings of each specific length randomly sampled from the corresponding dataset. 
 
%\shiva{This needs more discussion. Why is there a drop? Why does  Corollary~\ref{cor:APAFPA} not apply?}
 
%\shiva{can we show $9$ is almost close to what we expect based on the values? Remember the question in the ICML reviews which asked for something like this?}
%\shiva{Comparison to ICML does not show good results for us? We need to revisit this one?}





%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.26]{accuracy.png}
%    \caption{Results on  label inference using Algorithm~\LabelInf on the three real datasets: Titanic, Iris, and Satellite. The first row shows the performance of the label inference from log-loss. The second row shows the performance from sigmoid cross-entropy loss. The third row shows the performance from softmax cross-entropy loss. }
%    \label{accuracy}
%\end{figure}


%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.2]{binary_vs_icml.png}
%    \caption{Results comparing binary log-loss label inference using Algorithm~\LabelInf versus Algorithm 2 in ICML paper on the Titanic dataset. }
%    \label{binary_vs_icml}
%\end{figure}

%
%%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.2]{accuracy_multiquery.png}
%    \caption{Results on the multi-query label inference using Algorithm %\textsc{LabelInf} in shards from log-loss on the three real datasets: Titanic, Iris, and Satellite. }
%    \label{accuracy_multiquery}
%\end{figure}

==> neurips2021/short_paper_introduction.tex <==
Consider a situation where a machine learning (ML) modeler is interacting with a data curator. The data curator owns a private dataset for a classification task, and the curator agrees to evaluate on this private dataset the prediction vector (or an ML model) that the modeler submits, and replies back with loss function values. Such a situation is commonly encountered in machine learning competition settings like Kaggle~\cite{kaggle}, KDDCup~\cite{kdd_cup}, and ILSVRC Challenges~\cite{ilsvrc}. In some competitions, the features of the private (hold-out) dataset are revealed but not its labels, and the modeler submits the prediction vector on those features. In some other competitions, no information about the private dataset is revealed (i.e., neither the features nor the labels). The modeler submits a model that is then evaluated on the private dataset. In these settings, it is common for the curator to return the loss scores to the modeler (such as for the purposes of fine-turning the models or ranking etc.). A similar situation also appears when dealing with sensitive datasets, where either labels, or, both features and labels could be considered sensitive, and again a modeler and curator interact through loss scores. 

In this paper, we investigate if it is possible for a (malicious) modeler to recover all the private labels using these interactions with the data curator. 
% which has been split into a publicly available subset and a private subset. The curator exposes the public dataset for modelers to solve a classification task, which they can assess through interacting with the curator on the private dataset. For this evaluation, the modeler can submit their model predictions on the private dataset and the curator will reply with how accurate these predictions were, to help the modeler fine tune their model, as required. The labels for private dataset are never revealed to the modeler. Such a situation is commonly encountered in machine learning competition settings like Kaggle, KDDCup, and ILSVRC Challengs, where the modelers can only access the features in the private dataset but not its labels. 
More broadly, we investigate the problem of (robust) label inference, where the goal is to infer the labels of a hidden dataset from just the (noisy) loss function queries evaluated on the dataset. Our focus will be on a particularly strong inference attack where the modeler gets  {\em just one} loss query output, which could be distorted by noise. Surprisingly, we show that even with just this single query (and no access to the private feature set), for many common ML loss functions, our label inference attack succeeds in exactly recovering {\em  all} the true labels. This has important ramifications; for example, our attacks could be used by:
% \begin{list}{{\bf (\alph{enumi})}}
% 	{\usecounter{enumi}
% 		\setlength{\leftmargin}{14pt}
% 		\setlength{\listparindent}{14pt}
% 		\setlength{\parsep}{1pt}	
% }
% \item 
a) an unscrupulous participant to an ML competition who could learn the labels of the hold-out test set in order to construct a fake model that achieves perfect classification; or b) an adversary to execute a privacy breach by learning labels associated with a sensitive dataset (see our Ethics and Malpractice statement at the end).
% \footnote{See our ethics and malpractice statement at the end of this paper.\\} 
% \end{list}

% Through a notion of {\em codomain separability}, we characterize necessary and sufficient conditions for a loss function under which single query label inference is possible even with noisy responses. None of the presented attacks require any access to the private feature set or to any model training.

==> neurips2021/single_query_plot.tex <==
\begin{figure*}[t]
    \centering
    \vspace{-0.5em}
    \subfloat[]{\includegraphics[width=130pt]{neurips2021/individual_figure/logloss_100_singlequery.png}}
    \hspace{-0.1em}
    \subfloat[]{\includegraphics[width=130pt]{neurips2021/individual_figure/logloss_50_singlequery.png}} 
    \hspace{-0.1em}
    \subfloat[]{\includegraphics[width=130pt]{neurips2021/individual_figure/softmax_50_singlequery.png}}
    % \hspace{-0.1em}
    % \subfloat[]{\includegraphics[width=95pt]{individual_figure/softmax_50_singlequery.png}} 
    \vspace*{-1ex}
    \caption{Results for $\tau$-robust label inference using Algorithm~\LabelInf. Figures (a)-(b) plots the length of vector ($N$) on which Algorithm~\LabelInf always succeeds with multiclass cross-entropy loss with 100\%  and at least 50\% accuracy respectively. Here, Titanic$^{\star\star}$ implements the binary label inference attack proposed in~\cite{aggarwal2021icml}. Figure (c) plots the same for the softmax cross-entropy loss at 50\% accuracy (wherever computable). The computation time per inference attack is roughly 10 seconds.} 
    % \abhi{Reiterating Shiva's question here: Did we do multiple runs in these plots or just one run?}}
    \label{fig:singlequery}
    \vspace*{2ex}
\end{figure*}

==> overview.tex <==
\subsection{Reducing Robust Label Inference to Codomain Separability}
\label{sec:reduce_label_inference_to_codomain_separability}

\subsubsection{Connections to Blatant Non-Privacy}
\subsection{Results for Classes of Loss Functions}
\begin{theorem}[Additively Linearly Separable Losses]
\label{thm:linearly_separable_additive}
Let $\mathcal{L}:[0,1]^N \times \{0,1\}^N \to \mathbb{R}$ be a loss function such that for some invertible function $g:[0,1] \to \mathbb{R}$ and $h:[0,1]^N \to \mathbb{R}$, we can write:
$$\mathcal{L}(\theta,\sigma) = h(\theta) + \sum_{i=1}^N \sigma_i g(\theta_i).$$
Then, for given $\tau > 0$, the loss $\mathcal{L}$ is $\tau$-codomain separable using $\theta \in [0,1]^N$ with $\theta_i = g^{-1}(\tau \ln p_i)$, where $p_i$ denotes the $i^{th}$ prime number and assuming this inverse exists within the domain of $g$.
\end{theorem}

% \begin{theorem}[Multiplicatively Separable Losses]
% \label{thm:separable_multiplicative}
% Let $\mathcal{L}:[0,1]^N \times \{0,1\}^N \to \mathbb{R}$ be a loss function such that for some invertible function $g:[0,1] \to \mathbb{R}$ and $h:[0,1]^N \to \mathbb{R}$, we can write:
% $$\mathcal{L}(\theta,\sigma) = \prod_{i=1}^N \sigma_i g(\theta_i) + h(\theta).$$
% Then, for given $\tau > 0$, the loss $\mathcal{L}$ is $\tau$-codomain separable using $\theta \in [0,1]^N$ with $\theta_i = g^{-1}(p_i\tau)$, where $p_i$ denotes the $i^{th}$ prime number and assuming this inverse exists within the domain of $g$.
% \end{theorem}

\begin{theorem}[Bregman Divergence Based Losses]
\label{thm:bregman_general_result}
Let $F:[0,1] \times [0,1] \to \mathbb{R}$ be a strongly convex function and $DF(p,q) = F(p) - F(q) - \langle \nabla F(q),p - q\rangle$ be the Bregman divergence associated with $F$. Let $\mathcal{L}_F(\theta,\sigma)$ be the corresponding loss function, defined as follows:
$$\mathcal{L}_F(\theta,\sigma) = \frac{1}{N}\sum_{i=1}^N D_F([\sigma_i,1-\sigma_i], [\theta_i,1-\theta_i]).$$  
Then, the Bregman loss $\mathcal{L}_F(\theta,\sigma)$ is $\tau$-codomain separable for $\tau > 0$ using $\theta = [\theta_1,\dots,\theta_N]$ with the following:
$$\theta_i = \frac{N\tau \ln p_i + A}{B},$$
where $A = F([0,1]) + \langle \nabla F([1,0]), [1,-1] \rangle - F([1,0])$, and $B = \langle \nabla F([1,0]), [1,-1] \rangle-\langle \nabla F([0,1]), [1,-1] \rangle$ (assuming it is non-zero), and $p_i$ is the $i^{th}$ prime number.
\end{theorem}

\begin{theorem}[Composition with Inverse-Lipschitz Functions]
\label{thm:inverse_lipschitz}
Let $f:[0,1]^N \times \{0,1\}^N \to \mathbb{R}$ be $\tau$-codomain separable for some $\tau>0$ with respect to some $\theta \in [0,1]^N$. Let $g:\mathbb{R} \to \mathbb{R}$ be $k$-inverse Lipschitz for some constant $k > 0$. Then, the composition $g \circ f : [0,1]^N \times \{0,1\}^N \to \mathbb{R}$ is $k\tau$-codomain separable with respect to $\theta$.
\end{theorem}

% \subsection{Negative Results}
% \begin{theorem}
% \label{thm:lp_loss}
% For any $p > 0$, the function $f: \{0,1\}^N \times \{0,1\}^N \to \mathbb{R}$ of the form $f(\sigma,\theta) = \pnorm{p}{\theta-\sigma}$ is not $\tau$-codomain separable for any $\tau > 0$.
% \end{theorem}

% \begin{theorem}
% \label{thm:separability_monotonic}
% Let $\Omega = \{s_1,\dots,s_N\}$ be a set. Let $f: 2^\Omega \times \Theta \to \mathbb{R}_+$ be a function and $\theta \in \mathbb{R}^N$ be such that $f(\cdot,\theta)$ is monotonic, i.e.,, for all $A \subseteq B \subseteq [N]$, it holds that $f(A,\theta) \leq f(B,\theta)$. Then, $f$ is not $\tau$-codomain separable using $\theta$ for any 
% $$\tau > \min_{B \subset [N]}\min_{j \not\in B} \parfrac{f(B \cup \{j\},\theta) - f(B,\theta)}{2}.$$
% In particular, if $f(\emptyset,\theta) = 0$, then $f$ is not $\tau$-codomain separable using $\theta$ for any $\tau > \frac{1}{2} \paran{\min_{j \in [N]} f(\{j\},\theta)}$.
% \end{theorem}

% \begin{theorem}
% \label{thm:separability_monotonic_bounded}
% Let $\Omega = \{s_1,\dots,s_N\}$ be a set. Let $f: 2^\Omega \times \Theta  \to \mathbb{R}_+$ be a function such that $f(\cdot,\theta)$ is monotonic and $f(\cdot,\theta) \leq \beta$ for all $\theta \in \mathbb{R}^N$ and for some finite $\beta > 0$. Then, $f$ is not $\tau$-codomain separable for any $\tau > \beta/N$.
% \end{theorem}

% \subsection{Results on Computational Complexity and Model-Based Reconstruction}
% \begin{theorem}
% \textsc{Codomain-Separability} is Co-NP Hard.
% \end{theorem}

% \subsection{Model Based Reconstruction}
